Combinatorial geometry of neural codes, neural data analysis, and neural networks

This dissertation explores applications of discrete geometry in mathematical neuroscience. We begin with convex neural codes, which model the activity of hippocampal place cells and other neurons with convex receptive fields. In Chapter 4, we introduce order-forcing, a tool for constraining convex realizations of codes, and use it to construct new examples of non-convex codes with no local obstructions. In Chapter 5, we relate oriented matroids to convex neural codes, showing that a code has a realization with convex polytopes iff it is the image of a representable oriented matroid under a neural code morphism. We also show that determining whether a code is convex is at least as difficult as determining whether an oriented matroid is representable, implying that the problem of determining whether a code is convex is NP-hard. Next, we turn to the problem of the underlying rank of a matrix. This problem is motivated by the problem of determining the dimensionality of (neural) data which has been corrupted by an unknown monotone transformation. In Chapter 6, we introduce two tools for computing underlying rank, the minimal nodes and the Radon rank. We apply these to analyze calcium imaging data from a larval zebrafish. In Chapter 7, we explore the underlying rank in more detail, establish connections to oriented matroid theory, and show that computing underlying rank is also NP-hard. Finally, we study the dynamics of threshold-linear networks (TLNs), a simple model of the activity of neural circuits. In Chapter 9, we describe the nullcline arrangement of a threshold linear network, and show that a subset of its chambers are an attracting set. In Chapter 10, we focus on combinatorial threshold linear networks (CTLNs), which are TLNs defined from a directed graph. We prove that if the graph of a CTLN is a directed acyclic graph, then all trajectories of the CTLN approach a fixed point.

==> SupplementaryMaterial/Dedication.tex <==
% Place the dedication below.


==> SupplementaryMaterial/ListOfSymbols.tex <==
% Place the list of symbols below.
%\begin{eqlist}[\def\makelabel#1{\hfill#1}\labelsep 1em]
%
%%\item[$\alpha$]
%%The first greek letter, p.~\pageref{ChX-figure: FigureLabel3}
%%
%
%
%\end{eqlist}

==> SupplementaryMaterial/UserDefinedCommands.tex <==
% Place user-defined commands below.

% Define the \acro command.
\makeatletter
\newif\ifFirstPar       \FirstParfalse
\def\smc{\sc}
\def\ninepoint{\small}
\DeclareRobustCommand\SMC{%
  \ifx\@currsize\normalsize\small\else
   \ifx\@currsize\small\footnotesize\else
    \ifx\@currsize\footnotesize\scriptsize\else
     \ifx\@currsize\large\normalsize\else
      \ifx\@currsize\Large\large\else
       \ifx\@currsize\LARGE\Large\else
        \ifx\@currsize\scriptsize\tiny\else
         \ifx\@currsize\tiny\tiny\else
          \ifx\@currsize\huge\LARGE\else
           \ifx\@currsize\Huge\huge\else
            \small\SMC@unknown@warning
 \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi
}
\newcommand\SMC@unknown@warning{\TBWarning{\string\SMC: unrecognised
    text font size command -- using \string\small}}
\newcommand\textSMC[1]{{\SMC #1}}
\newcommand\acro[1]{\textSMC{#1}\@}

\makeatother

% command for vectors
\newcommand{\bv}[1]{\ensuremath{\vec{#1}}}
% command for unit vectors
\newcommand{\uv}[2][blank]{%
\ifthenelse{\equal{#1}{blank}}%
{\ensuremath{\hat{u}_{#2}}}%
{}%
%
\ifthenelse{\equal{#1}{.}}%
{\ensuremath{\dot{\hat{u}}_{#2}}}%
{}%
%
\ifthenelse{\equal{#1}{'}}%
{\ensuremath{\hat{u}'_{#2}}}%
{}%
}
\newcommand{\ui}{\ensuremath{\hat{\imath}}}
\newcommand{\uj}{\ensuremath{\hat{\jmath}}}
\newcommand{\uk}{\ensuremath{\hat{k}}}


==> ThresholdLinear/ThresholdLinear.tex <==
%auto-ignore 

% !TEX root = ../YourName-Dissertation.tex

\chapter{Threshold Linear Networks } \label{chapter:TLNs}
\section{Introduction}


Mathematical models of neural activity which are able to reproduce the rich variety of behavior observed in neural circuits must be nonlinear.
We study some of the simplest possible nonlinear models for neural activity, threshold-linear networks (TLNs). 
The firing rates $x_1, \ldots, x_n$ of neurons in a TLN are governed by the system of ordinary differential equations
\begin{align} \label{eqn:tln}
\frac{dx_i}{dt} &= -x_i + \left[\sum_{j = 1}^n W_{ij}x_j + b_i\right]_+,
\end{align}
which can be written in vector form as
\begin{align}
\frac{dx}{dt} &= -x + \left[Wx + b\right]_+. 
\end{align}
Here, $[y]_+ := \max\{y, 0\}$,  $W_{ij}$ the strength of the input to neuron $i$ from neuron $j$, and $ b$ is a constant external drive. 
TLNs have been used for decades as firing rate models of neural networks with simple, perceptron-like units. 
Because they are built out of locally linear systems, these networks are surprisingly tractable mathematically as compared to other high-dimensional nonlinear systems. 
However, while solutions to systems of linear ODEs either converge to a stable fixed point or diverge to infinity, solutions to TLNs can exhibit the full range of nonlinear behavior including multistability, limit cycles, and chaos. 

The activity of a neural circuit is determined by a variety of factors, such as intrinsic neural dynamics, external input, and the structure of network connectivity itself.  
Our goal is to understand the role of connectivity in shaping neural activity. 
Thus, we study models of neural activity which isolate the role of connectivity. 
Combinatorial threshold linear networks (CTLNs) are a special class of TLNs where $W$ is determined by a directed graph $G$ together with parameters $\epsilon$ and $\delta$ satisfying $\delta > 0$, $0< \epsilon< \frac{\delta}{\delta + 1}$, together with a constant external drive $\theta  >0   $ which is the same for all neurons.   
When $i\not \to j$, neuron $i$ strongly inhibits neuron $j$. When $i\to j$, neuron $i$ weakly inhibits neuron $j$. Values of $W_{ij}$ are given by the rule:

\vspace{-.15in}
\begin{align*}
W_{ij} = \begin{cases}
\;\;\; 0 &\mbox{ if }\,\, i = j\\
-1 + \epsilon&\mbox{ if } j \to i \mbox{ in }\,\, G\\
-1 - \delta &\mbox{ if } j \not \to i \mbox{ in }\,\, G.
\end{cases} 
\end{align*}
We interpret this as a network of $n$ excitatory neurons, against a background of instantaneous non-specific inhibition.  
Notice that the network is truly all-to-all connected, even when the graph $G$ is missing many edges. 
In particular, even networks which look feedforward are recurrent. CTLNs fall into a more general category of competitive TLNs, networks whose weights are negative. 
Given a competitive TLN with weight matrix $W$, we can define a graph $G_W$ by 
\[i\to j \mbox{ in } G_W \iff 	W_{ij}  > -1.\] 
Note that if $W$ is the weight matrix of a CTLN with graph $G$, $G_W = G$. We view the class of TLNs with graph $G$ as relaxations of the CTLN on $G$. 


A large body of work has focused on fixed points of TLNs in general and CTLNs in particular \cite{hahnloser2000permitted, 
curto2020combinatorial,  santander2021nerve, curto2019robust, curto2019fixed, curto2016pattern, curto2012flexible}. 
However, there is less known about their dynamic activity more broadly. On one end of the spectrum, the activity of a symmetric TLN always converges to a stable fixed point \cite{hahnloser2000permitted}. 
On the other end, \cite{morrison2016diversity} proves that CTLNs on oriented graphs with no sinks have bounded activity and no stable fixed points, and therefore must have persistent dynamic activity. 
It is possible to partially predict the structure of these attractors using graph properties \cite{parmelee2022core}. 
However, many CTLNs outside this family also exhibit persistent dynamic activity, and both dynamic attractors and stable fixed points can coexist in the same network. 
Even when a CTLN is guaranteed to have a dynamic attractor  by \cite{morrison2016diversity}, it is difficult to prove things about the structure of this attractor.  
One particular graph, the directed 3-cycle, is proved to have a limit cycle in \cite{bel2021periodic}. 


Here, we aim to characterize which CTLNs have dynamic attractors and which do not, and to constrain the dynamic attractors of CTLNs. 
Our proofs involve showing that we can force trajectories of TLNs into smaller regions of space. 
Because TLNs are threshold-linear, their nullclines are built from hyperplanes in a simple way.  
This allows us to use ideas from the theory of hyperplane arrangements, together with observations about the vector field in each chamber, to make conclusions about whether dynamic attractors are possible for networks corresponding to a given graph. 
Similar ideas are used in \cite{curto2020combinatorial} as a strategy for determining fixed points of general TLNs. 

We first prove that all trajectories of competitive TLNs approach and become trapped in a small region $\cA$ of phase space, corresponding to the set where at least one derivative is positive and at least one derivative is negative. This set is cut out by the hyperplanes defining the nullclines. 
\begin{ithm}
If $W,\theta$ defines a competitive TLN, $\cA$ is an attracting set, all trajectories approach it. 
\end{ithm}
This allows us to bound the total population activity of CTLNs: 
\begin{cor}
In CTLNs, \[\lim\inf_{t\to\infty} \sum_{i = 1}^n x_i \geq \frac{\theta}{1 + \delta}\] and  \[\lim\sup_{t\to\infty} \sum_{i = 1}^n x_i \leq \frac{\theta}{1 - \epsilon}.\] 
\end{cor}


We organize our work around the following conjecture: any CTLN with a dynamic attractor must have a proper directed cycle, as defined below. 
\begin{defn}
A \emph{proper directed cycle} of a directed graph is a directed cycle which has at least one edge which is not bidirectional. 
\end{defn}
\begin{conj}Let $G$ be a graph with no proper directed cycle. Then no CTLN with graph $G$ has a dynamic attractor. \label{conj:graph_struct}
\end{conj}

Note that the converse of this conjecture does not hold: see Figure \ref{fig:dir_no_attr} for an example of a graph which has a strongly directed cycle, but no dynamic attractor. 
We prove this conjecture in special cases. First, we note that applying the main result of \cite{hahnloser2000permitted} to symmetric CTLNs establishes that these networks do not have dynamic attractors. 
The next natural special case is the case of directed acyclic graphs (DAGs), graphs with no directed cycles at all. 

\begin{thm}
If $G$ is a directed acyclic graph, then no CTLN with graph $G$ has a dynamic attractor. \label{thm:dag}
\end{thm}

\begin{figure}
\begin{center}
\includegraphics[width = 5 in]{ThresholdLinear/Figures/tln_convergence_cases.pdf}
\end{center}
\caption{Classes of graphs such that all trajectories of their CTLNs are guaranteed to converge to a  fixed point.}
\label{fig:graph_classes}
\end{figure}


Thus, we have shown that CTLNs with either symmetric or feedforward architectures do not support dynamic attractors. 
It is natural to ask when it is possible to combine these two architectures to obtain a CTLN which we can guarantee has no dynamic attractors. 
One case in which we can do this is when a directed acyclic graph terminates on a symmetric graph. 

\begin{thm}
Let $G$ be a graph on vertex set $V$, and $\sigma, \tau$ be a partition of $V$. Suppose  the subgraph $G_\sigma$ is symmetric and connected, the subgraph $G_\tau$ is a directed acyclic graph, and that there are no edges from a vertex in $\tau$ back to a vertex in $\sigma$. 
Then no CTLN with graph $G$ has a dynamic attractor. \label{thm:dag_onto_symmetric}
\end{thm}

Our Conjecture \ref{conj:graph_struct} describes the much broader set of ways we believe it is possible to combine feedforward and symmetric elements to obtain a CTLN for which all trajectories are guaranteed to approach  a fixed point. 


Next, we explore to what extent our results extend to general competitive TLNs. In general, the graph $G$ does not determine the fixed point structure of the set of TLNs such that $G_W = G$ \cite{curto2019robust}. 
A graph $G$ is a \emph{robust motif} if all competitive TLNs with $G_W = G$ have the same set of fixed point supports. 
Almost all robust motifs fall into one of two infinite families, DAG1 and DAG2, with only a handful of exceptions. 
If $G$ is a robust motif, does the graph structure determine not just the fixed point structure of the graph, but also the presence of dynamic attractors?  Competitive TLNs with $G_W$ in either of these families each have a single stable fixed point. Further, in the CTLN case, these graphs have no dynamic attractors by our Theorems \ref{thm:dag} and \ref{thm:dag_onto_symmetric}, thus all trajectories approach the single stable fixed point.  It is natural to ask whether these graphs are ``dynamically robust": is it still true that all trajectories approach the single stable fixed point for all competitive TLNs such that $G_W$ is a member of DAG1 or DAG2? We conjecture that this is the case, and prove it in a special case, for graphs in a family we define and name \emph{shallow DAG1}. 

\begin{thm}
Let $G$ be a member of shallow DAG1. Then in any competitive TLN with $G_W = G$, all trajectories approach the single stable fixed point. 
\end{thm}






%Next, we use the combinatorial concept of domination, introduced in \cite{curto2019fixed}, to further constrain trajectories in terms of graph structure. In particular, we define strong and weak domination in terms of the graph structure of a CTLN, and show that this gives a constraint on its trajectories which we use to construct a dynamic memory network. 
%
%\begin{thm}
%\,
%\begin{itemize}
%\item If $k$ weakly dominates $j$, then the set $\{ x\in \R^n\mid x_k \geq x_j\}$ is a forward invariant set. That is, if $x_k \geq x_j$ at any time, then $x_k$ will remain greater than $x_j$ 
%
%\item If $k$ strongly dominates $j$, then the set $\{ x\in \R^n\mid x_k \geq x_j\}$ is an attracting setThat is, for all $\eta > 0$, there exists some $T_\eta \geq 0$ such that for all $t \geq T_\eta$, $x_k(t) +\eta > x_j(t)$. 
%
%\item If $k$ and $j$ receive equal input, the ordering of $x_k$ and $x_j$ is fixed. 
%\end{itemize}
%\end{thm}
%
%
%
%
%Next, we introduce  \emph{local Lyupanov-like functions}, which allow us to prove that trajectories of CTLNs become trapped in even smaller regions. Using this technique, we can constrain trajectories of CTLNs based on graph structure. This allows us to work towards a characterization of which CTLNs support dynamic attractors. In particular, \cite{curto2019fixed} proves that 	``sources die": if a neuron is a proper source in $G$, then it is not contained in the support of any fixed point of $G$. We prove a dynamic version of this result: if a graph $G$ satisfies a certain technical condition, then the activity of one of its sources must approach zero. 
%
%\begin{thm}
%\label{thm:sources_die}
%Let $G$ be a graph in which every vertex is reachable from a source. Then there is a source $j$ in $G$ such that $\lim_{t\to \infty} x_j(t) = 0$. 
%\end{thm}
%
%We use this result to obtain Theorems \ref{thm:dag} and \ref{thm:dag_onto_symmetric}. 
We also apply our results to classify CTLNs on three neurons. We prove that only the directed three-cycle has a dynamic attractor. 

\begin{thm}
The three-cycle is the only three neuron CTLN with persistent dynamic activity. 
\end{thm}





\section{Background}
Threshold linear networks (TLNs) are systems of ordinary differential equations whose dynamics are governed by Equation \ref{eqn:tln}. In this work, we are concerned with competitive TLNs. 
\begin{defn}
A TLN is \emph{competitive} if $W_{ij} \leq 0$ and $W_{ii} = 0$ for all $i$ and $j$, and $\theta \geq 0$.  
\end{defn}

Competitive TLNs always have bounded activity. While we will establish stronger bounds in this paper with Corollary \ref{cor:total_pop}, from \cite{curto2019fixed}, we have that trajectories of competitive TLNs which start in a box containing the origin stay there: if $x(0) \in \prod_{i = 1}^n[0, \theta]$, then $x(t) \in \prod_{i = 1}^n[0, \theta]$ for all $t >  0$.



Even though TLNs are nonlinear, they are locally or ``patchwork" linear. 
%, as illustrated in Figure \ref{fig:tln_eqn}.  That is, we can divide up the positive orthant into at most $2^n$ chambers based on whether $\sum_{j = 1}^n W_{ij}x_j + \theta \geq 0$ or  $\sum_{j = 1}^n W_{ij}x_j + \theta <0 $ for each $i$. We label each chamber by the set $\sigma = \{i \mid \sum_{j = 1}^n W_{ij}x_j + \theta \geq 0\}$. Within chamber $\sigma$, the dynamics are governed by the purely linear dynamical system 
%\begin{align*}
%\frac{dx_i}{dt} =\begin{cases} -x_i + W_{ij}x_j + \theta \qquad &i\in \theta\\
% -x_i \qquad &i \notin\theta.
% \end{cases}
%\end{align*}
%Define $A^\sigma$ to be the matrix of this linear system. That is, if $i\in \sigma$, the $i^{th}$ row of $A^\sigma$ is equal to the $i^{th}$ row of $-I + W$, and if $i\notin \sigma$, the $i^{th}$ row of $A_\sigma$ is equal to the $i^{th}$ row of $-I$. 
%
%\begin{figure}
%\begin{center}
%\includegraphics[width = 4 in]{ThresholdLinear/Figures/tln_equations.pdf}
%\end{center}
%\caption{TLNs can be seen as patchwork-linear networks, with a different linear system being active in each polyhedral chamber. \label{fig:tln_eqn}}
%\end{figure}
The fixed points of a dynamical system are the points $x^*\in \R^d$ such that 
$\frac{dx_i}{dt}\Big|_{x^*} = \,0$ for all $i\in [n]$. Because of patchwork linearity, each fixed point of a TLN must be a fixed point of the relevant linear system. However, a fixed point of a linear system may fail to be a fixed point of the TLN if that fixed point falls outside of the appropriate linear chamber. The \emph{support} of a fixed point is its set of active: $x^*$ is $\mathrm{supp}(x^*) := \{i \in [n]\mid x_i^* > 0\}$. There is at most one fixed point per support.  The set of fixed point supports for the TLN defined by $W, b$ is denoted $\FP(W, b)$. 

A fixed point is \emph{stable} if it is approached by all trajectories which start nearby. 
%The stability of a fixed point $x^*$ of a nonlinear system is determined by the eigenvalues of the Jacobian at $x^*$. In particular, $x^*$ is a stable fixed point if all of these eigenvalues have negative real part. Because TLN's are patchwork linear, the Jacobian at a point is just the matrix $A^\sigma$ of the linear system active in that chamber. Thus, the fixed point with support $\sigma$ of the TLN defined by $W, \theta$, if it exists, is stable if and only if all eigenvalues of the matrix $A^\sigma$ have negative real part.
Stable fixed points are a particular kind of attractor. 
\begin{defn}
A set $A$ is an \emph{attracting set} of a dynamical system if 
\begin{enumerate}
\item 
it is invariant: if $x (0) \in A$, then $x(t) \in A$ for all $t \geq 0$. 
\item 
it has an open basin of attraction: there is an open set $U$ containing $A$ such that if $x (0)\in U$, then the distance from $x(t)$ to $A$ approaches zero as $t$ approaches infinity. 
\end{enumerate}
An \emph{attractor} is a \emph{minimal} attracting set. That is, $A$ is an attractor if it is an attracting set and there is no $B\subsetneq A$ that is also an attracting set. 
\end{defn}
There are many attractors beyond stable fixed points, termed \emph{dynamic attractors}. These include limit cycles and strange attractors.   
By the main result of \cite{hahnloser2000permitted}, if the weight matrix $W$ is symmetric and the matrix $(I-W)$ is copositive, then the TLN defined by $W$ has a set of stable fixed points, and all trajectories of the network must approach one of these states. In particular, competitive TLNs satisfy this copositivity condition. Thus all trajectories of symmetric competitive TLNs (such as CTLNs defined from undirected graphs) must approach stable fixed points. Thus, these networks do not have dynamic attractors. 

On the opposite side of the spectrum, \cite{morrison2016diversity} proves that if $G$ is an oriented graph with no sinks, the CTLN defined by $G$ has no stable fixed points. Because trajectories of these networks cannot approach stable fixed points and cannot diverge to infinity, these networks must have dynamic attractors.  In one case, the directed three-cycle, this dynamic attractor has been explicitly characterized as a stable limit cycle \cite{bel2021periodic}. 

% I don't know where this paragraph should go. Move it up? Move it down? 
While Equation \ref{eqn:tln} is a common model for neural activity, other threshold linear models for neural activity appear in the literature, such as 
\begin{align} \label{eqn:tln_2}
\frac{d\mathbf v}{dt} &= -\mathbf v + W[\mathbf v]_+ +\theta\end{align}
The equivalence of models \ref{eqn:tln} and \ref{eqn:tln_2} is proven in \cite{miller2012mathematical}, generalizing a result from \cite{beer2006parameter}. When $W$ is invertible and $\theta$ is constant, \cite{beer2006parameter} shows that if $x$ evolves according to \ref{eqn:tln} if and only if $ v = W x + \theta$ evolves according to \ref{eqn:tln_2}. The more general case, when $W$ may not be invertible and $\theta$ may vary over time, is tackled in \cite{miller2012mathematical}. 	 

 \subsection{Nullclines, geometric picture}
We begin by describing nullclines of threshold linear networks in terms of hyperplane arrangements. 
A deeper account of the nullcline arrangement of a threshold linear network, from the perspective of oriented matroid theory, can be found in \cite{curto2020combinatorial}. 
\subsubsection{Defining nullclines}


The $i^{th}$ nullcline $\cN_i$ of a dynamical system is the set of all $x \in \R^n$ such that 
$\xdot_i = 0.$
Nullclines of linear systems are hyperplanes.
Because TLNs are threshold-linear, their nullclines are unions of pieces of hyperplanes. 


\begin{defn}
Given a weight matrix $W\in \R^{n\times n}$, $\theta \in \R$, we define affine-linear functionals
\begin{align*}
e_i^*(x) &:= -x_i\\
h_i^*(x) &:= -x_i + \sum_{j=1}^n W_{ij}x_j + \theta.
\end{align*}
These define hyperplanes $E_1, \ldots, E_n, H_1, \ldots, H_n $. The hyperplane arrangement of the TLN defined by $W$ and $\theta$ is the set $$\cA(W, \theta) = \{E_1, \ldots, E_n,H_1, \ldots, H_n\},$$ with the orientation (i.e. choice of positive and negative half-spaces) of each hyperplane given by $e_i^*$, $h_i^*$.   
\end{defn}

We describe the nullclines in terms of the hyperplanes $E_1, \ldots, E_n, H_1, \ldots, H_n$. 

\begin{prop}
The $i^{th}$ nullcline of a TLN is 
$$\cN_i = \left(H_i\cap E_i^-\right)\cup \left(E_i \cap H_i^-\right).$$
\end{prop}

\begin{proof}
We show that $x_i' < 0$ if and only if  $\vec{x}\in H_i^-\cap E_i^-$, and $x_i' > 0$ if $x \in H_i^+\cup E_i^+$. If $x\in H_i^-\cap E_i^-$, then  $$\max\left\{-x_i, -x_i + \sum_{j=1}^n W_{ij}x_j + \theta\right\} = -x_i + \left[\sum_{j=1}^n W_{ij}x_j + \theta\right]_+ < 0,$$ so $x_i' < 0$.  Now, if $x \in H_i^+\cup E_i^+$, then 
$$\max\left\{-x_i, -x_i + \sum_{j=1}^n W_{ij}x_j + \theta\right\} = -x_i + \left[\sum_{j=1}^n W_{ij}x_j + \theta\right]_+ > 0,$$
so $x_i' > 0$. 
Now, by continuity, we must have $x_i' = 0$ on the boundary between $H_i^-\cap E_i^-$ and $H_i^+\cup E_i^+$, which is the set $\left(H_i\cap E_i^-\right)\cup \left(E_i \cap H_i^-\right)$. 
\end{proof} 


\begin{ex}



Let $G$ be a the graph consisting of two vertices and a single directed edge from vertex 2 to vertex 1. Then the TLN arising from $G$ has the weight matrix 
$$W =  
\begin{pmatrix}
0& -1+ \epsilon \\
-1-\delta & 0
\end{pmatrix}.$$

\label{ex:edge_null}
\begin{figure}[ht!]
\includegraphics{ThresholdLinear/Figures/n=2_hyperplanes.pdf}
\caption{Nullclines for the CTLN of a single directed edge. The $x_1$ nullclines, $E_1$ and $H_1$, are in red, $E_2$ and $H_2$ are in blue. Black arrows point towards the positive side of each hyperplane. \label{fig:nullcline_edge}}
\end{figure}

The hyperplanes $E_1, E_2, H_1, H_2$, shown in the Figure \ref{fig:nullcline_edge}, are given by the equations 
\begin{align*}
E_1 &= \{x | -x_1 = 0\}\\
E_2 &= \{x | -x_2 = 0\}\\
H_1 &= \{x | -x_1 + (-1+\epsilon)x_2 + \theta = 0\}\\
H_2 &= \{x | -x_2 + (-1-\delta)x_2 + \theta = 0\}.
\end{align*}
The $x_1$ nullcline consists of the piece of $H_1$ on the negative side of $E_1$ together with the piece of $E_1$ on the negative side of $H_1$. Likewise, the $x_2$ nullcline consists of the piece of $H_2$ on the negative side of $E_2$ together with the piece of $E_2$ on the negative side of $H_2$. The pieces of $E_1, E_2, H_1$, and $H_2$ which act as nullclines are shown in darker colors in Figure \ref{fig:nullcline_edge}. The fixed point of this TLN is the point of intersection between these two nullclines, and appears as a white disk in the figure. 


\end{ex}

Notice that in this example, the fixed point occurs at the intersection of both nullclines. This is true in general: the set of fixed points of a TLN is the intersection of all of the nullclines, since this is exactly the set where all derivatives are zero.

%%%%%%%%%%%%%%%%%%%%%%%%% Drawing Nullclines %%%%%%%%%%%%%%%%%%%%%%%%%%%%positive orthant. This allows us to describe the $H_i$ in terms of convex hulls, which is helpful when sketching the nullclines. 
The following proposition makes it easier to sketch nullclines, especially in three dimensions. 
\begin{prop}\label{prop:cvx_hull}
Let $W$ be a competitive TLN. Define $b_{ij} = \frac{-\theta}{W_{ij}}e_j$ for $i\neq j$, $ b_{ii} = \theta \,e_i$. Then
\begin{align*}
H_i \cap \R^n_{\geq 0} =  \conv\left(\{b_{ij}\mid j = 1, ..., n\}\right).
\end{align*}
\end{prop}

\begin{proof}
Recall that $H_i$ is the zero set of 
$$h_i^*(x) = -x_i + \sum_{j=1}^n W_{ij}x_j + \theta.$$
Along the $x_j$ axis generated by $e_j$, we can set the other variables to zero, so for $i\neq j$, we have
\begin{align*}
0 = h_i^*(x) =  W_{ij}x_j + \theta\\
x_j = \frac{-\theta}{W_{ij}}
\end{align*}
and for $i = j$, 
\begin{align*}
0 = h_i^*(x) =  -x_i  + \theta\\
x_i = \theta 
\end{align*}
Thus, for each $j$, $b_j$ is the intersection of $H_i$ with the $x_j$ axis.  Thus, these points and their affine span are contained in $H_i$. These points are affinely independent, and there are $n$ of them, so affine span is equal to $H_i$. That is, each point of $H_i$ can be written as 
$$x = \sum \lambda_j b_j$$
subject to the constraint that $\sum_{j = 1}^n \lambda_j = 1$. 

Now, if $x\in H_i\cap \R^n_+$, we can take each $\lambda_i \geq 0$. Thus, $x$ a convex combination of the points $\{b_j\mid j = 1, \ldots, n\}$. Thus, $H_i \cap \R^n_{\geq 0} =  \conv\left(\{ b_{ij}\mid j = 1, ..., n\}\right)$. 
\end{proof}

\begin{ex}
We use Proposition \ref{prop:cvx_hull} to sketch nullclines for the CTLN corresponding to the graph $G = (V = \{1, 2, 3\}, E = \{2\to 1, 2 \to 3\})$ in Figure \ref{fig:nullclines_3}. Notice that specializing to the case of CTLNs simplifies our descriptions of the points $ b_{ij}$. If $j \not\to i$, $b_{ij} = \frac{\theta}{1+ \delta}$ and if $j \to i$, $ b_{ij} = \frac{\theta}{1-\epsilon}$. Also notice that $\frac{\theta}{1+ \delta} < \theta < \frac{\theta}{1-\epsilon}$. Thus, the absence or presence of an edge $j \to i$ tells us how the point where $H_j$ intersects the $x_i$ relates to the point where $H_i$ intersects the $x_i$ axis. The fixed points lie at the points of intersection between all three nullclines. These are marked with white circles. 
\begin{figure}[ht!]
\includegraphics[width = 6 in]{ThresholdLinear/Figures/nullclines_3.pdf}
\caption{Nullclines for a CTLN on three neurons.\label{fig:nullclines_3}}
\end{figure}
\end{ex}

\section{Nullcline chambers and dynamics}
\subsection{Basic definitions}
In the previous section, we talked about how the hyperplane arrangement $\cA(W, \theta)$ controls the fixed points of a TLN. Now, we explore how the hyperplane arrangement controls other dynamic properties of the TLN. In particular, we discuss the \emph{chambers} of this arrangement. These chambers are defined by the sign of the derivative at each point of $\R^n$.  

\begin{defn}
A \emph{sign vector} $X$ of length $n$ is an element of $\{0, +, -\}^n$. 
\end{defn}

\begin{defn}
Given a TLN defined by $W, \theta$ and a sign vector $X$, we define the \emph{chamber} of $X$ to be the set 
\begin{align*}
A_{W, \theta}(X) = \{x \in \R^n \mid \sign(x_i') = X_i\}.
\end{align*}
\end{defn}
Because TLNs are threshold linear, these chambers can be described in terms of the hyperplane arrangement. 
\begin{prop}
Let $X\in \{0,+, -\}^n$. 
\begin{align*}
A_{W, \theta}(X) = \bigcap_{X_i = +} (H_i ^+\cup E_i^+) \cap \bigcap_{X_j = -} (H_j^- \cap E_j^-) \cap \bigcap_{X_k = 0}\left( \left(H_i\cap E_i^-\right)\cup \left(E_i \cap H_i^-\right)\right).
\end{align*}
Within the strictly positive orthant, $\R^n_> = \{x\in \R^n\mid x_i > 0 \mbox{ for all } n \}$ this simplifies to 
\begin{align*}
A_{W, \theta}(X)\cap \R^n_> = \bigcap_{X_i = +} H_i ^+ \cap \bigcap_{X_j = -} H_j^-  \cap \bigcap_{X_k = 0} H_i
\end{align*}
\end{prop}

\begin{ex}
In Figure \ref{fig:edge_chambers}, we show the nullcline chambers for the graph with the single edge $1\to 2$. The four maximal nullcline chambers are the four possible sign vectors on $\{+, -\}^n$, $--, -+, +-, ++$. However, restricting to the positive orthant cuts off the $-+$, leaving us with three chambers $--, +-, ++$. 
\begin{figure}[ht!]
\includegraphics[width = 4 in]{ThresholdLinear/Figures/with_topes_labeled.pdf}
\caption{Maximal nullcline chambers for the single directed edge. The positive side of each hyperplane is indicated with an arrow. Additionally, the the positive side of each nullcline is shaded. Each chamber is labeled with the appropriate sign vector. \label{fig:edge_chambers}}
\end{figure}
\end{ex}

%%%%%%%%%%%%%%%%%%%%%%%% MIXED SIGN CHAMBERS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Activity sucked into union of mixed-sign chambers}
Now, we show that for competitive TLNs the chambers of $--\ldots-$ and $++\ldots+$ are repelling, and that all trajectories of the TLN eventually approach the union of the mixed-sign chambers. This constrains trajectories to a small subset of the positive orthant. 


\begin{defn}
We define the \emph{mixed sign region} $\cA$ as the closure of the set 
$$\{x\in \R^{n}_{\geq 0} \mid \mbox{ there exist } \, i, j \mbox{ such that } \sign(\xdot_i) = - \mbox{ and } \sign(\xdot_j) = +\}.$$
That is, $\cA$ is the region where not all derivatives have the same sign. 
Similarly, we define the two pieces of the complement of $\cA$ as
\begin{align*}
\cA^+ &= \{x\in \R^{n}_{\geq 0} \mid  \sign(\xdot_i) = +  \mbox{ for all } i\}\\
\cA^- &= \{x\in \R^{n}_{\geq 0} \mid  \sign(\xdot_i) = -  \mbox{ for all } i\}.
\end{align*}
\end{defn}
Notice that $\cA$ is bounded by the nullclines. In particular, within the positive orthant, it is bounded by the hyperplanes $H_1, \ldots, H_n$. Since the fixed points are the points where all nullclines intersect, they are always on the boundary of the mixed-sign chamber. A two-dimensional example is illustrated in Figure \ref{fig:mixed_sign}. 


\begin{thm}\label{thm:mixed_sign}
For any competitive TLN, the mixed sign region $\cA$ is a globally attracting set. In particular, trajectories which enter $\cA$ cannot leave. 
\end{thm}

\begin{proof}
First, note that within $\cA^+$, all derivatives $\xdot_i$ are positive. Thus, the trajectory must approach the boundary between $\cA^+$ and $\cA$. Likewise, within $\cA^-$, all derivatives $\xdot_i$ are negative, thus  the trajectory must approach the boundary between $\cA^-$ and $\cA$. 

Next, we show that if a trajectory is on the boundary between either $\cA^+$ and $\cA$ or $\cA^-$ and $\cA$, it must enter $\cA$. We first consider the boundary between $\cA^+$ and $\cA$. Since $W$ is the weight matrix of a competitive TLN, all entries of the normal vector $\vec h_i$ to the hyperplane $H_i$ are negative for all $i$. 
On the boundary between $\cA^+$ and $\cA$,  $\xdot \geq 0$ in all coordinates. Thus, $ \xdot\cdot \vec h_i \leq 0$, with equality only achieved at fixed points. Thus, unless the trajectory is at a fixed point, it must cross from $\cA^+$ into $\cA$. Likewise, if the trajectory is on the boundary between $\cA^-$ and $\cA$, $\xdot \leq 0$ in all coordinates.   Thus, $ \xdot\cdot \vec h_i \geq 0$, with equality only achieved at fixed points. Thus, the trajectory must cross from $\cA^+$ into $\cA$. 
\end{proof}



We can use this result to derive bounds on the total population activity of competitive TLNs in general, and CTLNs in particular.  

\begin{cor}\label{cor:total_pop}
Let $m = \min_{i, j}\{(I - W_{ij})\}$ and $M = \max_{i, j}\{(I - W_{ij})\}$. 
In competitive TLNs, 
\[\lim\inf_{t\to\infty} \sum_{i = 1}^n x_i \geq \frac{\theta}{M}\] and  \[\lim\sup_{t\to\infty} \sum_{i = 1}^n x_i \leq \frac{\theta}{m}.\] 
In CTLNs this result specializes to \[\lim\inf_{t\to\infty} \sum_{i = 1}^n x_i \geq \frac{\theta}{1 +\delta}\] and  \[\lim\sup_{t\to\infty} \sum_{i = 1}^n x_i \leq \frac{\theta}{1 -\epsilon}.\] 
\end{cor}

\begin{proof}
We show that, within the positive orthant, $\cA$ is contained between the hyperplanes $$\sum_{i = 1}^n x_i -\frac{\theta}{M} = 0 $$ and $$\sum_{i = 1}^n x_i - \frac{\theta}{m} =0.$$
By Proposition \ref{prop:cvx_hull}, for each $i$, the hyperplane $H_i$ is the convex hull of the points $\mathbf b_{ij} = \frac{-\theta}{W_{ij}}\mathbf{e_j}$ for $i\neq j$, $\mathbf b_{ii} = \theta \,\mathbf e_i$. Each point $\vec b_{ij}$ is on the positive side of the hyperplane defined by $\sum_{i = 1}^n x_i -\frac{\theta}{M} = 0 $ and on the negative side of the hyperplane defined by $\sum_{i = 1}^n x_i - \frac{\theta}{m} =0$. Thus, since all trajectories must approach $\cA$, they must also approach the region between the hyperplanes $\sum_{i = 1}^n x_i -\frac{\theta}{M} = 0 $ and $\sum_{i = 1}^n x_i - \frac{\theta}{m} =0$. Thus, 
\[\lim\inf_{t\to\infty} \sum_{i = 1}^n x_i \geq \frac{\theta}{M}\] and  \[\lim\sup_{t\to\infty} \sum_{i = 1}^n x_i \leq \frac{\theta}{m}.\] 
If $W$ is the matrix of a CTLN, then $m = 1-\epsilon$ and $M = 1+ \delta$, thus 
\[\lim\inf_{t\to\infty} \sum_{i = 1}^n x_i \geq \frac{\theta}{1 +\delta}\] and  \[\lim\sup_{t\to\infty} \sum_{i = 1}^n x_i \leq \frac{\theta}{1 -\epsilon}.\] 

\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%% NULLCLINE CHAMBERS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{How nullcline chambers shape dynamics}
\begin{defn}
Define a directed graph $T_{W, \theta} = (V, E)$ whose vertices correspond to nullcline chambers of the TLN defined by $W, \theta$ and whose edges correspond to possible transitions between chambers. That is, 
$V = \{ X\in \{+, -\}^n\mid A_{W, \theta, X} \neq \emptyset\}$, and the edge $(X\to Y) \in E$ if there is a point $x$ on the boundary between $X$ and $Y$ such that $\vec{\xdot}$ points from $X$ to $Y$. 
\end{defn}

We now prove that trajectories follow the edges of $T_{W, \theta}$. 
\begin{lem}\label{lem:folloW_edges}
Any trajectory of the TLN defined by $W, \theta$ must follow a directed path in $T_{W, \theta}$. 
\end{lem}

\begin{proof}
Suppose a trajectory crosses directly from the chamber $A_{W, \theta}(X)$ to the chamber $A_{W, \theta}(Y)$. Then at some time $t$, $x(t)$ is on the boundary between $A_{W, \theta}(X)$ and $A_{W, \theta}(Y)$. The direction it is going at time $t$ is given by $\xdot(t)$. Thus, in order to cross from $A_{W, \theta}(X)$ to $A_{W, \theta}(Y)$, $\xdot(t)$ must point from $A_{W, \theta}(X)$ to $A_{W, \theta}(Y)$.
\end{proof}

\begin{ex}
We consider again the directed edge. We have $T_{W, \theta} = (V, E)$ with $V = \{--, +-, ++\}$ and $E = \{(-- \to +-), (++ \to +-)$\}. To see this, we first note that edges must be between adjacent chambers. The edge between $--$ and $+-$ corresponds to crossing the $x_1$ nullcline $H_1$. On this nullcline, we have $x_1' = 0$ and $x_2' < 0$. Thus, we are going straight down. Therefore, $\xdot$ points from the chamber $--$ to the chamber $+-$. The edge between $++$ and $+-$ corresponds to crossing the $x_2$ nullcline. On this nullcline, we have $x_2' = 0$, $x_1' > 0$. Thus, we are going right. Therefore, whenever we cross this nullcline, we must cross from the chamber $++$ to the chamber $+-$. 

\begin{figure}[ht!]
\includegraphics[width = 4 in]{ThresholdLinear/Figures/transition_graph_edge.pdf}
\caption{The transition graph $T_{W, \theta}$ for the single directed edge. The gray arrows are the vectors $\xdot$ on the nullclines.  \label{fig:trans_graph}}
\end{figure}
\end{ex}

Not only must transitions between chambers follow edges of $T_{W, \theta}$, dynamic attractors must follow directed cycles in  $T_{W, \theta}$. To prove this, it is sufficient to prove that single chambers of  $T_{W, \theta}$ to not contain dynamic attractors. 


\begin{lem}\label{lem:single_chamber}
If a trajectory is contained on one side of the $i^{th}$ nullcline, then the value of $x_i(t)$ along this nullcline approaches a limit.  If a trajectory of a TLN is contained within a nullcline single chamber, then it approaches a fixed point. 
\end{lem}

\begin{proof}
If a trajectory is contained on one side of the $i^{th}$ nullcline, then the sign of $x_i'(t)$ along this trajectory is fixed. Thus, the function $x_i(t)$ is bounded and is either monotonically increasing or monotonically decreasing. Thus, $x_i(t)$ approaches a limit. 

Within a single chamber of $A_{W, \theta, X}$,  $x_i(t)$ approaches a limit for all $i = 1, ..., n$, thus the trajectory approaches a fixed point. 
\end{proof}

\begin{prop}\label{prop:directed_cycle} Any dynamic attractor of the TLN defined by $W, \theta$ must follow a directed cycle of $T_{W, \theta}$. 
\end{prop}

\begin{proof}
By Lemma \ref{lem:folloW_edges}, any trajectory must follow edges of $T_{W, \theta}$. By Lemma \ref{lem:single_chamber}, a dynamic attractor can never become trapped in a single chamber. Thus, it must transition between chambers infinitely many times. Since $T_{W, \theta}$ has only finitely many vertices of, the trajectory must thus return to a chamber is has visited before, thus following a directed cycle.  
\end{proof}

Proposition \ref{prop:directed_cycle} allows us to prove that a given TLN does not have a dynamic attractor. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% n = 2 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{$N = 2$ competitive TLN classification}
\begin{figure}[ht!]
\includegraphics[width = 5 in]{ThresholdLinear/Figures/n_2_class.pdf}
\caption{In each subplot, we have the nullcline arrangement and transition graph $T_{W, \theta}$ corresponding to the connectivity graph in the upper right corner. Gray arrows on nullclines give the direction of the derivative on this piece of the nullclines. \label{fig:n_2_class}}
\end{figure}

The transition graph $T_{W, \theta}$ allows us to easily prove that competitive TLNs with two neurons do not have dynamic attractors.

\begin{prop}\label{prop:n=2}
All trajectories of competitive TLNs with two neurons converge to stable fixed points. 
\end{prop}

\begin{proof}
The transition graph $T_{W, \theta}$ is completely determined by the connectivity graph $G_{W, \theta}$. In particular, if $W_{12} \leq -1$, the intersection of $H_1$ with the $x_2$ axis is closer to the origin than the intersection of $H_2$ with the $x_2$ axis, and if $W_{12} \leq -1$ the intersection of $H_1$ with the $x_2$ axis is further from the origin than the intersection of $H_2$ with the $x_2$ axis. Similarly, the relationship between $W_{21}$ and -1 determines the relative positions of the intersections of $H_1$ and $H_2$ with the $x_1$ axis. These relationships are sufficient to completely determine all combinatorial properties of the hyperplane arrangement $E_1, E_2, H_1, H_2$, and thus the graph $T_{W, \theta}$.  All possible arrangements are shown in Figure \ref{fig:n_2_class}. We notice that none of these graphs have directed cycles. Thus, by Proposition \ref{prop:directed_cycle}, none of these graphs have dynamic attractors.  
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%% n = 2, noncompetitive %%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Non-competitive TLNs for $n = 2$ }

While we have shown that competitive TLN's with 2 neurons, this result does not hold for general TLNs with two neurons. In particular, we consider the TLN defined by 
\begin{align*}
W = \begin{pmatrix}
2 & -1 \\ 2 & 0
\end{pmatrix} && \theta = \begin{pmatrix}
2 \\ 1 
\end{pmatrix},
\end{align*}
which is introduced in \cite{tang2005analysis}. This TLN does, in fact, have a limit cycle. We can see that this limit cycle corresponds to a directed cycle in its transition graph, as illustrated in Figure \ref{fig:n=2cycle}. 

\begin{figure}[ht!]
\includegraphics[width = 4 in]{ThresholdLinear/Figures/n_2_osc.pdf}
\caption{A two neuron, non competitive TLN with a limit cycle.\label{fig:n=2cycle} }
\end{figure}

Additionally, notice that this limit cycle is not confined to the union of the two mixed-sign chambers, $-+$ and $+-$. Instead, the limit cycle visits all four nullcline chambers. Thus, we see that the assumption that networks are competitive is necessary for Theorem \ref{thm:mixed_sign}. 


\section{Local Lyapunov Functions}
Our Proposition \ref{thm:mixed_sign} shows that all trajectories of TLNs approach the mixed sign chamber. In this section, we explore a wider variety of cases when we can prove that all trajectories of a dynamical system approach a smaller region of space. In particular, we introduce \emph{local Lyapunov functions}, a tool for showing all trajectories which are trapped in a region $B$ eventually approach a smaller region $A\subset B$. We begin with a few special cases, proving dynamic consequences of the combinatorial concept of graphical domination, before moving on to the general case. 

\subsection{Domination}

In this section, we review the concept of \emph{domination}, introduced in \cite{curto2019fixed}. While \cite{curto2019fixed} uses domination to establish constraints on fixed points of CTLNs, we show that it constrains dynamic attractors as well. 

\begin{defn}
Let $W$ be the weight matrix of a TLN on $n$ neurons. We say $k$ \emph{strongly dominates} $j$, written $k >_W j$,  if $\wt W_{ki} \geq \wt W_{ji}$ for all $i$.  

If $W$ is the weight matrix of a CTLN with graph $G$, then strong domination is equivalent to the following condition on $G$, termed \emph{graphical domination}: 
$k$ graphically dominates $j$, written $k >_G j$, if the following conditions hold: 
\begin{itemize}
\item For each vertex $i \neq j, k$, if $i\to j$, then $i \to k$. 
\item  $k\not\to j$
\item  $j \to k$
\end{itemize}
\end{defn}  

We also consider a weaker version of domination. 

\begin{defn}
Let $W$ be the weight matrix of a TLN on $n$ neurons. We say $k$ \emph{weakly dominates} $j$ if for all  $i\neq j, k$, $\wt W_{ki} \geq W_{ji}$, and $\wt W_{jk} = \wt W_{kj}$.   

If $W$ is the weight matrix of a CTLN with graph $G$, then weak domination is equivalent to the following condition on $G$, termed \emph{weak graphical domination}:  $k$ weakly graphically dominates $j$ if the following conditions hold

\begin{itemize}
\item For all $i$, if $i\to j$, then $i \to k$. 
\item $k\to j$ if and only if $j \to k$. 
\end{itemize}

\end{defn}  


\begin{defn}
Neurons $j$ and $k$ are \emph{equal input} if $j$ weakly dominates $k$ and $k$ weakly dominates $j$. 
\end{defn}


\begin{ex}
Consider the graph with $V = \{1, 2, 3\}$, $E = \{(1 \to 2), (2\leftrightarrow 3), (3 \to 1)\}$, pictured in Figure \ref{fig:dom_ex}. Then 2 strongly dominates 1, 2 weakly dominates 3, and 1 and 3 have no domination relationship.
\begin{figure}[ht!]
\begin{center}
\includegraphics{ThresholdLinear/Figures/dom_ex.pdf}
\end{center}
\caption{In this graph, 2 strongly dominates 1, 2 weakly dominates 3, and 1 and 3 have no domination relationship. \label{fig:dom_ex}}
\end{figure}
\end{ex}






\subsubsection{Basic results}
We begin with the following observation about strong domination: 
\begin{obs}\label{obs:strong_domination}
Let $k$ strongly dominate $j$,  $\wt W_{ki} \geq \wt W_{ji}$. Then for all $x$ in the positive orthant, 
$$h_k^*(x) - h_j^*(x) = \sum_{i= 1}^n (\wt W_{ki}-\wt W_{ji})x_i \geq 0.$$
\end{obs}

We first see how this shapes the arrangement of nullclines. 

\begin{prop}\label{prop:dom_sep}
If $k$ strongly dominates $j$, then $H_j$ separates $H_k$ from the origin. 
\end{prop}

\begin{proof}
By Observation \ref{obs:strong_domination}, $h_k^*(x) - h_j^*(x) \geq 0$ throughout the positive orthant.
Thus, on the $H_j$ nullcline, where  $h_j^*(x) = 0$, we must have $h_k^*(x)\geq 0$. Therefore, within the positive orthant, $H_j$ is contained on the positive side of $H_k$, thus $H_j$ separates $H_k$ from the origin. 
\end{proof}

Domination has some simple consequences for fixed points. For instance, if any neuron $k$ strongly dominates $j$, $j$ is not contained within any fixed point support. For a more thorough account of how domination constrains fixed points, see  \cite{curto2019fixed}.
We now turn to the easiest constraints on dynamic attractors provided by domination. 


\begin{prop}\label{prop:supersource}
If $i$ is a proper source in $G$, and $i\to j$ for all vertices $j$, then $\lim_{t\to\infty} x_i(t) = 0$. 
\end{prop}

\begin{proof}
Since $i$ is a proper source in $G$, and $i\to j$ for all $j\in [n]$, for any $j \in [n]$, $j$ strongly dominates $i$. Thus, $H_i$ separates all other $H_j$ from the origin. Thus, $H_i$ is the lower boundary of $\cA$. Thus, by Proposition \ref{thm:mixed_sign}, all trajectories approach the negative side of $H_i$. Any trajectory must either eventually cross $H_i$, or approach a fixed point on $H_i$. Since $i$ is proper source, it is not contained in any fixed points, to if a trajectory is approaching a fixed point, $\lim_{t\to\infty} x_i(t) = 0$. Otherwise, once our trajectory crosses $H_i$ at time $T$, for all $t >T$, $x_i' \leq 0$. Thus, since the quantity $x_i$ is monotonic, it approaches a fixed value. Thus, the trajectory must approach the $i^{th}$ nullcline. It cannot approach the interior of the nullcline $H_i$, thus it must approach $E_i$. Therefore, $\lim_{t\to\infty} x_i(t) = 0$.
\end{proof}

\begin{prop}\label{prop:supersink}
If $i$ is a proper sink in $G$, and $j\to i$ for all $j\in [n]$, then $\lim_{t\to\infty} x_i(t) = \theta$ and $\lim_{t\to\infty} x_j(t) = 0$ for all $j\neq i$. 
\end{prop}

\begin{proof}
Since $i$ is a proper sink in $G$ and $i$ receives an edge from every other neuron, $i$ dominates all other neurons $j\in [n]$. Thus, $H_j$ is separated from the origin from each $H_i$. Therefore, $H_i$ forms the outer boundary of $\cA$. Thus, by Proposition \ref{thm:mixed_sign}, all trajectories approach the positive side of $H_i$. Any trajectory must either eventually cross $H_i$, or approach a fixed point on $H_i$. Either way, the value of $x_i$ must approach a fixed value. Since $i$ dominates all other neurons, the only fixed point support of this network is the singleton set $\{i\}$. Thus, in this case $\lim_{t\to\infty} x_i(t) = \theta$ and  $\lim_{t\to\infty} x_j(t) = 0$ for all $j\neq i$. 
 
\end{proof}

 


%%%%%%%%%%%%%%%%%%%%%%%%% Dynamic domination  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Dynamic domination relationships}

While Propositions \ref{prop:supersource} and \ref{prop:supersink} demonstrate that the purely combinatorial property of graphical domination has dynamic consequences, they only apply in extremely restrictive cases. In this next section, we show that domination has further-reaching consequences. We prove several results that show that domination relationships between the neurons $j$ and $k$ have consequences for the relationship between activity levels $x_j(t)$ and $x_k(t)$ over the long run. In order to do this, we must first prove the following lemma about threshold nonlinearities. 
\begin{lem}\label{lem:thresh_ineq}
Let $a \leq 0$. If $a \leq x - y$, then $a \leq [x]_+ - [y]_+$. Further, these inequalities can be made strict: if $b < 0$, $b < x - y$, then $b < [x]_+ - [y]_+$.
\end{lem}
\begin{proof}
We consider four cases:
\begin{itemize}
\item Case 1: $x \geq 0$ and $y \geq 0$. Then 
\begin{align*}
a \leq x- y = [x]_+ - [y]_+\\
b < x- y = [x]_+ - [y]_+
\end{align*}
\item Case 2: $x \geq 0$ and $y < 0$. Then 
\begin{align*}
a \leq 0 \leq [x]_+ = [x]_+ - [y]_+\\
b < 0 \leq [x]_+ = [x]_+ - [y]_+
\end{align*}
\item Case 3: $x < 0$ and $y \geq 0$. Then 
\begin{align*}
a \leq x - y < [x]_+ - [y]_+\\
b < x - y < [x]_+ - [y]_+
\end{align*}
\item 
Case 4: $x < 0$ and $y < 0$. Then 
\begin{align*}
a \leq 0 = [x]_+ - [y]_+\\
b <0 = [x]_+ - [y]_+
\end{align*}
\end{itemize}
\end{proof}
\begin{prop}[Weak domination] \label{prop:weak_dom}
If $k$ weakly dominates $j$, then if $x_k(T) \geq x_j(T)$, then $x_k(t) \geq x_j(t)$ for all $t \geq T$. 
\end{prop}

\begin{proof}
We show that if $k$ weakly dominates $j$, it not possible to cross from the $x_k > x_j$ side of the hyperplane $x_k = x_j$ to the $x_j > x_k$ side. To do this, we show that if 
$x_j = x_k$, then $x_k '- x_j' > 0$. We have 
\begin{align*}
x_k' - x_j' = -x_k + x_j + \left[\sum_{i = 1}^{n} W_{ki}x_i + \theta \right]_+ - \left[\sum_{i = 1}^{n} W_{ji}x_i + \theta \right]_+.
\end{align*}
Since $x_j = x_k$, 
\begin{align*}
x_k' - x_j' = \left[\sum_{i = 1}^{n} W_{ki}x_i + \theta \right]_+ - \left[\sum_{i = 1}^{n} W_{ji}x_i + \theta \right]_+.
\end{align*}
Now, since the threshold nonlinearity if a monotone transformation, 
\begin{align*}
0 \leq \left[\sum_{i = 1}^{n} W_{ki}x_i + \theta \right]_+ - \left[\sum_{i = 1}^{n} W_{ji}x_i + \theta \right]_+ 
\end{align*}
if and only if 
\begin{align*}
0 \leq 
\left(\sum_{i = 1}^{n} W_{ki}x_i + \theta \right) - \left(\sum_{i = 1}^{n} W_{ji}x_i + \theta \right).
\end{align*}
We have 

\begin{align*}
\left(\sum_{i = 1}^{n} W_{ki}x_i + \theta \right) - \left(\sum_{i = 1}^{n} W_{ji}x_i + \theta \right) = 
\sum_{i \neq j, k}^{n} (W_{ki}-W_{ji})x_i  + W_{kj} x_j -  W_{jk}x_k.
\end{align*}
Because $k$ weakly dominates $j$, $(W_{ki}-W_{ji})\geq 0$ for all $i$, so $\sum_{i \neq j, k}^{n} (W_{ki}-W_{ji})x_i \geq 0$. Because $x_j = x_k$ and because $k$ weakly dominates $j$, $W_{kj} x_j = W_{jk}x_k$. 
Thus
\begin{align*}
0\leq\sum_{i \neq j, k}^{n} (W_{ki}-W_{ji})x_i  + W_{kj} x_j -  W_{jk}x_k
\end{align*}
as desired.  
\end{proof}

\begin{cor}[Equal input]\label{cor:equal_input}
If $x_k$ and $x_j$ are equal input, then if $x_k(T) > x_j(T)$, then $x_k(t) > x_k(t)$ for all $t > T$. If $x_k(T) = x_j(T)$, then $x_k(t) = x_k(t)$ for all $t > T$.
\end{cor}

\begin{proof}
If $j$ and $k$ are equal-input, then $j$ weakly dominates $k$ and $k$ weakly dominates $j$. Thus, if  $x_k(T) \geq x_j(T)$, then $x_k(t) \geq x_j(t)$ for all $t > T$. If $x_k(T) = x_j(T)$, then $x_k(T) \geq x_j(T)$ and $x_k(T) \leq x_j(T)$, so by Proposition \ref{prop:weak_dom}, $x_k(t) \geq x_j(t)$ and $x_k(t) \leq x_j(t)$ for all $t \geq T$, so $x_k(t) = x_j(t)$ for all $t \geq T$. 
\end{proof}

 
\begin{prop}[Strong domination]
\label{prop:strong_dom}
If $k$ strongly dominates $j$, then for all $\eta > 0$, there exists some $T_\eta \geq 0$ such that for all $t \geq T_\eta$, $x_k(t) +\eta > x_j(t)$. \end{prop}

\begin{proof}
We prove that if $x_j > x_k$, then $x_k' - x_j' > 0$. By Observation \ref{obs:strong_domination}, we have $h_k^*(x) > h_j^*(x)$ within the positive orthant. 
Now, we apply Lemma \ref{lem:thresh_ineq} to show that this still holds once we apply the threshold nonlinearity: 
\begin{align*}
h_k^*(x)  -h_j^*(x)  &=  -x_k + y_k +  x_j - y_j \geq 0\\
x_k - x_j &\geq  y_k - y_j \\
x_k - x_j &\geq [y_k]_+ - [y_j]_+\\
x_k' - x_j'&\geq 0
\end{align*}
whenever $x_j  \geq x_k$. Further, this inequality can be made strict whenever $x_j > x_k$, since in this case, we must have $h_k^*(x)  -h_j^*(x) > 0$. 


Now, we use this to prove the desired result. First, suppose that the trajectory starting at the point $x(0)$ has $x_k(T) \geq  x_j(T)$ at some time $T$. Then by Proposition \ref{prop:weak_dom} $x_k(t) \geq  x_j(t)$ for all time $t \geq T$. Thus, we can take $T_\eta= T$ for all $\eta > 0$. 

Now, suppose this does not happen, and that $x_k(t) <  x_j(t)$ for all $t \geq 0$. Then $x_k'(t) - x_j'(t) > 0$ for all $t\geq 0$. Thus, the quantity $x_k(t)-x_j(t)$ is monotonically increasing, and must thus approach a limit. This limit must be $x_k(t)-x_j(t) = 0$, since when $x_k(t) < x_j(t)$, $\xdot_k(t) -\xdot_j(t) >0$. Thus for all $\eta > 0$, there exists some $T_\eta \geq 0$ such that for all $t \geq T_\eta$, $x_k(t) +\eta > x_j(t)$.
\end{proof}


\subsection{General Local Lyapunov Functions}

The main idea in our proof of Proposition \ref{prop:strong_dom} is an example of something we will call a \emph{local Lyapunov function}. 
Lyapunov functions are typically used to show that all trajectories of a dynamical system approach a specified fixed point, conventionally taken to be the origin. Here, we generalize this style of argument by introducing local Lyapunov-like functions. We will use these to show that all trajectories which enter a region $B$ approach a smaller region $A$, as illustrated in Figure \ref{fig:llf}. 


\begin{figure}[ht!]
\begin{center}
\includegraphics[width = 2.5 in]{ThresholdLinear/Figures/local_lyapunov.pdf}
\end{center}
\caption{If $L$ is a local Lyapunov function for $A$ and $B$, then all trajectories which enter $B$ must approach $A$. \label{fig:llf}}
\end{figure}
 
\begin{defn}Let $A\subseteq B\subseteq \R^n$ be compact sets, and $\xdot = g(x)$ be a dynamical system on $\R^n$.  A continuous,continuously differentiable function $L: B \to \R$ is a \emph{local Lyapunov-like function} for the pair $A, B$ if it satisfies the following: 
\begin{enumerate}
\item  $\dot{L} < 0$ on $B\setminus A$.
\item $L > 0$ on $B\setminus A$.  
\item $L\leq 0$ on $A$. 
 \end{enumerate} 
\end{defn}

For instance, our proof of Proposition \ref{prop:strong_dom} established that the $L(x) = x_j - x_k$ is a local Lyupanov function for $B = \cA$, $A = \cA \cap \{ x \mid x_k \geq x_j\}$. 

\begin{lem}
If $L$ is a local Lyapunov-like function for $A,B$, then any trajectory which remains in $B$ for all time approaches $A$. 
\end{lem}

\begin{proof}
Let $x_0\in B$. By assumption, the trajectory $x(t)$ with this  initial condition remains in $B$ for all $t\geq 0$. Now, suppose $x(t)$ does not ever enter $A$. Then $\dot L < 0$ for all time. This means that the value $L(x(t))$ is monotonically decreasing, so it must approach a limit as $t\to \infty$. This means that $\dot L(x(t)) \to 0$ as $t\to \infty$. Since the only place within $B$ where it is possible that $\dot L = 0$ is $A$, the trajectory must approach $A$. 

Now, suppose the trajectory enters $A$. We show that it must stay there. Since $\dot L  < 0$ on $B\setminus A$, by continuity of $\dot L $ we have $\dot L \leq 0$ on $\partial A$. Thus, if the trajectory were to cross out of $A$, the value of $L$ must decrease as we cross out. However, since $L \leq 0$ on $A$ and $L > 0$ on $B$, this is not possible. 
\end{proof}

\section{Main results: CTLNs}

In this section, we work towards a proof of the following result, which has Theorems \ref{thm:dag} and \ref{thm:dag_onto_symmetric} as consequences. 


\begin{thm}
\label{thm:sources_die}
Let $G$ be a graph in which every vertex is reachable from a source. Then there is a source $j$ in $G$ such that $\lim_{t\to \infty} x_j(t) = 0$. 
\end{thm}

We begin by giving an informal summary of our argument. 
First, we prove that if $j$ is a source, and if $x_j \leq x_k$ for all other neurons $k$, then $\lim_{t\to \infty} x_j = 0$ (Lemma \ref{lem:smallest_sources_die}). We do this by showing that  within this set, the nullcline $H_j$ forms the lower boundary of the mixed-sign chamber (Figure \ref{fig:sources_die_arg} A), thus trajectories are trapped on the negative side of $H_j$. Thus once trajectories are trapped in this region, $\lim_{t\to  \infty}x_j$. 

\begin{figure}
\includegraphics{ThresholdLinear/Figures/sources_die_arg.pdf}
\caption{A) Within the region where the source numbered 1 is the smallest, the nullcline $H_1$ separates the other nullclines from the origin. B) We number our neurons along paths from the smallest source. C) The regions $\Omega_{1\ell}$ and $\Omega_{13}$. D) Our local Lyapunov functions.  \label{fig:sources_die_arg}}
\end{figure}

Next, we show that this condition is eventually satisfied for the smallest source: the source $j$ which has the $x_j \leq x_\ell$ for all other sources $\ell$ at our initial condition.
We show this using local Lyapunov functions for a nested sequence of sets $\Omega^{G}_1\supseteq \Omega^G_{2}\supseteq \cdots \supseteq\Omega^G_{n}$. These sets are defined by renumbering the neurons along paths from the source (Figure \ref{fig:sources_die_arg} B), and then requiring the activity of the source to be lower than that of other neurons along this path (Figure \ref{fig:sources_die_arg} C). Finally, we show that the function $L_\ell = x_j - x_\ell$ is a local Lyapunov function for the sets $A = \Omega^{G}_\ell$ and 
 $B =\Omega^{G}_{\ell -1}$. This means that trajectories get in $\Omega^{G}_{\ell -1}$ go towards $ \Omega^{G}_\ell$. Thus, trajectories must eventually enter the set where $x_j \leq x_{\ell}$ for all vertices $\ell$ reachable from $j$. 
This must also happen for every other source $i$. Thus, since $x_j$ is the smallest source, we must eventually have $x_j\leq x_i \leq x_\ell$ if $\ell$ is reachable from some other source $i$. Therefore, we must eventually enter the set where $x_j\leq x_\ell$ for all other neurons $\ell$. Thus, by Lemma \ref{lem:smallest_sources_die}, $\lim_{t\to \infty} x_j = 0$. 
Finally, the value of $x_j$ must become so low that its influence on the other neurons may be neglected. Thus, we let some other source take over as the smallest source. In this way, we show that the activity of all sources must decay to zero. 

In order to apply this result inductively in order to prove Theorems \ref{thm:dag} and \ref{thm:dag_onto_symmetric}, we wish to eventually neglect the activity of sources which have ``died". Thus, we will need to prove our results in a way which has some threshold for negligible activity which we allow ourselves to neglect. When we are proving Theorems \ref{thm:dag} and \ref{thm:dag_onto_symmetric} by induction, we will modify our graph by ignoring neurons whose activity is approaching zero. We will also need to deal with the fact that, if we have a local Lyapunov function for $A$ and $B$, this only guarantees that trajectories which remain in $B$ \emph{approach} $A$, not that they actually enter it. We handle both of these issues through our definition of $\Omega^{G}_\ell(\alpha, \beta)$. 

\begin{defn}\label{def:order_omega}
Let $G$ be a graph with vertices $V_G$. Let $L\subseteq V_G$.  Let $j$  be a particular source in $G|_L$.  Renumber the vertices in $L$ as follows: 
First, partially order the vertices by $k \leq_j \ell$ if the shortest path from $j$ to $k$ is shorter than the shortest path from $j$ to $\ell$, setting this length to be $\infty$ if $\ell$ is not reachable from $j$. Then, pick a linear extension of this order. Notice that under this order, we have labeled $j = 1$. Now, we can define
\begin{align*}
\Omega^{G_L}_\ell  &= \{x \mid x_j \leq x_k \mbox{ for all } k \leq \ell, k\in L, x_k = 0 \mbox{ for all } k \notin L\}\\
\Omega^{G_L}_\ell (\alpha, \beta) & = \{x \mid x_j \leq x_k + \alpha \mbox{ for all } k \leq \ell, k\in L, x_k \leq \beta, |\xdot_k|\leq \beta \mbox{ for all } k \notin L\}
\end{align*}
When $L = V_G$, we drop the parameter $\beta$, writing 
\begin{align*}
\Omega^{G_L}_\ell (\alpha) & = \{x \mid x_j \leq x_k + \alpha \mbox{ for all } k \leq \ell\}.
\end{align*}
\end{defn}

Notice that $\Omega^{G_L}_{|L|}$ is the set where the source numbered 1 has $x_1 \leq x_\ell$ for all $\ell \in L$, and $x_\ell = 0$ for all $\ell \notin L$. Our first lemma establishes that ``smallest sources die": if a trajectory stays in the set $\Omega^{G_L}_{|L|}$ where the source 1 is the neuron with lowest activity, then $x_1$ approaches zero. We prove a stronger result, that this holds on $ \Omega^{G_L}_{|L|}(\eta, \zeta)$ for some positive values of $\eta$ and $\zeta$.
 
\begin{lem}\label{lem:smallest_sources_die}
Let $L \subseteq V_G$ be our set of active neurons. Assume the neurons are numbered according to Definition \ref{def:order_omega} such that neuron 1 is a source in $G|_L$. Then there exist $\eta, \zeta > 0$ such that if $x \in \Omega^{G_L}_{|L|}(\eta, \zeta)$ for all $t \geq T$, then $\lim_{t\to \infty} x_1(t)= 0$. 
\end{lem}

%To motivate this claim, we first sketch the proof of an easier version with $\eta = 0$. Then we have $x_j \leq x_k$ for all $k$. By Proposition \ref{prop:weak_dom}, once $x_j \leq x_k$ at some time $T$,  $x_j \leq x_k$ for all $t > T$. Further, within the region where  $x_j \leq x_k$, the hyperplane $H_j$ forms the lower boundary of the mixed-sign chamber, separating all other hyperplanes $H_j$ from the origin. Thus, the entire mixed-sign chamber is contained on the negative side of $H_j$, so the value of $x_j$ must approach zero. Much of the work in the next proof goes into showing this argument can also be made to work for a positive $\eta > 0$. 

\begin{proof}

We first describe the value of $\eta$ and $\zeta$. If $1$ is a proper source, there are no fixed points on the set $ C := H_1\cap \R^n_\geq$, so $||\xdot||_1> 0$ on $H_1 \cap \R^n_\geq$. If $1$ is an isolated vertex, then the only fixed point $x^*$ on $H_1$ has support $\{1\}$, and therefore is separated from $\Omega^{G_L}_{|L|}$ by a positive distance $d$. Thus, $||\xdot||_1> 0$ on the compact set  $C := H_1\cap \R^n_\geq \setminus B_d(x^*)$ we get by deleting a $d$-neighborhood of this fixed point $x^*$.  Thus the continuous function $||\xdot||_1$ attains its minimum value on $C$. Therefore there exists some positive $\alpha > 0$ such that  $||\xdot||_1 \geq \alpha > 0$ on $C$. Let $\eta  = \frac{\alpha}{4n\delta }$. Let $\zeta = \delta \eta$. 

We first focus on the neurons in $L$ and show that if $x_1(T) < x_k(T) +\eta $ for some $T$, then $x_1'(t) \leq 0$ for all $t \geq T$. Thus $\lim_{t\to \infty}x_1(t) = 0$. For all $k$ such that $1\not \to k$,
\begin{align*}
h_k^*(x(t)) - h_1^*(x(t)) &= -x_k + x_1 +  (-1-\delta)x_1 - (-1-\delta)x_k + \sum_{i\neq 1, k} (W_{ki} - W_{1i})x_i  \\
h_k^*(x(t)) - h_1^*(x(t)) &= \delta(x_k - x_1) + \sum_{i\neq 1, k} (W_{ki} - W_{1i})x_i \\
h_k^*(x(t)) - h_1^*(x(t)) &\geq -\delta \eta. 
\end{align*}
Now, for $x(t)\in H_1 \cap \R^n_\geq$, $h_1^*(x(t)) = x_1'(t) = 0$. For all $x(t)$, $h_k^*(x(t)) \leq \xdot_k(t)$. Therefore, for $x(t)\in H_1 \cap \R^n_\geq$,
\begin{align*}
x_k'(t)  &\geq -\delta \eta. 
\end{align*}
If $1 \to k$, then the entirety of $H_1 \cap \R^n_\geq$ is contained on the positive side of $H_k$, so on $H_1 \cap \R^n_\geq$, 
\begin{align*}
\xdot_k(t)  \geq 0 \geq -\delta \eta\\ 
\xdot_k(t) \geq -\delta \eta. 
\end{align*}
Now, we note that this is also satisfied  by requirement for  the neurons outside $L$. 

Now, we show that it is only possible to cross the $H_1$ hyperplane from the positive to the negative side. We do this by showing that the dot product of $ \xdot(t)$ with the normal vector to $H_1$ is always negative. 
We have 
\begin{align*}
\sum_{i = 1}^n \xdot_i(t) = \sum_{x_i(t)\geq 0}\xdot_i(t) + \sum_{\xdot_i(t)< 0}\xdot_i(t) = \sum_{i = 1}^n | \xdot_i(t)| + 2 \sum_{x_i(t)< 0}\xdot_i(t) = ||\xdot(t)||_1+ 2 \sum_{x_i(t)< 0}\xdot_i(t).
\end{align*}
Since $\xdot_k(t)   \geq -\delta \varepsilon$ for all $k$,
\begin{align*}
2 \sum_{x_i(t)< 0}\xdot_i(t) \geq -2n\delta\varepsilon = -2n\delta \frac{\alpha}{4n\delta} = -\frac{\alpha}{2}.\\
\end{align*}

Thus 
\begin{align*}
\sum_{i = 1}^n \xdot_i = ||\xdot||_1+ 2 \sum_{x_i< 0}\xdot_i \geq \frac{\alpha}{2}  > 0.
\end{align*}
Now, recall that the normal vector to $H_i$ is $(-1, -1-\delta,-1-\delta, \ldots,  -1-\delta)$.  Thus, since $\xdot_1 = 0$ on $H_1\cap \R^n_\geq$, 
\begin{align*}
\xdot(t)\cdot h_1 = (-1-\delta)\sum_{i = 1}^n \xdot_i(t) < 0. 
\end{align*}
Thus, trajectories can only cross from the positive side to the negative side of $H_1$. Thus, the value of $x_1(t)$ eventually becomes monotone, and thus must approach a limit. This means the trajectory must approach the $x_1$ nullcline. The trajectory cannot approach $H_1$ because if $c\in  H_1$, $\xdot(t)\cdot h_1< 0$. Thus, the trajectory must approach $E_1$, so  $\lim_{t\to \infty}x_1(t) = 0$.

\end{proof}

Now, we show that the conditions of Lemma \ref{lem:smallest_sources_die} are ultimately achieved for some source, i.e.  for some source, $ \Omega^{G_L}_{|L|}$ is an attracting set. In particular, we show this for the smallest source, i.e. the source neuron $j$ such that $x_j \leq x_\ell$ for all other \emph{sources} $\ell$. 
We will prove by induction using this order that if $k$ is reachable along a path from a source $j$, then eventually $x_j  < x_k  + \eta$. We do this using local Lyapunov functions for a nested sequence of sets. 


\begin{lem}\label{lem:lyapunov} For any $\beta > 0$, the function $L_\ell = x_j - x_{\ell} + \beta$ is a local Lyapunov function for 
$B = \Omega^{G_L}_{\ell}(\beta, \zeta)$ and  $A =\Omega^{G_L}_{\ell-1}(\alpha, \zeta)\cap B$ for $\beta = \frac{ \alpha\epsilon}{2(\epsilon + \delta)}$ and $\zeta = \frac{\epsilon \alpha}{2n(\epsilon + \delta)}$. 
\end{lem}

\begin{proof}
By construction, we have $ L_\ell \leq 0$ on $A$ and $L_\ell > 0$ on $B \setminus A$.  
Now, we show that $\dot L_\ell <0$ on $B\setminus A$. 
We consider 
\begin{align*}
\dot L_\ell = \xdot_j - \xdot_\ell = -x_j + x_\ell + \left[\sum_{i=1}^n W_{ji}x_i + \theta \right]_+ - \left[\sum_{i=1}^n W_{\ell i}x_i + \theta\right]_+. 
\end{align*}
By Lemma \ref{lem:thresh_ineq}, when $x_j \geq x_k$
\begin{align*}
\xdot_j - \xdot_\ell &\leq -x_j + x_\ell + \left( \sum_{i=1}^n W_{ji}x_i + \theta\right)  - \left(\sum_{i=1}^n W_{\ell i}x_i + \theta \right)_+\\
\xdot_j - \xdot_\ell &\leq -x_j + x_\ell + \sum_{i=1}^n (W_{ji}-W_{\ell i})x_i \\
\xdot_j - \xdot_\ell &\leq (-1 - W_{\ell j})x_j + (1 + W_{j\ell})x_\ell + \sum_{i \in L\setminus \{j, \ell\}  }(W_{ji}-W_{\ell i})x_i + \sum_{k \notin L }(W_{ji}-W_{\ell i})x_k
\end{align*}
Now, since $j$ is source in $G|_L$, $(W_{ji}-W_{\ell i}) \leq 0$ for each neuron $i \in L\setminus \{j, \ell\} $. 
 Further, $1 + W_{j\ell} = -\delta \leq 0$.  
 Since $x\in B$, the total activity of the neurons outside $L$ is bounded above, thus $ \sum_{k \notin L }(W_{ji}-W_{\ell i})x_k \leq  2n(\epsilon + \delta) \frac{\epsilon \alpha}{2n(\epsilon +\delta)} = \frac{\epsilon \alpha}{2}$.  
 
Now, we consider two cases, if $\ell$ recieves an edge directly from $j$ or not. In the fist case,  then  $(-1 - W_{\ell j})  = -\epsilon <0$, so 
$$\xdot_j - \xdot_\ell \leq -\epsilon x_j + \frac{\epsilon\alpha}{2}.$$
Since $x_j \geq \alpha$ in $B\setminus A$, we have 
 $\xdot_j - \xdot_\ell \leq 0$ whenever $x_j \geq x_k$, thus $\dot L < 0$ on $B\setminus A$. 

Next, if $\ell$ does not receive an edge directly from $j$, by our ordering of neurons, we have that $\ell$ does receive an edge from some neuron $k < \ell$. For $x\in B$, we have $x_j \leq x_k + \beta$. We pull the $k^{th}$ term out of the summation in the right hand side, 
rewriting it as 
\begin{align*}
\xdot_j - \xdot_\ell &\leq (-1 - W_{\ell j})x_j + (1 + W_{j\ell})x_\ell + (W_{jk} - W_{\ell k})x_k  + \sum_{i\neq j, k,\ell \in L}(W_{ji}-W_{\ell i})x_i + \frac{\epsilon\alpha}{2}\\
\xdot_j - \xdot_\ell &\leq \delta x_j - \delta x_\ell  - (\delta + \epsilon)x_k  +\sum_{i\neq j, k,\ell \in L}(W_{ji}-W_{\ell i})x_i + \frac{\epsilon\alpha}{2}\\
\end{align*}
We can drop the terms $ - \delta x_\ell$ and $\sum_{i\neq j, k,\ell \in L}(W_{ji}-W_{\ell i})x_i$, as they are guaranteed to be non-positive, obtaining the bound 
\begin{align*}
\xdot_j - \xdot_\ell &\leq \delta x_j  - (\delta + \epsilon)x_k + \frac{\epsilon\alpha}{2}.
\end{align*}
Now, for $x\in B$, we have $x_j \leq x_k + \beta$, so 
\begin{align*}
\xdot_j - \xdot_\ell &\leq \delta x_j  - (\delta + \epsilon)(x_j - \beta)+ \frac{\epsilon\alpha}{2}\\
\xdot_j - \xdot_\ell &\leq -\epsilon x_j  + (\delta + \epsilon)\beta + \frac{\epsilon\alpha}{2}.
\end{align*}
Now, for all $x\notin A$, we have $x_j \geq x_k + \alpha \geq \alpha$, thus-
\begin{align*}
\xdot_j - \xdot_\ell &\leq -\epsilon \alpha + (\delta + \epsilon)\beta + \frac{\epsilon\alpha}{2}= 0,
\end{align*}
as desired. 
\end{proof}



\begin{lem}\label{lem:source_becomes_smallest_1}
Let $L \subseteq V_G$ be our set of active neurons,  numbered according to Definition \ref{def:order_omega} such that neuron 1 is a source in $G|_L$. Let $\ell$ be a vertex which is reachable from $1$ along a directed path. Then for each $\eta \geq 0$, there exists some  $T \geq 0$ and some $\zeta> 0$ such that if $x_k(t), |\xdot_k(t)| \leq \zeta$ for all  time $t$ and all inactive neurons $k\notin L$ such that $x(t) \in \Omega_\ell^{G|_L}(\eta, \zeta)$ for all $t \geq T$. 
\end{lem}

\begin{proof}
We prove this by induction, with the vertices labeled according to Definition \ref{def:order_omega}. If $\ell = 1$ this result is trivially true. 

Now, we assume as an inductive hypothesis that this result holds for all vertices $k < \ell$, and show that it must hold for $\ell$.  Then by Lemma \ref{lem:lyapunov}, we have that there is a local Lyapunov function $L$ for $B = \Omega_{\ell-1}^{G|_L}(\eta/2, \zeta)$ and  $A =\Omega_\ell^{G|_L}(\beta, \zeta)\cap B$ for $\beta = \frac{ \eta\epsilon}{2(\epsilon + \delta)}.$ Now, by the inductive hypothesis, there exists a time $T'$ such that $x(t) \in B$ for all $t \geq T'$. Thus, all trajectories must enter and remain in $B$, so they approach $A$. Thus, after some time $T$ all trajectories must actually enter and become trapped in the set  $\Omega_\ell^{G|_L}(\eta, \zeta)$. 
\end{proof}

Now, we have shown that each source eventually becomes (approximately) smaller than all vertices which are reachable from it. However, to apply Lemma \ref{lem:smallest_sources_die}, we need to show the source eventually becomes  (approximately) smaller than \emph{all} active neurons. 

\begin{lem}\label{lem:smallest_source_becomes_smallest}
Let $L \subseteq V_G$ be our set of active neurons,  numbered according to Definition \ref{def:order_omega} such that neuron 1 is a source in $G|_L$. Suppose $x_1(0) < x_k(0)$ for all other sources $k$ in $G|_L$. Then for each $\eta \geq 0$, there exists $\zeta> 0$ such that if $x_j \leq \zeta$ for all $j\notin L$ and $T \geq 0$ such that $x(t) \in \Omega_\ell^{G|_L}(\eta, \zeta)$ for all $\ell \in L$, $t \geq T$. 
\end{lem}

\begin{proof}
By assumption, every vertex $\ell$ is reachable from some source $k$ along a directed path.  Thus by numbering the vertices according to Definition  \ref{def:order_omega} such that $k$ is sent to $1$, we can apply Lemma  \ref{lem:source_becomes_smallest_1}, to show that exists a time $T_{k\ell}$ such that $x_k \leq x_\ell + \eta$ for all $t\geq T_{k\ell}$. Now, since  $x_1(0) < x_k(0)$ for all other sources $k$, there is some $\zeta$ such that if  $x_j \leq \zeta$ for all $j\notin L$, the order of $x_1$ and $x_k$ cannot switch, thus $x_1$ will remain smaller than $x_k$ for all other sources $k$. Thus, by taking $T \geq T_{k\ell}$ for each vertex $\ell$ and source $k$, we have that 
$x_j \leq x_j \leq x_\ell + \eta$  for each vertex $\ell$. Thus, for  $t \geq T$, we have  $x(t) \in \Omega_\ell^{G|_L}(\eta, \zeta)$, as desired. 
\end{proof}

Finally, we are ready to prove Theorem \ref{thm:sources_die}. 

\begin{proof}
Let $G$ be a graph for which every vertex is reachable from a source, and consider a CTLN with graph $G$. Let $j$ be the source in $G$ which satisfies $x_j \leq x_k$ for all other sources  at the initial condition. By Lemma \ref{lem:smallest_source_becomes_smallest}, there exists a time $T$ such that $x\in \Omega_\ell^{G}(\eta)$ for all neurons $\ell$ and the values of $\eta$ an used in Lemma \ref{lem:smallest_sources_die}. Therefore, $\lim_{t\to\infty} x_{j} = 0$. 
\end{proof}

Now, we use this result to prove Theorems \ref{thm:dag} and \ref{thm:dag_onto_symmetric}. The first part of our proof is to show that, in the case of a DAG, all neurons other than the sinks have their activity approach zero, and in the case of a symmetric graph, all neurons outside the symmetric part have their activity approach zero. We prove this for a more general family of graphs, which we define below. 

\begin{defn} 
Let $G$ be a graph and $\omega, \tau \subseteq V_G$. We say that $(\omega, \tau)$ is an \emph{inductively stable DAG decomposition} of $G$ if  $\omega \sqcup \tau$ is a partition of the vertices of $G$ satisfying the following inductive definition  
\begin{enumerate}
\item $G|_\omega$ is a DAG
\item $G|_\tau$ contains all sinks of $G$ 
\item there are no edges from $\tau$ back to $\omega$ 
\item every vertex of $\tau$ is reachable along a directed path from a vertex in $\omega$. 
\item for any source $i\in \omega$, $\omega \setminus \{i\}, \tau$ is an inductively stable DAG decomposition of $G|_{V_G\setminus \{i\}}$. 
\end{enumerate}
\end{defn}

\begin{lem}\label{lem:dag_decomp}
Let $G$ be a graph with inductively stable DAG decomposition $( \omega, \tau)$. Then for any $i\in \omega$, $\lim_{t\to \infty}x_i = 0$. 
\end{lem}


\begin{proof}

Let $G$ be a graph with inductively stable DAG decomposition $( \omega, \tau)$. We first prove that every vertex of $G$ is reachable from a source. First, if $i\in \omega$, then a path which follows edges backwards must remain in $\omega$, and must eventually terminate, since $G_\omega$ is a DAG. The vertex where this path terminates must be a source.  Now, by assumption, every vertex in $\tau$ is reachable along a path from a vetex in $\omega$. Thus, from a vertex in $\omega$, we can trace a path backwards into $\tau$, and then back to a source. 

Now, by Theorem \ref{thm:sources_die}, there is some source $i$ of $G$ whose activity must approach zero. Further, for this to be possible, all trajectories of the TLN must approach the $i^{th}$ nullcline. 
Thus we are guaranteed that for each value of $\zeta$, there exists a time $T$ such $x_i(t)\leq \zeta$, and $|\xdot_i(t)| \leq \zeta$ for all $t \geq T$. 
Now, by assumption, $\omega\setminus\{i\}, \tau$ is an inductively stable DAG decomposition of $G|_{V_G\setminus i}$.  
By choosing $\zeta$ small enough, we can satisfy the conditions of Lemmas \ref{lem:smallest_sources_die} and \ref{lem:lyapunov} when restricting to the graph  $G|_{V_G\setminus i}$. 
We can apply this argument inductively to show that for each $i\in \omega$, $\zeta > 0$, there is a time $T$ such that $x_i(t) \leq \zeta$ for all $t\geq T$. Thus, for any $i\in \omega$, $\lim_{t\to \infty}x_i = 0$. 
\end{proof}

Thus, we have shown that whenever $G$ has an inductively stable DAG decomposition $\omega$, $\tau$, all activity of the CTLN on $G$ becomes concentrated on $G|_\tau$. Now, we wish to prove that if $G_|\tau$ is symmetric, then all trajectories of the $CTLN$ on $G$ approach a fixed point. 
In order to prove this, we first prove the following lemma, which allows us to neglect the impact of neurons in $\omega$ upon those of $\tau$ once they have decayed sufficiently. 

\begin{lem}\label{lem:lyapunov_hell}
Let $\xdot = g(x)$ be a dynamical system on a compact set $A$ with a Lyapunov like function $L: A \to \R$ satisfying the following: 

\begin{itemize}
\item $\dot L \leq 0$ for all $x\in A$ 
\item $\dot L = 0$ only on a finite set of fixed points $X = \{x\in A\mid g(x) = 0\}$, 
\item $L$ is bounded below on $A$.  
\end{itemize}

Then for every $\epsilon > 0$, there exists $\delta > 0$ such that if $\dot x = g'(x, t)$ is a dynamical system satisfying $|g(x) - g'(x, t)| < \delta$, then there exists $T$ such that all trajectories of of the system $\dot x = g'(x, t)$ satisfy $|x(t) - X| < \epsilon$ for all $t > T.$


\end{lem}

\begin{figure}
\includegraphics[width = 6 in]{ThresholdLinear/Figures/Lyapunov_horror.pdf}
\caption{(a) The quantity $D(\delta)$. (b) The quantity $\epsilon'(\delta)$. (c) The quantity $E(\delta, x)$.  \label{fig:lyapunov}}
\end{figure}

\begin{proof}
We consider three quantities, $D(\delta)$, $\epsilon'(\delta)$,and $E(\delta)$. First, $D(\delta)$ gives the maximum value of $\int_{t_1}^{t_2} \nabla L(x(t)) \cdot g'(x(t),t)dt$ can assume along trajectories of the system $\xdot = g'(x, t)$  which begin and end in an $\epsilon/2$ neighborhood of $X$, but leave an $\epsilon$ neighborhood of $X$ along the way. We show that $D(\delta)$ approaches a negative limit as $\delta \to 0$. Notice that  
\begin{align*}\int_{t_1}^{t_2} \nabla L(x(t)) \cdot g'(x(t),t)dt \leq (t_2 - t_1)  \max_{x \in A, d(x, X) \geq \epsilon/2} (\nabla L(x(t)) \cdot g(x(t),t)).
\end{align*}
Now, since $\nabla L(x) \cdot g'(x,t)$ attains its negative maximum value $\alpha < 0$ on the compact set $\{x \in A\mid d(x, X) \geq \epsilon\}$ , and  $g'(x, t) \to g(x)$ as $ \delta\to 0$, we must have that  $\max_{x \in A, d(x, X) \geq \epsilon/2} (\nabla L(x) \cdot g'(x,t)) \to \alpha < 0$ as $\delta \to 0$.  Further, any trajectory which begins in an $\epsilon/2$ neighborhood of $X$, leaves an $\epsilon$ neighborhood of $X$, and returns to an  an $\epsilon/2$ neighborhood of $X$ must have length at least $\epsilon$, provided we have chosen $\epsilon$ small enough that all fixed points in $X$ are separated by a distance of at most $\epsilon$.  

Finally, since $g(x)$ is bounded above, so is $g'(x, t)$. Thus for a trajectory of length $\epsilon$, we must have $t_2 - t_1 \geq \epsilon / \max_{x\in A}(|g'(x,t)|)$. This must approach the positive limit $t_2 - t_1 \geq \epsilon / \max_{x\in A}(|g(x)|)$ as $\delta\to 0$. Thus, the product $(t_2 - t_1)  \max_{x \in A, d(x, X) \geq \epsilon/2} (\nabla L(x) \cdot g'(x,t))$ approaches a negative limit at $\delta \to 0$. Thus, so does $D(\delta)$. 

Now, we consider $\epsilon'(\delta)$, which we define as the maximum value of $\epsilon$ such that $ \nabla L(x) \cdot g'(x,t) < 0$ for all $x$ such that $|x - X| \geq \epsilon'$. Again, we have that $\epsilon' \to 0$ as $\delta \to 0$, since $ \nabla L(x) \cdot g'(x,t)\to \nabla L(x) \cdot g(x)$, and  $\nabla L(x) \cdot g(x) < 0$ for all $x\notin X$. Finally, we define 
\begin{align*}E(\delta, x):=\max_{y \in B_{\epsilon'(\delta)}(x)} L(y) - \min_{z \in B_{\epsilon'(\delta)}(x)}  L(z) 
\end{align*}
 Notice that  as $\delta \to 0$, $E(\delta, x) \to 0$ by continuity of $L$. Now, let $$E(\delta) := \max_{x \in X} E(\delta, x).$$ Since we are taking this maximum over a finite set, we also have that $E(\delta) \to 0$ as $\delta \to 0$. 
 
Thus, for $\delta$ small enough, we have $|E(\delta)| < |D(\delta)|$. When this is achieved, we claim that it is impossible for a trajectory to start within $B_{\epsilon'}(X)$, leave  $B_{\epsilon}(X)$, and return to $B_{\epsilon'}(X)$. We choose $\delta$ such that $\epsilon' < \epsilon/2$. Then along any trajectory starts from and returns from  $B_{\epsilon'}(X)$, the value of $L$ must decrease along the trajectory by at least $D(\delta)$. However, since the most the value of $L$ can change within $B_{\epsilon'}(x)$ is $E(\delta) < D(\delta)$, this is not possible. 

Finally, we show that this means that there exists $T$ such that all trajectories of of the system $\dot x = g'(x, t)$ satisfy $|x(t) - X| < \epsilon$ for all $t > T.$ By our definition of $\epsilon'(\delta)$, we have that $ \nabla L(x) \cdot g'(x,t) < 0$ outside of $B_{\epsilon'}(X)$. Thus, since $L$ is bounded below, all trajectories must visit the set $B_{\epsilon'}(X)$. Now, for each particular fixed point $x^*\in X$, it is not possible for a trajectory to leave the set $B_\epsilon(x^*)$ and return to $B_{\epsilon'}(x^*)$. Thus, since there are only finitely many fixed points $x^*$, our trajectory must eventually get stuck in  $B_\epsilon(x^*)$ for one of them. 


\end{proof}



\begin{proof}[Proof of Theorem \ref{thm:dag}]
Let $G$ be a DAG. Let $\tau$ be the set of all sinks of $G$, and $\omega$ be $V_G\setminus\tau$. Notice that this is an inductively stable DAG decomposition of $G$. Then by Lemma \ref{lem:dag_decomp}, $\lim_{t\to \infty}x_i(t) = 0$ for all $i\in \omega$. 
Now, since $G|_\tau$ is symmetric, it has  a Lyapunov-like function $L$ by \cite{hahnloser2000permitted}. 
Therefore, by considering the effect of $x_i, i\in \omega$ as a time varying external input on $x_j, j\in \tau$, by our Lemma \ref{lem:lyapunov_hell}, for each $\eta > 0$, we can find a time $T'$ such that $\{x_j\}_{j\in \tau}$  is contained within an $\eta$ neighborhood of a fixed point of the CTLN defined by $G|_\tau$. 
Thus, as $T\to \infty$, the trajectory approaches a fixed point whose support is contained within $\tau$. 
\end{proof}


\begin{proof}[Proof of Theorem \ref{thm:dag_onto_symmetric}]
Let $G$ be a graph and $\omega, \tau$ a partition of the vertices of $G$ such that $G|_\tau$ is symmetric and connected, $G|_\omega$ is a DAG, and there are no edges from $\tau$ to $\omega$. Then by Lemma \ref{lem:dag_decomp}, $\lim_{t\to \infty}x_i(t) = 0$ for all $i\in \omega$. 
Now, since $G|_\tau$ is symmetric, it has  a Lyapunov-like function $L$ by \cite{hahnloser2000permitted}. 
Therefore, by considering the effect of $x_i, i\in \omega$ as a time varying external input on $x_j, j\in \tau$, by our Lemma \ref{lem:lyapunov_hell}, for each $\eta > 0$, we can find a time $T'$ such that $\{x_j\}_{j\in \tau}$  is contained within an $\eta$ neighborhood of a fixed point of the CTLN defined by $G|_\tau$. 
Thus, as $T\to \infty$, the trajectory approaches a fixed point whose support is contained within $\tau$. 
\end{proof}









\section{Main results: competitive TLNs}
In \cite{curto2019robust}, Curto, Langdon, and Morrison relax the strict CTLN conditions, and investigate how and when the graph $G_W$ constrains the dynamics of a competitive TLN. In particular, they say that a graph $G$ is a \emph{robust motif} if $G$ fully determines $FP(W)$ for all weight matrices $W$ such that $G_W = G$. Their Theorem 1.6 gives a complete characterization of which graphs $G$ are robust motifs. 

\begin{thm}[Theorem 1.6, \cite{curto2019robust}]
 $G$ is a robust motif if and only if one of the following holds:
 \begin{enumerate}
\item $G$ belongs to one of the infinite families DAG1 or DAG2, or
\item  $G$ is one of the four invariant permitted motifs (the singleton, the 2-clique, the independent set of size 2, or the 3-cycle).
\end{enumerate}
\end{thm}

In particular, TLNs in the infinite families DAG1 and DAG2 each have a single fixed point, which is stable. However, the fixed point structure of a dynamical system does not fully determine its activity: in principle, a dynamical system with a unique fixed point which is stable may also have a limit cycle or a chaotic attractor. Thus, we would like to show that the families DAG1 and DAG2 are robust in the following sense:

\begin{conj}\label{conj:dyn_robust}
Let $(W, \theta)$ define a TLN such that $G_W$ is a member of DAG1 or DAG2. Then the unique fixed point is always a global attractor.
\end{conj}

We are not able to prove this conjecture for the full families DAG1 or DAG2. However, we define a smaller infinite family of graphs, \emph{shallow DAG1}, and show that graphs in this infinite family are dynamically robust in this sense. 

\begin{defn}
Let $G$ be a member of DAG1 with source node $s$ and target node $u$. We say $G$ is a member of \emph{shallow DAG1} if  it satisfies the additional property that if $i\to j$, then $i = s$ or $j = u$. 
 That is, if a node $j$ is not the target, then it may only receive input from the source $s$. 
\end{defn}

\begin{figure}[ht!]
\begin{center}
\includegraphics{ThresholdLinear/Figures/dynamic_robust.pdf}
\caption{A graph is a member of shallow DAG1 if only the target receives from a non-source vertex.}
\end{center}
\end{figure}

We prove Conjecture \ref{conj:dyn_robust} in the special case where $G$ is a member of shallow DAG1. 

\begin{thm}\label{thm:dag1global}
Let $G$ be a member of shallow DAG 1, and  $(W, \theta)$ be a TLN with  $G_W = G$.  This TLN has a unique fixed point which is a global attractor. 
\end{thm}

We also prove a second result, that if $G$ is any member of DAG1 and the coefficients are close enough to the CTLN coefficients, then all trajectories of the CTLN approach a fixed point. 

\begin{prop}\label{prop:near_ctln}
Let $G$ be a member of DAG1. There is an open set in $\R^{n\times n}$ containing the CTLN coefficients for $G$ such that if the weight matrix $W$ falls in this set, the TLN has a unique fixed point which is a global attractor. 
\end{prop}

\subsection{Shallow DAG1}

In order to prove Theorem \ref{thm:dag1global},  we generalize shallow DAG1 to a larger family of TLNs using strong domination. In order to do this, we need a notion of strong domination with respect to a set $\sigma\subseteq[n]$.

\begin{defn}
Neuron $k$ strongly dominates neuron $j$ with respect to $\sigma \subseteq [n]$ if $\wt W_{ji} \leq \wt W_{ki}$ for all $i\in \sigma$. 
\end{defn}

\begin{defn} Let $W$ be the weight matrix of a TLN. We say that $W$ satisfies the \emph{shallow DAG1 domination property} if there exist neurons $s$ and $u$ such that the following conditions hold:
\begin{enumerate}
\item  $u$ strongly dominates $s$ with respect to $[n]$
\item  for all $i\notin\{s, u\}$,  $u$ strongly dominates $i$ with respect to $[n]\setminus \{s\}$. 
\end{enumerate}

\end{defn}

\begin{prop}
If $G$ is a member of shallow DAG1, and $G_W = G$, then $W$ satisfies the shallow DAG1 domination property. 
Further, suppose that $G$ is a graph such that $W$ satisfies the shallow DAG1 property whenever $G_W = G$. Then $G$ is a member of shallow DAG1. 
\end{prop}

\begin{proof}
First, suppose $G$ is a member of shallow DAG1. Because $s$ is a source and $u$ is a target, then $W_{ui} >-1$ for all $i\neq u$, and $W_{si} < -1$ for all $i\neq s$. Thus $\wt W_{ui} > \wt W_{si}$ for all $i$, thus $u$ strongly dominates $s$. 
Now, because if $i\to j$, either $i = s$ or $j = u$, we have $W_{ij} < -1$ for all $j\neq s, i$ and $W_{uj} > -1$ for all $j\neq u$. Thus, $\wt W_{uj} > \wt W_{ij}$. 

Now, we show that if $G$ is not a member of shallow DAG1, there is some weight matrix $W$ such that $G = G_W$, but $W$ does not satisfy the shallow DAG1 domination property. If $s$ is not a source, then there is some $i$ such that $i\to s$. Then we can choose $W_{ui}$ such that $W_{ui} <W_{si}$.  Likewise, if $u$ is not a target,  then there is some $i$ such that $i\not \to u$. Then we can choose $W_{ui} < W_{si}$. In both of these cases, we violate the condition that $u$ strongly dominates $s$. 

Now, suppose that there is some $i\neq s$, $j\neq s$ such that $i\to j$. Then $W_{ji} > -1$. Then we can choose $W_{ji} > W_{ui}$, which means that $u$ does not strongly dominate $j$ with respect to $[n]\setminus \{s\}$. 
\end{proof}

We will prove that if a TLN satisfies the shallow DAG1 domination property, it has a unique fixed point which is globally attracting. This means if the graph  $G$ is a member of the shallow DAG1 family, then any TLN with $G_W = G$ has a unique fixed point which is globally attracting. Thus, these graphs are dynamically robust in the sense of Conjecture \ref{conj:dyn_robust}. 

\begin{prop}\label{prop:dag1domglobal}
Let $W$ be the weight matrix of a TLN satisfying the shallow DAG1 domination property. 
Then all activity of the TLN defined by $W$ approaches a stable fixed point at which $u$ is the only active neuron. 
\end{prop}

Notice that this implies Theorem \ref{thm:dag1global}, since all TLNs whose graphs are in DAG1 satisfy the shallow DAG1 domination property. 

%We begin with a simple lemma about strong domination. 
%
%\begin{lem}  \label{lem:strong_domination} 
%If $k$ strongly dominates $j$ with respect to $\sigma$, then 
%$$h_k^*(x) - h_j^*(x) > 0$$
%for all 
%$
%x\in \{\R^n \mid 
% x_i = 0 \mbox{ if } i\notin \sigma, 
%x_i \geq 0 \mbox{ if } i\in \sigma
%\}\setminus\{0\}
%$
%In particular, when $\sigma = [n]$, $h_k^*(x) > h_j^*(x)$ on the entire positive orthant, excluding the origin. 
%\end{lem}
%
%\begin{proof}
%We have 
%
%\begin{align*}
%h_k^*(x) - h_j^*(x)  &= \left(-x_k+ \sum_{i=1}^n W_{ki}x_i  + \theta \right) - \left(-x_j + \sum_{i=1}^n W_{ji}x_{i} + \theta \right) \\
%h_k^*(x) - h_j^*(x)  &= \sum_{i = 1}^n \wt W_{ki}x_i -  \sum_{i = 1}^n \wt W_{ji} x_i  = \sum_{i = 1}^n  (\wt W_{ki} - \wt W_{ji} )x_i 
%\end{align*}
%By the definition of strong domination, all coefficients $\wt W_{ki} - \wt W_{ji} $ of this sum are positive for $i\in \sigma$. Thus  when $ x\in \{\R^n \mid 
% x_i = 0 \mbox{ if } i\notin \sigma, 
%x_i \geq 0 \mbox{ if } i\in \sigma
%\}\setminus\{0\}$, 
%we have $h_k^*(x) - h_j^*(x) < 0 $. 
%
%\end{proof}
%
%This lemma has the following geometric interpretation: if $k$ strongly dominates $j$ with respect to $[n]$, then $H_j \cap H_k \cap \R^n_{> 0} = \emptyset$. Further, $H_k$ is separated from the origin by $H_j$. If  $k$ strongly dominates $j$ with respect to $\sigma$, then $H_k$ is separated from the origin by $H_j$ within the surface where $x_i$ is set to zero for all $i\in [n]\setminus \sigma$.  

\begin{lem}\label{lem:strong_dom_deriv}
If $k$ strongly dominates $j$, then either:
\begin{align*}
\xdot_k  > \xdot_j 
\end{align*}
or

\begin{align*}
y_j < 0,\,\, \xdot_j = -x_j
\end{align*}
\end{lem}

\begin{proof}
We have 
\begin{align*}
\xdot_k - \xdot_j &= -x_k +x_j + [y_k]_+ - [y_j]+\\
\xdot_k - \xdot_j &= h_k^*(x) - h_j^*(x) + ([y_k]_+ -y_k) - ([y_j]_+- y_j) 
\end{align*}
By Observation \ref{obs:strong_domination}, the term $h_k^*(x) - h_j^*(x)$ is always positive. By the definition of the threshold nonlinearity, the term $[y_k]_+ -y_k$ is always positive. Thus, we can only have $\xdot_k - \xdot_j \leq 0$ when the term $[y_j]_+- y_j$  is positive, which occurs when $y_j < 0$, $\xdot_j = -x_j$. 
\end{proof}

The next lemma is main part of the proof of Proposition \ref{prop:dag1domglobal}. 
Essentially, we are showing that for TLNs which satisfy the shallow DAG1 domination property, the function $x_u - x_s$ is a Lyapunov-like function within $\cA$. 
We will use this to show that trajectories which enter $\cA$ must approach a fixed point. 

\begin{lem}\label{lem:lyapanov}
If a TLN satisfies the shallow DAG1 domination property, then $\xdot_u - \xdot_s >  0$ on the interior of  $\cA$, with equality achieved on the boundary of $\cA$ on the set where $\xdot_u = \xdot_s = 0$. 
\end{lem}

\begin{figure}[ht!]
\begin{center}
\includegraphics[width = 4 in]{ThresholdLinear/Figures/robust_4.pdf}
\end{center}
\caption{Linear chambers and nullclines restricted to the $x_s, x_u$ plane. Nullclines are shown in red and blue, boundaries of linear chambers are shown in gray. The surface $\dot{x_s} = \dot{x_u}$ is shown in green.  \label{fig:cham}   }
\end{figure}

\begin{proof}
We prove this statement by considering the surface where $\xdot_u = \xdot_s$, and show that it does not intersect with the interior of $\cA$. Because the equations for $\xdot_s$ and $\xdot_u$ are threshold-linear, the surface  $\xdot_u = \xdot_s$ consists of at most four hyperplanes, one in each linear chamber. The surface $\dot{x_s} = \dot{x_u}$ and the linear chambers are illustrated in two dimensions in Figure \ref{fig:cham}. 

We first consider the case where $y_s\geq 0$, which covers the linear chambers $y_s \geq 0, y_u \geq 0$ and $y_s \geq 0, y_u< 0$. By Lemma \ref{lem:strong_dom_deriv}, we have $\xdot_u > \xdot_s$. 
%We first show that the surface  $\xdot_u = \xdot_s$  does not actually intersect with the chambers $\sum_{i=1}^n W_{ui}x_i + \theta\geq 0,     \,\, \sum_{i=1}^n W_{si}x_i + \theta \geq 0$ or $\sum_{i=1}^n W_{ui}x_i + \theta < 0,     \,\, \sum_{i=1}^n W_{si}x_i + \theta \geq 0$. 
%
%\begin{itemize}
% 
% \item 
% %$++$: 
% 
% $\sum_{i=1}^n W_{ui}x_i + \theta\geq 0,     \,\, \sum_{i=1}^n W_{si}x_i + \theta \geq 0$. \\ 
% In this case, the threshold nonlinearities have no effect, and 
% \begin{align*}
%\xdot_u- \xdot_s &= h_u^*(x) - h_s^*(x)%\xdot_u - \xdot_s &= (-1 - W_{su})x_u +(1+W_{us})x_s +  \sum_{i\neq s,u}^n (W_{ui}-W_{si})x_i 
% \end{align*}
%Because $u$ strongly dominates $s$, by  Lemma \ref{lem:strong_domination} this expression is always positive for all $x\in \R^n_\geq \setminus \{0\}$.   Thus, $\xdot_u-\xdot_s > 0$  within this chamber. 
%
%\item 
%% $-+$: 
%$\sum_{i=1}^n W_{ui}x_i + \theta < 0,     \,\, \sum_{i=1}^n W_{si}x_i + \theta \geq 0$. \\
% In this case, only the threshold nonlinearity for $u$ has an effect, so 
% \begin{align*}
%\xdot_u- \xdot_s &= x_s - x_u  - \sum_{i=1}^n W_{si}x_i -\theta\\
%\xdot_u- \xdot_s&= h_u^*(x) - h_s^*(x)- \left(\sum_{i=1}^n W_{ui}x_i -\theta\right)
% \end{align*}
%Again by Lemma \ref{lem:strong_domination}, the sum of the first four terms  is positive throughout the positive orthant. Where this case applies, the quantity  $\sum_{i=1}^n W_{ui}x_i -\theta$ is negative. 
%Thus $\xdot_u -\xdot_s > 0$ within this chamber as well. 
% \end{itemize}
% 
% 
Thus, the surface  $\xdot_u = \xdot_s$  does not actually intersect either of these chambers or their closures. 

We next consider the region where $y_s < 0$, which covers the chambers $y_s < 0, y_u \geq 0$ and $y_s < 0, y_u < 0$. We let $b\neq s, u$ be some bystander neuron.  We show that the surface where $\xdot_u = \xdot_s$ is strictly confined to the negative side of the $x_b$ nullcline $H_b$. To do this, we consider the quantity $\xdot_u - \xdot_s - \xdot_b$, and show that  $\xdot_u - \xdot_s - \xdot_b > 0$ when  $\xdot_b> 0$. 

Notice that when $\xdot_b > 0$, we must have $y_b > 0$. Thus, 
\begin{align*}
 \xdot_u - \xdot_s - \xdot_b &= -x_u + x_s + x_b + [y_u]_+-[y_s]_+- [y_b]\\
 \xdot_u - \xdot_s - \xdot_b &= -x_u + x_s + x_b + [y_u]_+- y_b\\
  \xdot_u - \xdot_s - \xdot_b &\geq -x_u + x_s + x_b + y_u- y_b\
 \end{align*}
 Now, we expand this to 
    \begin{align*}
\xdot_u-\xdot_s -\xdot_b &= x_b + x_s - x_u + \left(\sum_{i=1}^n W_{ui}x_i +\theta\right)  -\left( \sum_{i=1}^n W_{bi}x_i + \theta\right)\\
\xdot_u-\xdot_s -\xdot_b &= (1 -W_{bs}+W_{us})x_s +(-1-W_{bu})x_u + (1 +W_{ub})x_b + \sum_{i\neq u, s,b}^n (W_{ui}-W_{bi})x_i 
\end{align*}

The coefficients $  (1 -W_{bs}+W_{us})$, $(-1-W_{bu})$, and  $(1 +W_{ub})$  are positive because $u$ strongly dominates $s$ with respect to $[n]$.  The coefficients $(W_{ui}-W_{bi})$ are positive because $b$ strongly dominates $u$ with respect to $[n]\setminus \{s\}$.  Thus, this quantity is positive within the positive orthant.  Thus, when $\xdot_b > 0$, we must also have $\xdot_u - \xdot_s > 0$. This means that the surface where $\xdot_u = \xdot_s$ is contained strictly within the negative side of  $H_b$.  
 
% \begin{itemize}
% \item 
%  $y_u\geq 0,     \,\, y_s< 0$. \\ 
%  In this case, we have 
%  \begin{align*}
% \xdot_u - \xdot_s &= x_s - x_u +\sum_{i=1}^n W_{ui}x_i +\theta \\
%  \end{align*}
%  Now, let $b$ be some ``bystander" neuron, $b\neq s, u$. We show that the surface where $\xdot_u = \xdot_s$ is confined to the negative side of the $x_b$ nullcline $H_b$. Notice that when $\xdot_b > 0$, we must have $\xdot_b = -x_b + \sum_{i=1}^n W_{bi}x_i + \theta$.  Thus when $\xdot_b> 0$, where this case applies, 
%   \begin{align*}
%\xdot_u-\xdot_s -\xdot_b = x_b + x_s - x_u + \left(\sum_{i=1}^n W_{ui}x_i +\theta\right)  -\left( \sum_{i=1}^n W_{bi}x_i + \theta\right)\\
%\xdot_u-\xdot_s -\xdot_b = (1 -W_{bs}+W_{us})x_s +(-1-W_{bu})x_u + (1 +W_{ub})x_b + \sum_{i\neq u, s,b}^n (W_{ui}-W_{bi})x_i 
%\end{align*}
%The coefficients $  (1 -W_{bs}+W_{us})$, $(-1-W_{bu})$, and  $(1 +W_{ub})$  are positive because $u$ is a target and $s$ is a source. The coefficients $(W_{ui}-W_{bi})$ are positive on the assumption that if $b$ is not the target, it only receives from the source $s$. Thus, this quantity is positive within the positive orthant.  Thus, when $\xdot_b > 0$, we must also have $\xdot_u - \xdot_s \geq 0$. This means that the surface where $\xdot_u = \xdot_s$ is contained within the negative side of  $H_b$.  
%\item $\sum_{i=1}^n W_{ui}x_i + \theta < 0.,\,\,   \sum_{i=1}^n W_{si}x_i + \theta < 0$. \\

%In this case, we have 
%
%
%\begin{align*}
%\xdot_u - \xdot_s &= x_s - x_u \end{align*}
%
%Then the surface where $\xdot_s = \xdot_u$ is given by the plane $x_s = x_u$.
% \end{itemize}
% 
% Finally, we look at how these two pieces of $\xdot_s = \xdot_u$ intersect. The piece of the surface $x_s = x_u$ is bounded away from the origin by the piece $ \xdot_u - \xdot_s = x_s - x_u +\sum_{i=1}^n W_{ui}x_i +\theta $. 
%We showed that for every bystander neuron $b$, the piece of the surface  $ \xdot_u - \xdot_s = x_s - x_u +\sum_{i=1}^n W_{ui}x_i +\theta $ is contained on negative side of the $x_b$ nullcline $H_b$. 
%
% This surface is also contained on the closure of the negative side of both the $x_u$ and $x_s$ nullclines $H_u$ and $H_s$. To see this, we again apply Lemma \ref{lem:strong_domination}. However, we to have $\xdot_u = \xdot_s = 0$ along the intersection $H_u \cap E_s$. 

Finally, by Lemma \ref{lem:strong_dom_deriv}, if $\xdot_u = \xdot_s$, then $\xdot_s = -x_s\leq 0$, so we must have $\xdot_u \leq 0$. This means that the surface $\xdot_u = \xdot_s$ is confined to the negative side of $H_u$, but this might not be strict. 
 
Since our bystander neuron was arbitrary, we have shown that within the mixed-sign chamber $\cA$, $\xdot_u \geq \xdot_s$. On the piece of the boundary of the mixed sign chamber made up by $H_u$, we have $\xdot_u = \xdot_s = 0$ along the surface defined by $x_s = 0, -x_u + \sum_{i = 1}W_{ui}x_i +\theta = 0$. 
\end{proof}


Finally, we are ready to prove Proposition \ref{prop:dag1domglobal}. 
\begin{proof}

By Theorem \ref{thm:mixed_sign}, all trajectories approach $\cA$. First, we consider trajectories which do not ever enter $\cA$. Such trajectories remain in either $\cA^+$ or $\cA^-$ for all time. Then along these trajectories, the signs of each derivative $\xdot_i$ are fixed. Thus, for each $i$, the value of $x_i$ approaches a constant. Thus, these trajectories approach a limit, which must be a fixed point. This must be the unique fixed point of the network. 

Next, we consider trajectories which do enter $\cA$. By Lemma \ref{lem:lyapanov}, once the trajectory has entered $\cA$, it is subject to the constraint $\xdot_u - \xdot_s > 0$. Then this trajectory must approach the limit on the boundary of $\cA$ where $\xdot_u = \xdot_s = 0$. On this set, by Lemma \ref{lem:strong_dom_deriv}, $x_s = 0$. Thus, this trajectory must approach the surface where $x_s = 0$. 

Now, by condition (2) of the shallow DAG1 decomposition property, for all $i\notin \{s, u\}$, we have that $u$ strongly dominates $i$ with respect to $[n]\setminus \{s\}$. Thus, within the plane where $x_s = 0$, for each $i\neq u$, $H_i$ strictly separates $H_u$ from the origin. Because this separation is strict, there must be some $\epsilon > 0$ such that $H_i$ separates $H_u$ from the origin for all $x\in \R^n_{\geq 0}$ satisfying $0 \leq x_s < \epsilon$. Because the trajectory approaches this surface where $x_s =0$, after some time, the trajectory must satisfy $x_s < \epsilon$. At this point, to remain within the mixed-sign region $\cA$, the trajectory must have $\xdot_u > 0$. 

Thus, the trajectory must approach the nullcline for $x_u$. In particular, since we are increasing as we approach the nullcline, we must approach $H_u$. Thus, the trajectory also gets trapped on the negative side of each $H_i$. Therefore, since the signs of all derivatives are fixed, the trajectory must approach a limit, which must be a fixed point.  This must be the unique fixed point of the network. 
 \end{proof}

\subsection{Near CTLNs}

If a CTLN is a member of either DAG1 or DAG2, then by Theorem \ref{thm:dag_onto_symmetric} the unique fixed point is globally attracting. However, this result does not automatically extend to general TLNs. We are able to prove, however, that if a TLN has a graph $G_W$ that is a member of DAG1, and if the weights in $W$ are not too different from the CTLN weights, then the unique fixed point is a global attractor. 


\begin{prop}\label{prop:near_ctln}
Let $G$ be a member of DAG1 with a target vertex $n$. Let $W$ be a weight matrix satisfying $G_W = G$ and  for all $i,k\neq n$, $W_{nk} - W_{ik}> \frac{1}{d_{in}(i)}  (W_{in} + 1)$. Then all trajectories of a TLN defined by $W$ approach the unique fixed point. 
\end{prop}

Notice that this is a relaxation of the CTLN condition. The quantity $ \frac{1}{d_{in}(i)}  (W_{in} + 1)$ is negative, since $n$ is a sink. Now, in the CTLN case, since $n$ is a target, the quantity $W_{nk} - W_{ik}$ is always non-negative. We relax the CTLN condition by allowing the terms $W_{nk} - W_{ik}$ to be negative, but not \emph{too negative}, relative to 
$\frac{1}{d_{in}(i)}  (W_{in} + 1)$. The condition  $W_{nk} - W_{ik}> \frac{1}{d_{in}(i)}  (W_{in} + 1)$ is met on an open set of the parameter space containing the CTLN parameters. 

Our proof resembles that of Theorem \ref{thm:sources_die}, using local Lyapunov functions for a sequence of nested sets. 
\begin{figure}
\includegraphics[width =6 in]{ThresholdLinear/Figures/dag_lyapunov.pdf}

\caption{Proof idea for Proposition \ref{prop:near_ctln}. We label the vertices of $G$ with $1, \ldots, n$ according to a topological order (right).  A sequence of local Lyapunov-like functions  $L_1, \ldots, L_{n-1}$ (left) force trajectories into a nested sequence of regions $\Omega_1 \supset \Omega_2 \supset \cdots \supset \Omega_{n-1}$. }
\end{figure}

\begin{figure}
\includegraphics[width =4  in]{ThresholdLinear/Figures/composite_nested.pdf}

\caption{The regions $\Omega_1$ and $\Omega_2$ for a three-neuron network are obtained by intersecting the cones $\{x\mid x_1 \leq x_3\}$ and $\{x \mid x_1, x_2 \leq x_3\}$, illustrated here, with $\cA$. }
\end{figure}



\begin{defn}
Fix a topological ordering of the vertices of $G$ such that the source is numbered 1 and the target is numbered  $n$. 
Define 
\begin{align*}
\Omega_i(\epsilon) :&= \{ x\in \R^n_{\geq 0}\mid x_j \leq x_n +\epsilon\mbox{ for all } j \leq i\}\cap \cA\\
\Omega_i :&= \Omega_i(0)\\
\Omega_0 :&= \cA\\
\end{align*}

\end{defn}



Now, we will eventually prove that for some $\delta_i$, $L = x_i - x_n$ is a local Lyapunov function for $A = \Omega_i$, $B = \Omega_{i-1}(\delta_i)$. We will need to prove two lemmas first. 

\begin{lem}\label{lem:i_vs_n}
Under the assumptions of Proposition \ref{prop:near_ctln},
there exists a constant $\delta_i := \delta_i(W) > 0$ such that if $x\in \Omega_{i-1}(\delta_i)$, then $h_i^*(x) - h_n^*(x) < 0$. 
\end{lem}

\begin{proof}
We have 
\begin{align*}
  h_i^*(x) - h_n^*(x) = -(1 + W_{ni})x_i + (1 + W_{in})x_n + \sum_{k\to i} (W_{ik} - W_{nk})x_k + \sum_{j\not\to i}(W_{ij}-W_{nj})x_j .
\end{align*}
Notice that except for those of $ \sum_{k\to i} (W_{ik} - W_{nk})x_k$, all coefficients of this sum are non-positive.  Thus 

\begin{align*}
  h_i^*(x) - h_n^*(x) \leq  (1 + W_{in})x_n + \sum_{k\to i} (W_{ik} - W_{nk})x_k  + C,
\end{align*}

where $C = -(1 + W_{ni})x_i + \sum_{j\not\to i}(W_{ij}-W_{nj})x_j $. 

Let $a = \max_{k\to i}(W_{ik}-W_{nk})$. If $a\leq0$, then all terms of the sum are non-positive, thus we have   $h_i^*(x) - h_n^*(x) \leq 0$ throughout the positive orthant. Otherwise, we use the assumption that $x\in \Omega_{i-1}(\delta_i )$ to show that 
\begin{align*}
  h_i^*(x) - h_n^*(x) \leq (1 + W_{in})x_n + \sum_{k\to i} a x_k + C \\
  h_i^*(x) - h_n^*(x) \leq (1 + W_{in})x_n + \sum_{k\to i} a (x_n + \delta_i) +C \\
  h_i^*(x) - h_n^*(x) \leq (1 + W_{in} +d_{in}(i)a)x_n + d_{in}(i)a\delta_i + C 
\end{align*}
The term $(1 + W_{in} +d_{in}(i)a)x_n$ is negative by the assumption that  $W_{nk} - W_{ik}> \frac{1}{d_{in}(i)}  (W_{in} + 1)$. On the other hand, the term $ d_{in}(i)a\delta_i $ is positive. We show that for the appropriate $\delta_i $,  $x\in \Omega_{i-1}(\delta_i) $ implies that 
$ (1 + W_{in} +d_{in}(i)a)x_n + d_{in}(i)a\delta_i  \leq 0$. 

By Corollary  \ref{cor:total_pop}, $x\in \cA$ implies that $\sum_{\ell = 1}^n x_\ell \geq \frac{1}{-\min(W_{ij})}$. Let $c := \frac{1}{-\min(W_{ij})}$. Then $\sum_{\ell = 1}^n x_\ell \geq c$. Thus, there is some neuron $\ell$ such that $x_\ell \geq c/n$. Now, we consider two cases. First, if $\ell \leq i$, then we have $x_\ell \leq x_n + \delta$, so $x_n \geq c/n - \delta$. 
Then \begin{align*}
  h_i^*(x) - h_n^*(x) \leq (1 + W_{in} +d_{in}(i)a)\left(c/n - \delta \right)+ d_{in}(i)a\delta_i  + C
\end{align*}
  %  
Thus, for 
    
\begin{align*}
\delta_i (W) < \frac{-(1 + W_{in} + d_{in}(i)a)(c/n-\delta)}{d_{in}(i)a}
\end{align*}
we have 
\begin{align*}
  h_i^*(x) - h_n^*(x) &\leq 0
\end{align*}
as desired. 

Now, we consider the second case, when $\ell \geq i$. In this case, we expand the term $C$:

\begin{align*}
h_i^*(x) - h_n^*(x) \leq (1 + W_{in} +d_{in}(i)a)x_n + d_{in}(i)a\delta_i +  -(1 + W_{ni})x_i + \sum_{j\not\to i}(W_{ij}-W_{nj})x_j.
\end{align*}

Now, let $m = \max_{\ell \geq i}(W_{i\ell}-W_{n\ell})$. We are guaranteed $m \leq 0$, since we chose a topological ordering to label our neurons. Thus, we have

\begin{align*}
h_i^*(x) - h_n^*(x) \leq  d_{in}(i)a\delta_i + m x_\ell \\
h_i^*(x) - h_n^*(x) \leq  d_{in}(i)a\delta_i + m c/n .\\
\end{align*}

Thus, for $\delta_i \leq \frac{-mc/n}{d_{in}(i) a}$, we have $h_i^*(x) - h_n^*(x) $ as desired. 

Thus, for $$\delta_i <\frac 1 2\min\left(\frac{-mc/n}{d_{in}(i) a}, \frac{-(1 + W_{in} + d_{in}(i)a)(c/n-\delta)}{d_{in}(i)a}\right),$$
we have  $h_i^*(x) - h_n^*(x) $. 
Here $m =  \max_{\ell \geq i}(W_{i\ell}-W_{n\ell})$, $c = \frac{1}{-\min(W_{ij})}$, and $a = \max_{k\to i}(W_{ik}-W_{nk})$. 



\end{proof}



\begin{lem}
\label{lem:lyapunov_2}
Under the assumptions of Proposition \ref{prop:near_ctln},
there exists a constant $\delta_i := \delta_i(W)>0$ such that the function $L(x) = x_{i} - x_n$ is a local Lyapunov function for $A = \Omega_{i}, B = \Omega_{i-1}(\delta_i)$. 
\end{lem}

\begin{proof}


First, we notice that  for any value of $\delta \geq 0$, $L > 0$ on $\Omega_{i-1}(\delta_i)\setminus  \Omega_{i}(0)$ and $L \leq 0$ on $\Omega_{i}(0)$. Now, we show  that for the value of $\delta_i = \delta_i(W)$ used in Lemma \ref{lem:i_vs_n},  $\dot L < 0$ on $\Omega_{i-1}(\delta_i )\setminus  \Omega_{i}(0)$.  
We have 
\begin{align*}
\dot L (x) = \xdot_{i} -\xdot_n = -x_{i} + x_n + [y_{i}]_+ - [y_n]_+
\end{align*}
Pick $x\in \Omega_{i-1}(\delta_i) \setminus  \Omega_{i}(0)$ 
Since $x\notin  \Omega_{i}(0)$, we have $x_{i} > x_n$. Thus, by Lemma \ref{lem:thresh_ineq}, we have 
\begin{align*}
\xdot_{i} -\xdot_n \leq h^*_i(x) - h_n^*(x) 
\end{align*}
Now, by Lemma \ref{lem:i_vs_n}, $h^*_i(x) - h^*(n) < 0$. Thus $\dot L < 0$ on $\Omega_{i-1}(\delta_i)\setminus  \Omega_{i}(0)$.  


Finally, we check that $ \Omega_{i-1}(0)$ is a forward invariant set for our TLN. For $i = 1$, this follows from Theorem \ref{thm:mixed_sign}. For $i > 1$, this follows from the fact that $L = x_{i-1} - x_{n}$ is a local Lyapunov function for $A = \Omega_{i-1}$, $B  = \Omega_{i-2}(\delta_{i-1})$.

\end{proof}


Finally, we are ready to prove Proposition \ref{prop:near_ctln}. 

\begin{proof}[Proof of Proposition \ref{prop:near_ctln}]

We consider two cases, trajectories which do not enter $\cA$ and those which do. First, if a trajectory does not enter $\cA$, then signs of all derivatives are fixed, thus the trajectory approaches a fixed point. 

Next, we consider trajectories which enter $\cA$. We prove by induction along our topological order that for each $\epsilon> 0$, $i = 1, \ldots, n-1$, there exists $T$ such that if $t \geq T$, $x\in  \Omega_i(\epsilon)$. First, we prove the base case. Since the vertex $1$ is a source and $n$ is a target, $n$ strongly dominates $1$, so $h^*_1(x ) < h^*_n(x)$ for all $x$ in the positive orthant. Further, for $x\notin \Omega_1$, $x_1 > x_n$, so 
\begin{align*}
\xdot_1 - \xdot_n & = -x_1 + x_n + [y_1]_+ - [y_n]_+ \leq    -x_1 + x_n + y_1 - y_n\\
\xdot_1 - \xdot_n  &\leq  h^*_1(x ) - h^*_n(x) \leq 0.
\end{align*}
Thus $L= x_1 - x_n$ is a local Lyapunov like function for $\R^n_{\geq 0}, \Omega_1$. Thus, all trajectories approach $\Omega_1$. Therefore, there exists  $t \geq T$, $x(t) \in \Omega_i(\epsilon)$. 

Now, assume as an inductive hypothesis that the statement has been proved for all $j \leq i$. Pick $\epsilon > 0$. By Lemma \ref{lem:lyapunov_2}, there is a constant $\delta_i> 0$ so that  $L = x_{i+1} -x_n$ is a local Lyapunov function for $A = \Omega_i$, $B = \Omega_{i-1}(\delta) $. By the inductive hypothesis, we can choose $T_i$ so that for all $t\geq T_i$, $x\in \Omega_{i-1}(\delta_i)$. Therefore, by Lemma \ref{lem:lyapanov}, for $t> T$ the trajectory approaches $\Omega_i$. Thus, there is some $T$ such that for all $t\geq T$, $x(t) \in  \Omega_{i}(\epsilon)$.

Thus, for all $\epsilon > 0$, all trajectories enter the set $\Omega_{n-1}(\epsilon)$. Now, we pick $\delta = \max_{i \in[n]} \delta_i$. Then by Lemma \ref{lem:i_vs_n}, $h^*i(x) - h_n^*(x) < 0$ for all $x\in \Omega_{n-1}(\delta)$. This shows that the $x_n$ nullcline is separated from the origin by each $x_i$ nullcline within $\Omega_{n-1}(\delta)$.  Thus $\Omega_{n-1}(\delta) \subseteq H_n^+$. By our inductive argument, all trajectories which enter $\cA$ eventually enter the region $\Omega_{n-1}(\delta)$. Once they enter this region, $\xdot_n > 0$ for all time. Thus, the value of $x_n$ becomes monotonically increasing. Thus, it must approach a limit on $H_n$. Since $H_n$ is contained on the negative side of all other $H_i$, the signs of all derivatives $\xdot_i$ are fixed. Thus, the trajectory must approach the unique fixed point of the network.


\end{proof}





==> ThresholdLinear/ThresholdLinear_old.tex <==
% !TEX root = ../YourName-Dissertation.tex

\chapter{Threshold Linear Networks } \label{chapter:TLNs}
\section{Introduction}


Mathematical models of neural activity which are able to reproduce the rich variety of behavior observed in neural circuits must be nonlinear.
We study some of the simplest possible nonlinear models for neural activity, threshold-linear networks (TLNs). 
The firing rates $x_1, \ldots, x_n$ of neurons in a TLN are governed by the system of ordinary differential equations
\begin{align} \label{eqn:tln}
\frac{dx_i}{dt} &= -x_i + \left[\sum_{j = 1}^n W_{ij}x_j + b_i\right]_+,
\end{align}
which can be written in vector form as
\begin{align}
\frac{dx}{dt} &= -x + \left[Wx + b\right]_+. 
\end{align}
Here, $[y]_+ := \max\{y, 0\}$,  $W_{ij}$ the strength of the input to neuron $i$ from neuron $j$, and $ b$ is a constant external drive. 
TLNs have been used for decades as firing rate models of neural networks with simple, perceptron-like units. 
Because they are built out of locally linear systems, these networks are surprisingly tractable mathematically as compared to other high-dimensional nonlinear systems. 
However, while solutions to systems of linear ODEs either converge to a stable fixed point or diverge to infinity, solutions to TLNs can exhibit the full range of nonlinear behavior including multistability, limit cycles, and chaos. 

The activity of a neural circuit is determined by a variety of factors, such as intrinsic neural dynamics, external input, and the structure of network connectivity itself.  
Our goal is to understand the role of connectivity in shaping neural activity. 
Thus, we study models of neural activity which isolate the role of connectivity. 
Combinatorial threshold linear networks (CTLNs) are a special class of TLNs where $W$ is determined by a directed graph $G$ together with parameters $\epsilon$ and $\delta$ satisfying $\delta > 0$, $0< \epsilon< \frac{\delta}{\delta + 1}$, together with a constant external drive $\theta  >0   $ which is the same for all neurons.   
When $i\not \to j$, neuron $i$ strongly inhibits neuron $j$. When $i\to j$, neuron $i$ weakly inhibits neuron $j$. Values of $W_{ij}$ are given by the rule:

\vspace{-.15in}
\begin{align*}
W_{ij} = \begin{cases}
\;\;\; 0 &\mbox{ if }\,\, i = j\\
-1 + \epsilon&\mbox{ if } j \to i \mbox{ in }\,\, G\\
-1 - \delta &\mbox{ if } j \not \to i \mbox{ in }\,\, G.
\end{cases} 
\end{align*}
We interpret this as a network of $n$ excitatory neurons, against a background of instantaneous non-specific inhibition.  
Notice that the network is truly all-to-all connected, even when the graph $G$ is missing many edges. 
In particular, even networks which look feedforward are recurrent. CTLNs fall into a more general category of competitive TLNs, networks whose weights are negative. 
Given a competitive TLN with weight matrix $W$, we can define a graph $G_W$ by 
\[i\to j \mbox{ in } G_W \iff 	W_{ij}  > -1.\] 
Note that if $W$ is the weight matrix of a CTLN with graph $G$, $G_W = G$. We view the class of TLNs with graph $G$ as relaxations of the CTLN on $G$. 


A large body of work has focused on fixed points of TLNs in general and CTLNs in particular \cite{hahnloser2000permitted, 
curto2020combinatorial,  santander2021nerve, curto2019robust, curto2019fixed, curto2016pattern, curto2012flexible}. 
However, there is less known about their dynamic activity more broadly. On one end of the spectrum, the activity of a symmetric TLN always converges to a stable fixed point \cite{hahnloser2000permitted}. 
On the other end, \cite{morrison2016diversity} proves that CTLNs on oriented graphs with no sinks have bounded activity and no stable fixed points, and therefore must have persistent dynamic activity. 
It is possible to partially predict the structure of these attractors using graph properties \cite{parmelee2022core}. 
However, many CTLNs outside this family also exhibit persistent dynamic activity, and both dynamic attractors and stable fixed points can coexist in the same network. 
Even when a CTLN is guaranteed to have a dynamic attractor  by \cite{morrison2016diversity}, it is difficult to prove things about the structure of this attractor.  
One particular graph, the directed 3-cycle, is proved to have a limit cycle in \cite{bel2021periodic}. 


Here, we aim to characterize which CTLNs have dynamic attractors and which do not, and to constrain the dynamic attractors of CTLNs. 
Our proofs involve showing that we can force trajectories of TLNs into smaller regions of space. 
Because TLNs are threshold-linear, their nullclines are built from hyperplanes in a simple way.  
This allows us to use ideas from the theory of hyperplane arrangements, together with observations about the vector field in each chamber, to make conclusions about whether dynamic attractors are possible for networks corresponding to a given graph. 
Similar ideas are used in \cite{curto2020combinatorial} as a strategy for determining fixed points of general TLNs. 

We first prove that all trajectories of competitive TLNs approach and become trapped in a small region $\cA$ of phase space, corresponding to the set where at least one derivative is positive and at least one derivative is negative. This set is cut out by the hyperplanes defining the nullclines. 
\begin{ithm}
If $W,\theta$ defines a competitive TLN, $\cA$ is an attracting set, all trajectories approach it. 
\end{ithm}
This allows us to bound the total population activity of CTLNs: 
\begin{cor}
In CTLNs, \[\lim\inf_{t\to\infty} \sum_{i = 1}^n x_i \geq \frac{\theta}{1 + \delta}\] and  \[\lim\sup_{t\to\infty} \sum_{i = 1}^n x_i \leq \frac{\theta}{1 - \epsilon}.\] 
\end{cor}


We organize our work around the following conjecture: any CTLN with a dynamic attractor must have a proper directed cycle, as defined below. 
\begin{defn}
A \emph{proper directed cycle} of a directed graph is a directed cycle which has at least one edge which is not bidirectional. 
\end{defn}
\begin{conj}Let $G$ be a graph with no proper directed cycle. Then no CTLN with graph $G$ has a dynamic attractor. \label{conj:graph_struct}
\end{conj}

Note that the converse of this conjecture does not hold: see Figure \ref{fig:dir_no_attr} for an example of a graph which has a strongly directed cycle, but no dynamic attractor. 
We prove this conjecture in special cases. First, we note that applying the main result of \cite{hahnloser2000permitted} to symmetric CTLNs establishes that these networks do not have dynamic attractors. 
The next natural special case is the case of directed acyclic graphs (DAGs), graphs with no directed cycles at all. 

\begin{thm}
If $G$ is a directed acyclic graph, then no CTLN with graph $G$ has a dynamic attractor. \label{thm:dag}
\end{thm}

\begin{figure}
\begin{center}
\includegraphics[width = 5 in]{ThresholdLinear/Figures/tln_convergence_cases.pdf}
\end{center}
\caption{Classes of graphs such that all trajectories of their CTLNs are guaranteed to converge to a  fixed point.}
\label{fig:graph_classes}
\end{figure}


Thus, we have shown that CTLNs with either symmetric or feedforward architectures do not support dynamic attractors. 
It is natural to ask when it is possible to combine these two architectures to obtain a CTLN which we can guarantee has no dynamic attractors. 
One case in which we can do this is when a directed acyclic graph terminates on a symmetric graph. 

\begin{thm}
Let $G$ be a graph on vertex set $V$, and $\sigma, \tau$ be a partition of $V$. Suppose  the subgraph $G_\sigma$ is symmetric and connected, the subgraph $G_\tau$ is a directed acyclic graph, and that there are no edges from a vertex in $\tau$ back to a vertex in $\sigma$. 
Then no CTLN with graph $G$ has a dynamic attractor. \label{thm:dag_onto_symmetric}
\end{thm}

Our Conjecture \ref{conj:graph_struct} describes the much broader set of ways we believe it is possible to combine feedforward and symmetric elements to obtain a CTLN for which all trajectories are guaranteed to approach  a fixed point. 


Next, we explore to what extent our results extend to general competitive TLNs. In general, the graph $G$ does not determine the fixed point structure of the set of TLNs such that $G_W = G$ \cite{curto2019robust}. 
A graph $G$ is a \emph{robust motif} if all competitive TLNs with $G_W = G$ have the same set of fixed point supports. 
Almost all robust motifs fall into one of two infinite families, DAG1 and DAG2, with only a handful of exceptions. 
If $G$ is a robust motif, does the graph structure determine not just the fixed point structure of the graph, but also the presence of dynamic attractors?  Competitive TLNs with $G_W$ in either of these families each have a single stable fixed point. Further, in the CTLN case, these graphs have no dynamic attractors by our Theorems \ref{thm:dag} and \ref{thm:dag_onto_symmetric}, thus all trajectories approach the single stable fixed point.  It is natural to ask whether these graphs are ``dynamically robust": is it still true that all trajectories approach the single stable fixed point for all competitive TLNs such that $G_W$ is a member of DAG1 or DAG2? We conjecture that this is the case, and prove it in a special case, for graphs in a family we define and name \emph{shallow DAG1}. 

\begin{thm}
Let $G$ be a member of shallow DAG1. Then in any competitive TLN with $G_W = G$, all trajectories approach the single stable fixed point. 
\end{thm}






%Next, we use the combinatorial concept of domination, introduced in \cite{curto2019fixed}, to further constrain trajectories in terms of graph structure. In particular, we define strong and weak domination in terms of the graph structure of a CTLN, and show that this gives a constraint on its trajectories which we use to construct a dynamic memory network. 
%
%\begin{thm}
%\,
%\begin{itemize}
%\item If $k$ weakly dominates $j$, then the set $\{ x\in \R^n\mid x_k \geq x_j\}$ is a forward invariant set. That is, if $x_k \geq x_j$ at any time, then $x_k$ will remain greater than $x_j$ 
%
%\item If $k$ strongly dominates $j$, then the set $\{ x\in \R^n\mid x_k \geq x_j\}$ is an attracting setThat is, for all $\eta > 0$, there exists some $T_\eta \geq 0$ such that for all $t \geq T_\eta$, $x_k(t) +\eta > x_j(t)$. 
%
%\item If $k$ and $j$ receive equal input, the ordering of $x_k$ and $x_j$ is fixed. 
%\end{itemize}
%\end{thm}
%
%
%
%
%Next, we introduce  \emph{local Lyupanov-like functions}, which allow us to prove that trajectories of CTLNs become trapped in even smaller regions. Using this technique, we can constrain trajectories of CTLNs based on graph structure. This allows us to work towards a characterization of which CTLNs support dynamic attractors. In particular, \cite{curto2019fixed} proves that 	``sources die": if a neuron is a proper source in $G$, then it is not contained in the support of any fixed point of $G$. We prove a dynamic version of this result: if a graph $G$ satisfies a certain technical condition, then the activity of one of its sources must approach zero. 
%
%\begin{thm}
%\label{thm:sources_die}
%Let $G$ be a graph in which every vertex is reachable from a source. Then there is a source $j$ in $G$ such that $\lim_{t\to \infty} x_j(t) = 0$. 
%\end{thm}
%
%We use this result to obtain Theorems \ref{thm:dag} and \ref{thm:dag_onto_symmetric}. 
We also apply our results to classify CTLNs on three neurons. We prove that only the directed three-cycle has a dynamic attractor. 

\begin{thm}
The three-cycle is the only three neuron CTLN with persistent dynamic activity. 
\end{thm}





\section{Background}
Threshold linear networks (TLNs) are systems of ordinary differential equations whose dynamics are governed by Equation \ref{eqn:tln}. In this work, we are concerned with competitive TLNs. 
\begin{defn}
A TLN is \emph{competitive} if $W_{ij} \leq 0$ and $W_{ii} = 0$ for all $i$ and $j$, and $\theta \geq 0$.  
\end{defn}

Competitive TLNs always have bounded activity. While we will establish stronger bounds in this paper with Corollary \ref{cor:total_pop}, from \cite{curto2019fixed}, we have that trajectories of competitive TLNs which start in a box containing the origin stay there: if $x(0) \in \prod_{i = 1}^n[0, \theta]$, then $x(t) \in \prod_{i = 1}^n[0, \theta]$ for all $t >  0$.



Even though TLNs are nonlinear, they are locally or ``patchwork" linear. 
%, as illustrated in Figure \ref{fig:tln_eqn}.  That is, we can divide up the positive orthant into at most $2^n$ chambers based on whether $\sum_{j = 1}^n W_{ij}x_j + \theta \geq 0$ or  $\sum_{j = 1}^n W_{ij}x_j + \theta <0 $ for each $i$. We label each chamber by the set $\sigma = \{i \mid \sum_{j = 1}^n W_{ij}x_j + \theta \geq 0\}$. Within chamber $\sigma$, the dynamics are governed by the purely linear dynamical system 
%\begin{align*}
%\frac{dx_i}{dt} =\begin{cases} -x_i + W_{ij}x_j + \theta \qquad &i\in \theta\\
% -x_i \qquad &i \notin\theta.
% \end{cases}
%\end{align*}
%Define $A^\sigma$ to be the matrix of this linear system. That is, if $i\in \sigma$, the $i^{th}$ row of $A^\sigma$ is equal to the $i^{th}$ row of $-I + W$, and if $i\notin \sigma$, the $i^{th}$ row of $A_\sigma$ is equal to the $i^{th}$ row of $-I$. 
%
%\begin{figure}
%\begin{center}
%\includegraphics[width = 4 in]{ThresholdLinear/Figures/tln_equations.pdf}
%\end{center}
%\caption{TLNs can be seen as patchwork-linear networks, with a different linear system being active in each polyhedral chamber. \label{fig:tln_eqn}}
%\end{figure}
The fixed points of a dynamical system are the points $x^*\in \R^d$ such that 
$\frac{dx_i}{dt}\Big|_{x^*} = \,0$ for all $i\in [n]$. Because of patchwork linearity, each fixed point of a TLN must be a fixed point of the relevant linear system. However, a fixed point of a linear system may fail to be a fixed point of the TLN if that fixed point falls outside of the appropriate linear chamber. The \emph{support} of a fixed point is its set of active: $x^*$ is $\mathrm{supp}(x^*) := \{i \in [n]\mid x_i^* > 0\}$. There is at most one fixed point per support.  The set of fixed point supports for the TLN defined by $W, b$ is denoted $\FP(W, b)$. 

A fixed point is \emph{stable} if it is approached by all trajectories which start nearby. 
%The stability of a fixed point $x^*$ of a nonlinear system is determined by the eigenvalues of the Jacobian at $x^*$. In particular, $x^*$ is a stable fixed point if all of these eigenvalues have negative real part. Because TLN's are patchwork linear, the Jacobian at a point is just the matrix $A^\sigma$ of the linear system active in that chamber. Thus, the fixed point with support $\sigma$ of the TLN defined by $W, \theta$, if it exists, is stable if and only if all eigenvalues of the matrix $A^\sigma$ have negative real part.
Stable fixed points are a particular kind of attractor. 
\begin{defn}
A set $A$ is an \emph{attracting set} of a dynamical system if 
\begin{enumerate}
\item 
it is invariant: if $x (0) \in A$, then $x(t) \in A$ for all $t \geq 0$. 
\item 
it has an open basin of attraction: there is an open set $U$ containing $A$ such that if $x (0)\in U$, then the distance from $x(t)$ to $A$ approaches zero as $t$ approaches infinity. 
\end{enumerate}
An \emph{attractor} is a \emph{minimal} attracting set. That is, $A$ is an attractor if it is an attracting set and there is no $B\subsetneq A$ that is also an attracting set. 
\end{defn}
There are many attractors beyond stable fixed points, termed \emph{dynamic attractors}. These include limit cycles and strange attractors.   
By the main result of \cite{hahnloser2000permitted}, if the weight matrix $W$ is symmetric and the matrix $(I-W)$ is copositive, then the TLN defined by $W$ has a set of stable fixed points, and all trajectories of the network must approach one of these states. In particular, competitive TLNs satisfy this copositivity condition. Thus all trajectories of symmetric competitive TLNs (such as CTLNs defined from undirected graphs) must approach stable fixed points. Thus, these networks do not have dynamic attractors. 

On the opposite side of the spectrum, \cite{morrison2016diversity} proves that if $G$ is an oriented graph with no sinks, the CTLN defined by $G$ has no stable fixed points. Because trajectories of these networks cannot approach stable fixed points and cannot diverge to infinity, these networks must have dynamic attractors.  In one case, the directed three-cycle, this dynamic attractor has been explicitly characterized as a stable limit cycle \cite{bel2021periodic}. 

% I don't know where this paragraph should go. Move it up? Move it down? 
While Equation \ref{eqn:tln} is a common model for neural activity, other threshold linear models for neural activity appear in the literature, such as 
\begin{align} \label{eqn:tln_2}
\frac{d\mathbf v}{dt} &= -\mathbf v + W[\mathbf v]_+ +\theta\end{align}
The equivalence of models \ref{eqn:tln} and \ref{eqn:tln_2} is proven in \cite{miller2012mathematical}, generalizing a result from \cite{beer2006parameter}. When $W$ is invertible and $\theta$ is constant, \cite{beer2006parameter} shows that if $x$ evolves according to \ref{eqn:tln} if and only if $ v = W x + \theta$ evolves according to \ref{eqn:tln_2}. The more general case, when $W$ may not be invertible and $\theta$ may vary over time, is tackled in \cite{miller2012mathematical}. 	 

 \subsection{Nullclines, geometric picture}
We begin by describing nullclines of threshold linear networks in terms of hyperplane arrangements. 
A deeper account of the nullcline arrangement of a threshold linear network, from the perspective of oriented matroid theory, can be found in \cite{curto2020combinatorial}. 
\subsubsection{Defining nullclines}


The $i^{th}$ nullcline $\cN_i$ of a dynamical system is the set of all $x \in \R^n$ such that 
$\xdot_i = 0.$
Nullclines of linear systems are hyperplanes.
Because TLNs are threshold-linear, their nullclines are unions of pieces of hyperplanes. 


\begin{defn}
Given a weight matrix $W\in \R^{n\times n}$, $\theta \in \R$, we define affine-linear functionals
\begin{align*}
e_i^*(x) &:= -x_i\\
h_i^*(x) &:= -x_i + \sum_{j=1}^n W_{ij}x_j + \theta.
\end{align*}
These define hyperplanes $E_1, \ldots, E_n, H_1, \ldots, H_n $. The hyperplane arrangement of the TLN defined by $W$ and $\theta$ is the set $$\cA(W, \theta) = \{E_1, \ldots, E_n,H_1, \ldots, H_n\},$$ with the orientation (i.e. choice of positive and negative half-spaces) of each hyperplane given by $e_i^*$, $h_i^*$.   
\end{defn}

We describe the nullclines in terms of the hyperplanes $E_1, \ldots, E_n, H_1, \ldots, H_n$. 

\begin{prop}
The $i^{th}$ nullcline of a TLN is 
$$\cN_i = \left(H_i\cap E_i^-\right)\cup \left(E_i \cap H_i^-\right).$$
\end{prop}

\begin{proof}
We show that $x_i' < 0$ if and only if  $\vec{x}\in H_i^-\cap E_i^-$, and $x_i' > 0$ if $x \in H_i^+\cup E_i^+$. If $x\in H_i^-\cap E_i^-$, then  $$\max\left\{-x_i, -x_i + \sum_{j=1}^n W_{ij}x_j + \theta\right\} = -x_i + \left[\sum_{j=1}^n W_{ij}x_j + \theta\right]_+ < 0,$$ so $x_i' < 0$.  Now, if $x \in H_i^+\cup E_i^+$, then 
$$\max\left\{-x_i, -x_i + \sum_{j=1}^n W_{ij}x_j + \theta\right\} = -x_i + \left[\sum_{j=1}^n W_{ij}x_j + \theta\right]_+ > 0,$$
so $x_i' > 0$. 
Now, by continuity, we must have $x_i' = 0$ on the boundary between $H_i^-\cap E_i^-$ and $H_i^+\cup E_i^+$, which is the set $\left(H_i\cap E_i^-\right)\cup \left(E_i \cap H_i^-\right)$. 
\end{proof} 


\begin{ex}



Let $G$ be a the graph consisting of two vertices and a single directed edge from vertex 2 to vertex 1. Then the TLN arising from $G$ has the weight matrix 
$$W =  
\begin{pmatrix}
0& -1+ \epsilon \\
-1-\delta & 0
\end{pmatrix}.$$

\label{ex:edge_null}
\begin{figure}[ht!]
\includegraphics{ThresholdLinear/Figures/n=2_hyperplanes.pdf}
\caption{Nullclines for the CTLN of a single directed edge. The $x_1$ nullclines, $E_1$ and $H_1$, are in red, $E_2$ and $H_2$ are in blue. Black arrows point towards the positive side of each hyperplane. \label{fig:nullcline_edge}}
\end{figure}

The hyperplanes $E_1, E_2, H_1, H_2$, shown in the Figure \ref{fig:nullcline_edge}, are given by the equations 
\begin{align*}
E_1 &= \{x | -x_1 = 0\}\\
E_2 &= \{x | -x_2 = 0\}\\
H_1 &= \{x | -x_1 + (-1+\epsilon)x_2 + \theta = 0\}\\
H_2 &= \{x | -x_2 + (-1-\delta)x_2 + \theta = 0\}.
\end{align*}
The $x_1$ nullcline consists of the piece of $H_1$ on the negative side of $E_1$ together with the piece of $E_1$ on the negative side of $H_1$. Likewise, the $x_2$ nullcline consists of the piece of $H_2$ on the negative side of $E_2$ together with the piece of $E_2$ on the negative side of $H_2$. The pieces of $E_1, E_2, H_1$, and $H_2$ which act as nullclines are shown in darker colors in Figure \ref{fig:nullcline_edge}. The fixed point of this TLN is the point of intersection between these two nullclines, and appears as a white disk in the figure. 


\end{ex}

Notice that in this example, the fixed point occurs at the intersection of both nullclines. This is true in general: the set of fixed points of a TLN is the intersection of all of the nullclines, since this is exactly the set where all derivatives are zero.

%%%%%%%%%%%%%%%%%%%%%%%%% Drawing Nullclines %%%%%%%%%%%%%%%%%%%%%%%%%%%%positive orthant. This allows us to describe the $H_i$ in terms of convex hulls, which is helpful when sketching the nullclines. 
The following proposition makes it easier to sketch nullclines, especially in three dimensions. 
\begin{prop}\label{prop:cvx_hull}
Let $W$ be a competitive TLN. Define $b_{ij} = \frac{-\theta}{W_{ij}}e_j$ for $i\neq j$, $ b_{ii} = \theta \,e_i$. Then
\begin{align*}
H_i \cap \R^n_{\geq 0} =  \conv\left(\{b_{ij}\mid j = 1, ..., n\}\right).
\end{align*}
\end{prop}

\begin{proof}
Recall that $H_i$ is the zero set of 
$$h_i^*(x) = -x_i + \sum_{j=1}^n W_{ij}x_j + \theta.$$
Along the $x_j$ axis generated by $e_j$, we can set the other variables to zero, so for $i\neq j$, we have
\begin{align*}
0 = h_i^*(x) =  W_{ij}x_j + \theta\\
x_j = \frac{-\theta}{W_{ij}}
\end{align*}
and for $i = j$, 
\begin{align*}
0 = h_i^*(x) =  -x_i  + \theta\\
x_i = \theta 
\end{align*}
Thus, for each $j$, $b_j$ is the intersection of $H_i$ with the $x_j$ axis.  Thus, these points and their affine span are contained in $H_i$. These points are affinely independent, and there are $n$ of them, so affine span is equal to $H_i$. That is, each point of $H_i$ can be written as 
$$x = \sum \lambda_j b_j$$
subject to the constraint that $\sum_{j = 1}^n \lambda_j = 1$. 

Now, if $x\in H_i\cap \R^n_+$, we can take each $\lambda_i \geq 0$. Thus, $x$ a convex combination of the points $\{b_j\mid j = 1, \ldots, n\}$. Thus, $H_i \cap \R^n_{\geq 0} =  \conv\left(\{ b_{ij}\mid j = 1, ..., n\}\right)$. 
\end{proof}

\begin{ex}
We use Proposition \ref{prop:cvx_hull} to sketch nullclines for the CTLN corresponding to the graph $G = (V = \{1, 2, 3\}, E = \{2\to 1, 2 \to 3\})$ in Figure \ref{fig:nullclines_3}. Notice that specializing to the case of CTLNs simplifies our descriptions of the points $ b_{ij}$. If $j \not\to i$, $b_{ij} = \frac{\theta}{1+ \delta}$ and if $j \to i$, $ b_{ij} = \frac{\theta}{1-\epsilon}$. Also notice that $\frac{\theta}{1+ \delta} < \theta < \frac{\theta}{1-\epsilon}$. Thus, the absence or presence of an edge $j \to i$ tells us how the point where $H_j$ intersects the $x_i$ relates to the point where $H_i$ intersects the $x_i$ axis. The fixed points lie at the points of intersection between all three nullclines. These are marked with white circles. 
\begin{figure}[ht!]
\includegraphics[width = 6 in]{ThresholdLinear/Figures/nullclines_3.pdf}
\caption{Nullclines for a CTLN on three neurons.\label{fig:nullclines_3}}
\end{figure}
\end{ex}

\section{Nullcline chambers and dynamics}
\subsection{Basic definitions}
In the previous section, we talked about how the hyperplane arrangement $\cA(W, \theta)$ controls the fixed points of a TLN. Now, we explore how the hyperplane arrangement controls other dynamic properties of the TLN. In particular, we discuss the \emph{chambers} of this arrangement. These chambers are defined by the sign of the derivative at each point of $\R^n$.  

\begin{defn}
A \emph{sign vector} $X$ of length $n$ is an element of $\{0, +, -\}^n$. 
\end{defn}

\begin{defn}
Given a TLN defined by $W, \theta$ and a sign vector $X$, we define the \emph{chamber} of $X$ to be the set 
\begin{align*}
A_{W, \theta}(X) = \{x \in \R^n \mid \sign(x_i') = X_i\}.
\end{align*}
\end{defn}
Because TLNs are threshold linear, these chambers can be described in terms of the hyperplane arrangement. 
\begin{prop}
Let $X\in \{0,+, -\}^n$. 
\begin{align*}
A_{W, \theta}(X) = \bigcap_{X_i = +} (H_i ^+\cup E_i^+) \cap \bigcap_{X_j = -} (H_j^- \cap E_j^-) \cap \bigcap_{X_k = 0}\left( \left(H_i\cap E_i^-\right)\cup \left(E_i \cap H_i^-\right)\right).
\end{align*}
Within the strictly positive orthant, $\R^n_> = \{x\in \R^n\mid x_i > 0 \mbox{ for all } n \}$ this simplifies to 
\begin{align*}
A_{W, \theta}(X)\cap \R^n_> = \bigcap_{X_i = +} H_i ^+ \cap \bigcap_{X_j = -} H_j^-  \cap \bigcap_{X_k = 0} H_i
\end{align*}
\end{prop}

\begin{ex}
In Figure \ref{fig:edge_chambers}, we show the nullcline chambers for the graph with the single edge $1\to 2$. The four maximal nullcline chambers are the four possible sign vectors on $\{+, -\}^n$, $--, -+, +-, ++$. However, restricting to the positive orthant cuts off the $-+$, leaving us with three chambers $--, +-, ++$. 
\begin{figure}[ht!]
\includegraphics[width = 4 in]{ThresholdLinear/Figures/with_topes_labeled.pdf}
\caption{Maximal nullcline chambers for the single directed edge. The positive side of each hyperplane is indicated with an arrow. Additionally, the the positive side of each nullcline is shaded. Each chamber is labeled with the appropriate sign vector. \label{fig:edge_chambers}}
\end{figure}
\end{ex}

%%%%%%%%%%%%%%%%%%%%%%%% MIXED SIGN CHAMBERS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Activity sucked into union of mixed-sign chambers}
Now, we show that for competitive TLNs the chambers of $--\ldots-$ and $++\ldots+$ are repelling, and that all trajectories of the TLN eventually approach the union of the mixed-sign chambers. This constrains trajectories to a small subset of the positive orthant. 


\begin{defn}
We define the \emph{mixed sign region} $\cA$ as the closure of the set 
$$\{x\in \R^{n}_{\geq 0} \mid \mbox{ there exist } \, i, j \mbox{ such that } \sign(\xdot_i) = - \mbox{ and } \sign(\xdot_j) = +\}.$$
That is, $\cA$ is the region where not all derivatives have the same sign. 
Similarly, we define the two pieces of the complement of $\cA$ as
\begin{align*}
\cA^+ &= \{x\in \R^{n}_{\geq 0} \mid  \sign(\xdot_i) = +  \mbox{ for all } i\}\\
\cA^- &= \{x\in \R^{n}_{\geq 0} \mid  \sign(\xdot_i) = -  \mbox{ for all } i\}.
\end{align*}
\end{defn}
Notice that $\cA$ is bounded by the nullclines. In particular, within the positive orthant, it is bounded by the hyperplanes $H_1, \ldots, H_n$. Since the fixed points are the points where all nullclines intersect, they are always on the boundary of the mixed-sign chamber. A two-dimensional example is illustrated in Figure \ref{fig:mixed_sign}. 


\begin{thm}\label{thm:mixed_sign}
For any competitive TLN, the mixed sign region $\cA$ is a globally attracting set. In particular, trajectories which enter $\cA$ cannot leave. 
\end{thm}

\begin{proof}
First, note that within $\cA^+$, all derivatives $\xdot_i$ are positive. Thus, the trajectory must approach the boundary between $\cA^+$ and $\cA$. Likewise, within $\cA^-$, all derivatives $\xdot_i$ are negative, thus  the trajectory must approach the boundary between $\cA^-$ and $\cA$. 

Next, we show that if a trajectory is on the boundary between either $\cA^+$ and $\cA$ or $\cA^-$ and $\cA$, it must enter $\cA$. We first consider the boundary between $\cA^+$ and $\cA$. Since $W$ is the weight matrix of a competitive TLN, all entries of the normal vector $\vec h_i$ to the hyperplane $H_i$ are negative for all $i$. 
On the boundary between $\cA^+$ and $\cA$,  $\xdot \geq 0$ in all coordinates. Thus, $ \xdot\cdot \vec h_i \leq 0$, with equality only achieved at fixed points. Thus, unless the trajectory is at a fixed point, it must cross from $\cA^+$ into $\cA$. Likewise, if the trajectory is on the boundary between $\cA^-$ and $\cA$, $\xdot \leq 0$ in all coordinates.   Thus, $ \xdot\cdot \vec h_i \geq 0$, with equality only achieved at fixed points. Thus, the trajectory must cross from $\cA^+$ into $\cA$. 
\end{proof}



We can use this result to derive bounds on the total population activity of competitive TLNs in general, and CTLNs in particular.  

\begin{cor}\label{cor:total_pop}
Let $m = \min_{i, j}\{(I - W_{ij})\}$ and $M = \max_{i, j}\{(I - W_{ij})\}$. 
In competitive TLNs, 
\[\lim\inf_{t\to\infty} \sum_{i = 1}^n x_i \geq \frac{\theta}{M}\] and  \[\lim\sup_{t\to\infty} \sum_{i = 1}^n x_i \leq \frac{\theta}{m}.\] 
In CTLNs this result specializes to \[\lim\inf_{t\to\infty} \sum_{i = 1}^n x_i \geq \frac{\theta}{1 +\delta}\] and  \[\lim\sup_{t\to\infty} \sum_{i = 1}^n x_i \leq \frac{\theta}{1 -\epsilon}.\] 
\end{cor}

\begin{proof}
We show that, within the positive orthant, $\cA$ is contained between the hyperplanes $$\sum_{i = 1}^n x_i -\frac{\theta}{M} = 0 $$ and $$\sum_{i = 1}^n x_i - \frac{\theta}{m} =0.$$
By Proposition \ref{prop:cvx_hull}, for each $i$, the hyperplane $H_i$ is the convex hull of the points $\mathbf b_{ij} = \frac{-\theta}{W_{ij}}\mathbf{e_j}$ for $i\neq j$, $\mathbf b_{ii} = \theta \,\mathbf e_i$. Each point $\vec b_{ij}$ is on the positive side of the hyperplane defined by $\sum_{i = 1}^n x_i -\frac{\theta}{M} = 0 $ and on the negative side of the hyperplane defined by $\sum_{i = 1}^n x_i - \frac{\theta}{m} =0$. Thus, since all trajectories must approach $\cA$, they must also approach the region between the hyperplanes $\sum_{i = 1}^n x_i -\frac{\theta}{M} = 0 $ and $\sum_{i = 1}^n x_i - \frac{\theta}{m} =0$. Thus, 
\[\lim\inf_{t\to\infty} \sum_{i = 1}^n x_i \geq \frac{\theta}{M}\] and  \[\lim\sup_{t\to\infty} \sum_{i = 1}^n x_i \leq \frac{\theta}{m}.\] 
If $W$ is the matrix of a CTLN, then $m = 1-\epsilon$ and $M = 1+ \delta$, thus 
\[\lim\inf_{t\to\infty} \sum_{i = 1}^n x_i \geq \frac{\theta}{1 +\delta}\] and  \[\lim\sup_{t\to\infty} \sum_{i = 1}^n x_i \leq \frac{\theta}{1 -\epsilon}.\] 

\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%% NULLCLINE CHAMBERS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{How nullcline chambers shape dynamics}
\begin{defn}
Define a directed graph $T_{W, \theta} = (V, E)$ whose vertices correspond to nullcline chambers of the TLN defined by $W, \theta$ and whose edges correspond to possible transitions between chambers. That is, 
$V = \{ X\in \{+, -\}^n\mid A_{W, \theta, X} \neq \emptyset\}$, and the edge $(X\to Y) \in E$ if there is a point $x$ on the boundary between $X$ and $Y$ such that $\vec{\xdot}$ points from $X$ to $Y$. 
\end{defn}

We now prove that trajectories follow the edges of $T_{W, \theta}$. 
\begin{lem}\label{lem:folloW_edges}
Any trajectory of the TLN defined by $W, \theta$ must follow a directed path in $T_{W, \theta}$. 
\end{lem}

\begin{proof}
Suppose a trajectory crosses directly from the chamber $A_{W, \theta}(X)$ to the chamber $A_{W, \theta}(Y)$. Then at some time $t$, $x(t)$ is on the boundary between $A_{W, \theta}(X)$ and $A_{W, \theta}(Y)$. The direction it is going at time $t$ is given by $\xdot(t)$. Thus, in order to cross from $A_{W, \theta}(X)$ to $A_{W, \theta}(Y)$, $\xdot(t)$ must point from $A_{W, \theta}(X)$ to $A_{W, \theta}(Y)$.
\end{proof}

\begin{ex}
We consider again the directed edge. We have $T_{W, \theta} = (V, E)$ with $V = \{--, +-, ++\}$ and $E = \{(-- \to +-), (++ \to +-)$\}. To see this, we first note that edges must be between adjacent chambers. The edge between $--$ and $+-$ corresponds to crossing the $x_1$ nullcline $H_1$. On this nullcline, we have $x_1' = 0$ and $x_2' < 0$. Thus, we are going straight down. Therefore, $\xdot$ points from the chamber $--$ to the chamber $+-$. The edge between $++$ and $+-$ corresponds to crossing the $x_2$ nullcline. On this nullcline, we have $x_2' = 0$, $x_1' > 0$. Thus, we are going right. Therefore, whenever we cross this nullcline, we must cross from the chamber $++$ to the chamber $+-$. 

\begin{figure}[ht!]
\includegraphics[width = 4 in]{ThresholdLinear/Figures/transition_graph_edge.pdf}
\caption{The transition graph $T_{W, \theta}$ for the single directed edge. The gray arrows are the vectors $\xdot$ on the nullclines.  \label{fig:trans_graph}}
\end{figure}
\end{ex}

Not only must transitions between chambers follow edges of $T_{W, \theta}$, dynamic attractors must follow directed cycles in  $T_{W, \theta}$. To prove this, it is sufficient to prove that single chambers of  $T_{W, \theta}$ to not contain dynamic attractors. 


\begin{lem}\label{lem:single_chamber}
If a trajectory is contained on one side of the $i^{th}$ nullcline, then the value of $x_i(t)$ along this nullcline approaches a limit.  If a trajectory of a TLN is contained within a nullcline single chamber, then it approaches a fixed point. 
\end{lem}

\begin{proof}
If a trajectory is contained on one side of the $i^{th}$ nullcline, then the sign of $x_i'(t)$ along this trajectory is fixed. Thus, the function $x_i(t)$ is bounded and is either monotonically increasing or monotonically decreasing. Thus, $x_i(t)$ approaches a limit. 

Within a single chamber of $A_{W, \theta, X}$,  $x_i(t)$ approaches a limit for all $i = 1, ..., n$, thus the trajectory approaches a fixed point. 
\end{proof}

\begin{prop}\label{prop:directed_cycle} Any dynamic attractor of the TLN defined by $W, \theta$ must follow a directed cycle of $T_{W, \theta}$. 
\end{prop}

\begin{proof}
By Lemma \ref{lem:folloW_edges}, any trajectory must follow edges of $T_{W, \theta}$. By Lemma \ref{lem:single_chamber}, a dynamic attractor can never become trapped in a single chamber. Thus, it must transition between chambers infinitely many times. Since $T_{W, \theta}$ has only finitely many vertices of, the trajectory must thus return to a chamber is has visited before, thus following a directed cycle.  
\end{proof}

Proposition \ref{prop:directed_cycle} allows us to prove that a given TLN does not have a dynamic attractor. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% n = 2 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{$N = 2$ competitive TLN classification}
\begin{figure}[ht!]
\includegraphics[width = 5 in]{ThresholdLinear/Figures/n_2_class.pdf}
\caption{In each subplot, we have the nullcline arrangement and transition graph $T_{W, \theta}$ corresponding to the connectivity graph in the upper right corner. Gray arrows on nullclines give the direction of the derivative on this piece of the nullclines. \label{fig:n_2_class}}
\end{figure}

The transition graph $T_{W, \theta}$ allows us to easily prove that competitive TLNs with two neurons do not have dynamic attractors.

\begin{prop}\label{prop:n=2}
All trajectories of competitive TLNs with two neurons converge to stable fixed points. 
\end{prop}

\begin{proof}
The transition graph $T_{W, \theta}$ is completely determined by the connectivity graph $G_{W, \theta}$. In particular, if $W_{12} \leq -1$, the intersection of $H_1$ with the $x_2$ axis is closer to the origin than the intersection of $H_2$ with the $x_2$ axis, and if $W_{12} \leq -1$ the intersection of $H_1$ with the $x_2$ axis is further from the origin than the intersection of $H_2$ with the $x_2$ axis. Similarly, the relationship between $W_{21}$ and -1 determines the relative positions of the intersections of $H_1$ and $H_2$ with the $x_1$ axis. These relationships are sufficient to completely determine all combinatorial properties of the hyperplane arrangement $E_1, E_2, H_1, H_2$, and thus the graph $T_{W, \theta}$.  All possible arrangements are shown in Figure \ref{fig:n_2_class}. We notice that none of these graphs have directed cycles. Thus, by Proposition \ref{prop:directed_cycle}, none of these graphs have dynamic attractors.  
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%% n = 2, noncompetitive %%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Non-competitive TLNs for $n = 2$ }

While we have shown that competitive TLN's with 2 neurons, this result does not hold for general TLNs with two neurons. In particular, we consider the TLN defined by 
\begin{align*}
W = \begin{pmatrix}
2 & -1 \\ 2 & 0
\end{pmatrix} && \theta = \begin{pmatrix}
2 \\ 1 
\end{pmatrix},
\end{align*}
which is introduced in \cite{tang2005analysis}. This TLN does, in fact, have a limit cycle. We can see that this limit cycle corresponds to a directed cycle in its transition graph, as illustrated in Figure \ref{fig:n=2cycle}. 

\begin{figure}[ht!]
\includegraphics[width = 4 in]{ThresholdLinear/Figures/n_2_osc.pdf}
\caption{A two neuron, non competitive TLN with a limit cycle.\label{fig:n=2cycle} }
\end{figure}

Additionally, notice that this limit cycle is not confined to the union of the two mixed-sign chambers, $-+$ and $+-$. Instead, the limit cycle visits all four nullcline chambers. Thus, we see that the assumption that networks are competitive is necessary for Theorem \ref{thm:mixed_sign}. 


\section{Local Lyapunov Functions}
Our Proposition \ref{thm:mixed_sign} shows that all trajectories of TLNs approach the mixed sign chamber. In this section, we explore a wider variety of cases when we can prove that all trajectories of a dynamical system approach a smaller region of space. In particular, we introduce \emph{local Lyapunov functions}, a tool for showing all trajectories which are trapped in a region $B$ eventually approach a smaller region $A\subset B$. We begin with a few special cases, proving dynamic consequences of the combinatorial concept of graphical domination, before moving on to the general case. 

\subsection{Domination}

In this section, we review the concept of \emph{domination}, introduced in \cite{curto2019fixed}. While \cite{curto2019fixed} uses domination to establish constraints on fixed points of CTLNs, we show that it constrains dynamic attractors as well. 

\begin{defn}
Let $W$ be the weight matrix of a TLN on $n$ neurons. We say $k$ \emph{strongly dominates} $j$, written $k >_W j$,  if $\wt W_{ki} \geq \wt W_{ji}$ for all $i$.  

If $W$ is the weight matrix of a CTLN with graph $G$, then strong domination is equivalent to the following condition on $G$, termed \emph{graphical domination}: 
$k$ graphically dominates $j$, written $k >_G j$, if the following conditions hold: 
\begin{itemize}
\item For each vertex $i \neq j, k$, if $i\to j$, then $i \to k$. 
\item  $k\not\to j$
\item  $j \to k$
\end{itemize}
\end{defn}  

We also consider a weaker version of domination. 

\begin{defn}
Let $W$ be the weight matrix of a TLN on $n$ neurons. We say $k$ \emph{weakly dominates} $j$ if for all  $i\neq j, k$, $\wt W_{ki} \geq W_{ji}$, and $\wt W_{jk} = \wt W_{kj}$.   

If $W$ is the weight matrix of a CTLN with graph $G$, then weak domination is equivalent to the following condition on $G$, termed \emph{weak graphical domination}:  $k$ weakly graphically dominates $j$ if the following conditions hold

\begin{itemize}
\item For all $i$, if $i\to j$, then $i \to k$. 
\item $k\to j$ if and only if $j \to k$. 
\end{itemize}

\end{defn}  


\begin{defn}
Neurons $j$ and $k$ are \emph{equal input} if $j$ weakly dominates $k$ and $k$ weakly dominates $j$. 
\end{defn}


\begin{ex}
Consider the graph with $V = \{1, 2, 3\}$, $E = \{(1 \to 2), (2\leftrightarrow 3), (3 \to 1)\}$, pictured in Figure \ref{fig:dom_ex}. Then 2 strongly dominates 1, 2 weakly dominates 3, and 1 and 3 have no domination relationship.
\begin{figure}[ht!]
\begin{center}
\includegraphics{ThresholdLinear/Figures/dom_ex.pdf}
\end{center}
\caption{In this graph, 2 strongly dominates 1, 2 weakly dominates 3, and 1 and 3 have no domination relationship. \label{fig:dom_ex}}
\end{figure}
\end{ex}






\subsubsection{Basic results}
We begin with the following observation about strong domination: 
\begin{obs}\label{obs:strong_domination}
Let $k$ strongly dominate $j$,  $\wt W_{ki} \geq \wt W_{ji}$. Then for all $x$ in the positive orthant, 
$$h_k^*(x) - h_j^*(x) = \sum_{i= 1}^n (\wt W_{ki}-\wt W_{ji})x_i \geq 0.$$
\end{obs}

We first see how this shapes the arrangement of nullclines. 

\begin{prop}\label{prop:dom_sep}
If $k$ strongly dominates $j$, then $H_j$ separates $H_k$ from the origin. 
\end{prop}

\begin{proof}
By Observation \ref{obs:strong_domination}, $h_k^*(x) - h_j^*(x) \geq 0$ throughout the positive orthant.
Thus, on the $H_j$ nullcline, where  $h_j^*(x) = 0$, we must have $h_k^*(x)\geq 0$. Therefore, within the positive orthant, $H_j$ is contained on the positive side of $H_k$, thus $H_j$ separates $H_k$ from the origin. 
\end{proof}

Domination has some simple consequences for fixed points. For instance, if any neuron $k$ strongly dominates $j$, $j$ is not contained within any fixed point support. For a more thorough account of how domination constrains fixed points, see  \cite{curto2019fixed}.
We now turn to the easiest constraints on dynamic attractors provided by domination. 


\begin{prop}\label{prop:supersource}
If $i$ is a proper source in $G$, and $i\to j$ for all vertices $j$, then $\lim_{t\to\infty} x_i(t) = 0$. 
\end{prop}

\begin{proof}
Since $i$ is a proper source in $G$, and $i\to j$ for all $j\in [n]$, for any $j \in [n]$, $j$ strongly dominates $i$. Thus, $H_i$ separates all other $H_j$ from the origin. Thus, $H_i$ is the lower boundary of $\cA$. Thus, by Proposition \ref{thm:mixed_sign}, all trajectories approach the negative side of $H_i$. Any trajectory must either eventually cross $H_i$, or approach a fixed point on $H_i$. Since $i$ is proper source, it is not contained in any fixed points, to if a trajectory is approaching a fixed point, $\lim_{t\to\infty} x_i(t) = 0$. Otherwise, once our trajectory crosses $H_i$ at time $T$, for all $t >T$, $x_i' \leq 0$. Thus, since the quantity $x_i$ is monotonic, it approaches a fixed value. Thus, the trajectory must approach the $i^{th}$ nullcline. It cannot approach the interior of the nullcline $H_i$, thus it must approach $E_i$. Therefore, $\lim_{t\to\infty} x_i(t) = 0$.
\end{proof}

\begin{prop}\label{prop:supersink}
If $i$ is a proper sink in $G$, and $j\to i$ for all $j\in [n]$, then $\lim_{t\to\infty} x_i(t) = \theta$ and $\lim_{t\to\infty} x_j(t) = 0$ for all $j\neq i$. 
\end{prop}

\begin{proof}
Since $i$ is a proper sink in $G$ and $i$ receives an edge from every other neuron, $i$ dominates all other neurons $j\in [n]$. Thus, $H_j$ is separated from the origin from each $H_i$. Therefore, $H_i$ forms the outer boundary of $\cA$. Thus, by Proposition \ref{thm:mixed_sign}, all trajectories approach the positive side of $H_i$. Any trajectory must either eventually cross $H_i$, or approach a fixed point on $H_i$. Either way, the value of $x_i$ must approach a fixed value. Since $i$ dominates all other neurons, the only fixed point support of this network is the singleton set $\{i\}$. Thus, in this case $\lim_{t\to\infty} x_i(t) = \theta$ and  $\lim_{t\to\infty} x_j(t) = 0$ for all $j\neq i$. 
 
\end{proof}

 


%%%%%%%%%%%%%%%%%%%%%%%%% Dynamic domination  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Dynamic domination relationships}

While Propositions \ref{prop:supersource} and \ref{prop:supersink} demonstrate that the purely combinatorial property of graphical domination has dynamic consequences, they only apply in extremely restrictive cases. In this next section, we show that domination has further-reaching consequences. We prove several results that show that domination relationships between the neurons $j$ and $k$ have consequences for the relationship between activity levels $x_j(t)$ and $x_k(t)$ over the long run. In order to do this, we must first prove the following lemma about threshold nonlinearities. 
\begin{lem}\label{lem:thresh_ineq}
Let $a \leq 0$. If $a \leq x - y$, then $a \leq [x]_+ - [y]_+$. Further, these inequalities can be made strict: if $b < 0$, $b < x - y$, then $b < [x]_+ - [y]_+$.
\end{lem}
\begin{proof}
We consider four cases:
\begin{itemize}
\item Case 1: $x \geq 0$ and $y \geq 0$. Then 
\begin{align*}
a \leq x- y = [x]_+ - [y]_+\\
b < x- y = [x]_+ - [y]_+
\end{align*}
\item Case 2: $x \geq 0$ and $y < 0$. Then 
\begin{align*}
a \leq 0 \leq [x]_+ = [x]_+ - [y]_+\\
b < 0 \leq [x]_+ = [x]_+ - [y]_+
\end{align*}
\item Case 3: $x < 0$ and $y \geq 0$. Then 
\begin{align*}
a \leq x - y < [x]_+ - [y]_+\\
b < x - y < [x]_+ - [y]_+
\end{align*}
\item 
Case 4: $x < 0$ and $y < 0$. Then 
\begin{align*}
a \leq 0 = [x]_+ - [y]_+\\
b <0 = [x]_+ - [y]_+
\end{align*}
\end{itemize}
\end{proof}
\begin{prop}[Weak domination] \label{prop:weak_dom}
If $k$ weakly dominates $j$, then if $x_k(T) \geq x_j(T)$, then $x_k(t) \geq x_j(t)$ for all $t \geq T$. 
\end{prop}

\begin{proof}
We show that if $k$ weakly dominates $j$, it not possible to cross from the $x_k > x_j$ side of the hyperplane $x_k = x_j$ to the $x_j > x_k$ side. To do this, we show that if 
$x_j = x_k$, then $x_k '- x_j' > 0$. We have 
\begin{align*}
x_k' - x_j' = -x_k + x_j + \left[\sum_{i = 1}^{n} W_{ki}x_i + \theta \right]_+ - \left[\sum_{i = 1}^{n} W_{ji}x_i + \theta \right]_+.
\end{align*}
Since $x_j = x_k$, 
\begin{align*}
x_k' - x_j' = \left[\sum_{i = 1}^{n} W_{ki}x_i + \theta \right]_+ - \left[\sum_{i = 1}^{n} W_{ji}x_i + \theta \right]_+.
\end{align*}
Now, since the threshold nonlinearity if a monotone transformation, 
\begin{align*}
0 \leq \left[\sum_{i = 1}^{n} W_{ki}x_i + \theta \right]_+ - \left[\sum_{i = 1}^{n} W_{ji}x_i + \theta \right]_+ 
\end{align*}
if and only if 
\begin{align*}
0 \leq 
\left(\sum_{i = 1}^{n} W_{ki}x_i + \theta \right) - \left(\sum_{i = 1}^{n} W_{ji}x_i + \theta \right).
\end{align*}
We have 

\begin{align*}
\left(\sum_{i = 1}^{n} W_{ki}x_i + \theta \right) - \left(\sum_{i = 1}^{n} W_{ji}x_i + \theta \right) = 
\sum_{i \neq j, k}^{n} (W_{ki}-W_{ji})x_i  + W_{kj} x_j -  W_{jk}x_k.
\end{align*}
Because $k$ weakly dominates $j$, $(W_{ki}-W_{ji})\geq 0$ for all $i$, so $\sum_{i \neq j, k}^{n} (W_{ki}-W_{ji})x_i \geq 0$. Because $x_j = x_k$ and because $k$ weakly dominates $j$, $W_{kj} x_j = W_{jk}x_k$. 
Thus
\begin{align*}
0\leq\sum_{i \neq j, k}^{n} (W_{ki}-W_{ji})x_i  + W_{kj} x_j -  W_{jk}x_k
\end{align*}
as desired.  
\end{proof}

\begin{cor}[Equal input]\label{cor:equal_input}
If $x_k$ and $x_j$ are equal input, then if $x_k(T) > x_j(T)$, then $x_k(t) > x_k(t)$ for all $t > T$. If $x_k(T) = x_j(T)$, then $x_k(t) = x_k(t)$ for all $t > T$.
\end{cor}

\begin{proof}
If $j$ and $k$ are equal-input, then $j$ weakly dominates $k$ and $k$ weakly dominates $j$. Thus, if  $x_k(T) \geq x_j(T)$, then $x_k(t) \geq x_j(t)$ for all $t > T$. If $x_k(T) = x_j(T)$, then $x_k(T) \geq x_j(T)$ and $x_k(T) \leq x_j(T)$, so by Proposition \ref{prop:weak_dom}, $x_k(t) \geq x_j(t)$ and $x_k(t) \leq x_j(t)$ for all $t \geq T$, so $x_k(t) = x_j(t)$ for all $t \geq T$. 
\end{proof}

 
\begin{prop}[Strong domination]
\label{prop:strong_dom}
If $k$ strongly dominates $j$, then for all $\eta > 0$, there exists some $T_\eta \geq 0$ such that for all $t \geq T_\eta$, $x_k(t) +\eta > x_j(t)$. \end{prop}

\begin{proof}
We prove that if $x_j > x_k$, then $x_k' - x_j' > 0$. By Observation \ref{obs:strong_domination}, we have $h_k^*(x) > h_j^*(x)$ within the positive orthant. 
Now, we apply Lemma \ref{lem:thresh_ineq} to show that this still holds once we apply the threshold nonlinearity: 
\begin{align*}
h_k^*(x)  -h_j^*(x)  &=  -x_k + y_k +  x_j - y_j \geq 0\\
x_k - x_j &\geq  y_k - y_j \\
x_k - x_j &\geq [y_k]_+ - [y_j]_+\\
x_k' - x_j'&\geq 0
\end{align*}
whenever $x_j  \geq x_k$. Further, this inequality can be made strict whenever $x_j > x_k$, since in this case, we must have $h_k^*(x)  -h_j^*(x) > 0$. 


Now, we use this to prove the desired result. First, suppose that the trajectory starting at the point $x(0)$ has $x_k(T) \geq  x_j(T)$ at some time $T$. Then by Proposition \ref{prop:weak_dom} $x_k(t) \geq  x_j(t)$ for all time $t \geq T$. Thus, we can take $T_\eta= T$ for all $\eta > 0$. 

Now, suppose this does not happen, and that $x_k(t) <  x_j(t)$ for all $t \geq 0$. Then $x_k'(t) - x_j'(t) > 0$ for all $t\geq 0$. Thus, the quantity $x_k(t)-x_j(t)$ is monotonically increasing, and must thus approach a limit. This limit must be $x_k(t)-x_j(t) = 0$, since when $x_k(t) < x_j(t)$, $\xdot_k(t) -\xdot_j(t) >0$. Thus for all $\eta > 0$, there exists some $T_\eta \geq 0$ such that for all $t \geq T_\eta$, $x_k(t) +\eta > x_j(t)$.
\end{proof}


\subsection{General Local Lyapunov Functions}

The main idea in our proof of Proposition \ref{prop:strong_dom} is an example of something we will call a \emph{local Lyapunov function}. 
Lyapunov functions are typically used to show that all trajectories of a dynamical system approach a specified fixed point, conventionally taken to be the origin. Here, we generalize this style of argument by introducing local Lyapunov-like functions. We will use these to show that all trajectories which enter a region $B$ approach a smaller region $A$, as illustrated in Figure \ref{fig:llf}. 


\begin{figure}[ht!]
\begin{center}
\includegraphics[width = 2.5 in]{ThresholdLinear/Figures/local_lyapunov.pdf}
\end{center}
\caption{If $L$ is a local Lyapunov function for $A$ and $B$, then all trajectories which enter $B$ must approach $A$. \label{fig:llf}}
\end{figure}
 
\begin{defn}Let $A\subseteq B\subseteq \R^n$ be compact sets, and $\xdot = g(x)$ be a dynamical system on $\R^n$.  A continuous,continuously differentiable function $L: B \to \R$ is a \emph{local Lyapunov-like function} for the pair $A, B$ if it satisfies the following: 
\begin{enumerate}
\item  $\dot{L} < 0$ on $B\setminus A$.
\item $L > 0$ on $B\setminus A$.  
\item $L\leq 0$ on $A$. 
 \end{enumerate} 
\end{defn}

For instance, our proof of Proposition \ref{prop:strong_dom} established that the $L(x) = x_j - x_k$ is a local Lyupanov function for $B = \cA$, $A = \cA \cap \{ x \mid x_k \geq x_j\}$. 

\begin{lem}
If $L$ is a local Lyapunov-like function for $A,B$, then any trajectory which remains in $B$ for all time approaches $A$. 
\end{lem}

\begin{proof}
Let $x_0\in B$. By assumption, the trajectory $x(t)$ with this  initial condition remains in $B$ for all $t\geq 0$. Now, suppose $x(t)$ does not ever enter $A$. Then $\dot L < 0$ for all time. This means that the value $L(x(t))$ is monotonically decreasing, so it must approach a limit as $t\to \infty$. This means that $\dot L(x(t)) \to 0$ as $t\to \infty$. Since the only place within $B$ where it is possible that $\dot L = 0$ is $A$, the trajectory must approach $A$. 

Now, suppose the trajectory enters $A$. We show that it must stay there. Since $\dot L  < 0$ on $B\setminus A$, by continuity of $\dot L $ we have $\dot L \leq 0$ on $\partial A$. Thus, if the trajectory were to cross out of $A$, the value of $L$ must decrease as we cross out. However, since $L \leq 0$ on $A$ and $L > 0$ on $B$, this is not possible. 
\end{proof}

\section{Main results: CTLNs}

In this section, we work towards a proof of the following result, which has Theorems \ref{thm:dag} and \ref{thm:dag_onto_symmetric} as consequences. 


\begin{thm}
\label{thm:sources_die}
Let $G$ be a graph in which every vertex is reachable from a source. Then there is a source $j$ in $G$ such that $\lim_{t\to \infty} x_j(t) = 0$. 
\end{thm}

We begin by giving an informal summary of our argument. 
First, we prove that if $j$ is a source, and if $x_j \leq x_k$ for all other neurons $k$, then $\lim_{t\to \infty} x_j = 0$ (Lemma \ref{lem:smallest_sources_die}). We do this by showing that  within this set, the nullcline $H_j$ forms the lower boundary of the mixed-sign chamber (Figure \ref{fig:sources_die_arg} A), thus trajectories are trapped on the negative side of $H_j$. Thus once trajectories are trapped in this region, $\lim_{t\to  \infty}x_j$. 

\begin{figure}
\includegraphics{ThresholdLinear/Figures/sources_die_arg.pdf}
\caption{A) Within the region where the source numbered 1 is the smallest, the nullcline $H_1$ separates the other nullclines from the origin. B) We number our neurons along paths from the smallest source. C) The regions $\Omega_{1\ell}$ and $\Omega_{13}$. D) Our local Lyapunov functions.  \label{fig:sources_die_arg}}
\end{figure}

Next, we show that this condition is eventually satisfied for the smallest source: the source $j$ which has the $x_j \leq x_\ell$ for all other sources $\ell$ at our initial condition.
We show this using local Lyapunov functions for a nested sequence of sets $\Omega^{G}_1\supseteq \Omega^G_{2}\supseteq \cdots \supseteq\Omega^G_{n}$. These sets are defined by renumbering the neurons along paths from the source (Figure \ref{fig:sources_die_arg} B), and then requiring the activity of the source to be lower than that of other neurons along this path (Figure \ref{fig:sources_die_arg} C). Finally, we show that the function $L_\ell = x_j - x_\ell$ is a local Lyapunov function for the sets $A = \Omega^{G}_\ell$ and 
 $B =\Omega^{G}_{\ell -1}$. This means that trajectories get in $\Omega^{G}_{\ell -1}$ go towards $ \Omega^{G}_\ell$. Thus, trajectories must eventually enter the set where $x_j \leq x_{\ell}$ for all vertices $\ell$ reachable from $j$. 
This must also happen for every other source $i$. Thus, since $x_j$ is the smallest source, we must eventually have $x_j\leq x_i \leq x_\ell$ if $\ell$ is reachable from some other source $i$. Therefore, we must eventually enter the set where $x_j\leq x_\ell$ for all other neurons $\ell$. Thus, by Lemma \ref{lem:smallest_sources_die}, $\lim_{t\to \infty} x_j = 0$. 
Finally, the value of $x_j$ must become so low that its influence on the other neurons may be neglected. Thus, we let some other source take over as the smallest source. In this way, we show that the activity of all sources must decay to zero. 

In order to apply this result inductively in order to prove Theorems \ref{thm:dag} and \ref{thm:dag_onto_symmetric}, we wish to eventually neglect the activity of sources which have ``died". Thus, we will need to prove our results in a way which has some threshold for negligible activity which we allow ourselves to neglect. When we are proving Theorems \ref{thm:dag} and \ref{thm:dag_onto_symmetric} by induction, we will modify our graph by ignoring neurons whose activity is approaching zero. We will also need to deal with the fact that, if we have a local Lyapunov function for $A$ and $B$, this only guarantees that trajectories which remain in $B$ \emph{approach} $A$, not that they actually enter it. We handle both of these issues through our definition of $\Omega^{G}_\ell(\alpha, \beta)$. 

\begin{defn}\label{def:order_omega}
Let $G$ be a graph with vertices $V_G$. Let $L\subseteq V_G$.  Let $j$  be a particular source in $G|_L$.  Renumber the vertices in $L$ as follows: 
First, partially order the vertices by $k \leq_j \ell$ if the shortest path from $j$ to $k$ is shorter than the shortest path from $j$ to $\ell$, setting this length to be $\infty$ if $\ell$ is not reachable from $j$. Then, pick a linear extension of this order. Notice that under this order, we have labeled $j = 1$. Now, we can define
\begin{align*}
\Omega^{G_L}_\ell  &= \{x \mid x_j \leq x_k \mbox{ for all } k \leq \ell, k\in L, x_k = 0 \mbox{ for all } k \notin L\}\\
\Omega^{G_L}_\ell (\alpha, \beta) & = \{x \mid x_j \leq x_k + \alpha \mbox{ for all } k \leq \ell, k\in L, x_k \leq \beta, |\xdot_k|\leq \beta \mbox{ for all } k \notin L\}
\end{align*}
When $L = V_G$, we drop the parameter $\beta$, writing 
\begin{align*}
\Omega^{G_L}_\ell (\alpha) & = \{x \mid x_j \leq x_k + \alpha \mbox{ for all } k \leq \ell\}.
\end{align*}
\end{defn}

Notice that $\Omega^{G_L}_{|L|}$ is the set where the source numbered 1 has $x_1 \leq x_\ell$ for all $\ell \in L$, and $x_\ell = 0$ for all $\ell \notin L$. Our first lemma establishes that ``smallest sources die": if a trajectory stays in the set $\Omega^{G_L}_{|L|}$ where the source 1 is the neuron with lowest activity, then $x_1$ approaches zero. We prove a stronger result, that this holds on $ \Omega^{G_L}_{|L|}(\eta, \zeta)$ for some positive values of $\eta$ and $\zeta$.
 
\begin{lem}\label{lem:smallest_sources_die}
Let $L \subseteq V_G$ be our set of active neurons. Assume the neurons are numbered according to Definition \ref{def:order_omega} such that neuron 1 is a source in $G|_L$. Then there exist $\eta, \zeta > 0$ such that if $x \in \Omega^{G_L}_{|L|}(\eta, \zeta)$ for all $t \geq T$, then $\lim_{t\to \infty} x_1(t)= 0$. 
\end{lem}

%To motivate this claim, we first sketch the proof of an easier version with $\eta = 0$. Then we have $x_j \leq x_k$ for all $k$. By Proposition \ref{prop:weak_dom}, once $x_j \leq x_k$ at some time $T$,  $x_j \leq x_k$ for all $t > T$. Further, within the region where  $x_j \leq x_k$, the hyperplane $H_j$ forms the lower boundary of the mixed-sign chamber, separating all other hyperplanes $H_j$ from the origin. Thus, the entire mixed-sign chamber is contained on the negative side of $H_j$, so the value of $x_j$ must approach zero. Much of the work in the next proof goes into showing this argument can also be made to work for a positive $\eta > 0$. 

\begin{proof}

We first describe the value of $\eta$ and $\zeta$. If $1$ is a proper source, there are no fixed points on the set $ C := H_1\cap \R^n_\geq$, so $||\xdot||_1> 0$ on $H_1 \cap \R^n_\geq$. If $1$ is an isolated vertex, then the only fixed point $x^*$ on $H_1$ has support $\{1\}$, and therefore is separated from $\Omega^{G_L}_{|L|}$ by a positive distance $d$. Thus, $||\xdot||_1> 0$ on the compact set  $C := H_1\cap \R^n_\geq \setminus B_d(x^*)$ we get by deleting a $d$-neighborhood of this fixed point $x^*$.  Thus the continuous function $||\xdot||_1$ attains its minimum value on $C$. Therefore there exists some positive $\alpha > 0$ such that  $||\xdot||_1 \geq \alpha > 0$ on $C$. Let $\eta  = \frac{\alpha}{4n\delta }$. Let $\zeta = \delta \eta$. 

We first focus on the neurons in $L$ and show that if $x_1(T) < x_k(T) +\eta $ for some $T$, then $x_1'(t) \leq 0$ for all $t \geq T$. Thus $\lim_{t\to \infty}x_1(t) = 0$. For all $k$ such that $1\not \to k$,
\begin{align*}
h_k^*(x(t)) - h_1^*(x(t)) &= -x_k + x_1 +  (-1-\delta)x_1 - (-1-\delta)x_k + \sum_{i\neq 1, k} (W_{ki} - W_{1i})x_i  \\
h_k^*(x(t)) - h_1^*(x(t)) &= \delta(x_k - x_1) + \sum_{i\neq 1, k} (W_{ki} - W_{1i})x_i \\
h_k^*(x(t)) - h_1^*(x(t)) &\geq -\delta \eta. 
\end{align*}
Now, for $x(t)\in H_1 \cap \R^n_\geq$, $h_1^*(x(t)) = x_1'(t) = 0$. For all $x(t)$, $h_k^*(x(t)) \leq \xdot_k(t)$. Therefore, for $x(t)\in H_1 \cap \R^n_\geq$,
\begin{align*}
x_k'(t)  &\geq -\delta \eta. 
\end{align*}
If $1 \to k$, then the entirety of $H_1 \cap \R^n_\geq$ is contained on the positive side of $H_k$, so on $H_1 \cap \R^n_\geq$, 
\begin{align*}
\xdot_k(t)  \geq 0 \geq -\delta \eta\\ 
\xdot_k(t) \geq -\delta \eta. 
\end{align*}
Now, we note that this is also satisfied  by requirement for  the neurons outside $L$. 

Now, we show that it is only possible to cross the $H_1$ hyperplane from the positive to the negative side. We do this by showing that the dot product of $ \xdot(t)$ with the normal vector to $H_1$ is always negative. 
We have 
\begin{align*}
\sum_{i = 1}^n \xdot_i(t) = \sum_{x_i(t)\geq 0}\xdot_i(t) + \sum_{\xdot_i(t)< 0}\xdot_i(t) = \sum_{i = 1}^n | \xdot_i(t)| + 2 \sum_{x_i(t)< 0}\xdot_i(t) = ||\xdot(t)||_1+ 2 \sum_{x_i(t)< 0}\xdot_i(t).
\end{align*}
Since $\xdot_k(t)   \geq -\delta \varepsilon$ for all $k$,
\begin{align*}
2 \sum_{x_i(t)< 0}\xdot_i(t) \geq -2n\delta\varepsilon = -2n\delta \frac{\alpha}{4n\delta} = -\frac{\alpha}{2}.\\
\end{align*}

Thus 
\begin{align*}
\sum_{i = 1}^n \xdot_i = ||\xdot||_1+ 2 \sum_{x_i< 0}\xdot_i \geq \frac{\alpha}{2}  > 0.
\end{align*}
Now, recall that the normal vector to $H_i$ is $(-1, -1-\delta,-1-\delta, \ldots,  -1-\delta)$.  Thus, since $\xdot_1 = 0$ on $H_1\cap \R^n_\geq$, 
\begin{align*}
\xdot(t)\cdot h_1 = (-1-\delta)\sum_{i = 1}^n \xdot_i(t) < 0. 
\end{align*}
Thus, trajectories can only cross from the positive side to the negative side of $H_1$. Thus, the value of $x_1(t)$ eventually becomes monotone, and thus must approach a limit. This means the trajectory must approach the $x_1$ nullcline. The trajectory cannot approach $H_1$ because if $c\in  H_1$, $\xdot(t)\cdot h_1< 0$. Thus, the trajectory must approach $E_1$, so  $\lim_{t\to \infty}x_1(t) = 0$.

\end{proof}

Now, we show that the conditions of Lemma \ref{lem:smallest_sources_die} are ultimately achieved for some source, i.e.  for some source, $ \Omega^{G_L}_{|L|}$ is an attracting set. In particular, we show this for the smallest source, i.e. the source neuron $j$ such that $x_j \leq x_\ell$ for all other \emph{sources} $\ell$. 
We will prove by induction using this order that if $k$ is reachable along a path from a source $j$, then eventually $x_j  < x_k  + \eta$. We do this using local Lyapunov functions for a nested sequence of sets. 


\begin{lem}\label{lem:lyapunov} For any $\beta > 0$, the function $L_\ell = x_j - x_{\ell} + \beta$ is a local Lyapunov function for 
$B = \Omega^{G_L}_{\ell}(\beta, \zeta)$ and  $A =\Omega^{G_L}_{\ell-1}(\alpha, \zeta)\cap B$ for $\beta = \frac{ \alpha\epsilon}{2(\epsilon + \delta)}$ and $\zeta = \frac{\epsilon \alpha}{2n(\epsilon + \delta)}$. 
\end{lem}

\begin{proof}
By construction, we have $ L_\ell \leq 0$ on $A$ and $L_\ell > 0$ on $B \setminus A$.  
Now, we show that $\dot L_\ell <0$ on $B\setminus A$. 
We consider 
\begin{align*}
\dot L_\ell = \xdot_j - \xdot_\ell = -x_j + x_\ell + \left[\sum_{i=1}^n W_{ji}x_i + \theta \right]_+ - \left[\sum_{i=1}^n W_{\ell i}x_i + \theta\right]_+. 
\end{align*}
By Lemma \ref{lem:thresh_ineq}, when $x_j \geq x_k$
\begin{align*}
\xdot_j - \xdot_\ell &\leq -x_j + x_\ell + \left( \sum_{i=1}^n W_{ji}x_i + \theta\right)  - \left(\sum_{i=1}^n W_{\ell i}x_i + \theta \right)_+\\
\xdot_j - \xdot_\ell &\leq -x_j + x_\ell + \sum_{i=1}^n (W_{ji}-W_{\ell i})x_i \\
\xdot_j - \xdot_\ell &\leq (-1 - W_{\ell j})x_j + (1 + W_{j\ell})x_\ell + \sum_{i \in L\setminus \{j, \ell\}  }(W_{ji}-W_{\ell i})x_i + \sum_{k \notin L }(W_{ji}-W_{\ell i})x_k
\end{align*}
Now, since $j$ is source in $G|_L$, $(W_{ji}-W_{\ell i}) \leq 0$ for each neuron $i \in L\setminus \{j, \ell\} $. 
 Further, $1 + W_{j\ell} = -\delta \leq 0$.  
 Since $x\in B$, the total activity of the neurons outside $L$ is bounded above, thus $ \sum_{k \notin L }(W_{ji}-W_{\ell i})x_k \leq  2n(\epsilon + \delta) \frac{\epsilon \alpha}{2n(\epsilon +\delta)} = \frac{\epsilon \alpha}{2}$.  
 
Now, we consider two cases, if $\ell$ recieves an edge directly from $j$ or not. In the fist case,  then  $(-1 - W_{\ell j})  = -\epsilon <0$, so 
$$\xdot_j - \xdot_\ell \leq -\epsilon x_j + \frac{\epsilon\alpha}{2}.$$
Since $x_j \geq \alpha$ in $B\setminus A$, we have 
 $\xdot_j - \xdot_\ell \leq 0$ whenever $x_j \geq x_k$, thus $\dot L < 0$ on $B\setminus A$. 

Next, if $\ell$ does not receive an edge directly from $j$, by our ordering of neurons, we have that $\ell$ does receive an edge from some neuron $k < \ell$. For $x\in B$, we have $x_j \leq x_k + \beta$. We pull the $k^{th}$ term out of the summation in the right hand side, 
rewriting it as 
\begin{align*}
\xdot_j - \xdot_\ell &\leq (-1 - W_{\ell j})x_j + (1 + W_{j\ell})x_\ell + (W_{jk} - W_{\ell k})x_k  + \sum_{i\neq j, k,\ell \in L}(W_{ji}-W_{\ell i})x_i + \frac{\epsilon\alpha}{2}\\
\xdot_j - \xdot_\ell &\leq \delta x_j - \delta x_\ell  - (\delta + \epsilon)x_k  +\sum_{i\neq j, k,\ell \in L}(W_{ji}-W_{\ell i})x_i + \frac{\epsilon\alpha}{2}\\
\end{align*}
We can drop the terms $ - \delta x_\ell$ and $\sum_{i\neq j, k,\ell \in L}(W_{ji}-W_{\ell i})x_i$, as they are guaranteed to be non-positive, obtaining the bound 
\begin{align*}
\xdot_j - \xdot_\ell &\leq \delta x_j  - (\delta + \epsilon)x_k + \frac{\epsilon\alpha}{2}.
\end{align*}
Now, for $x\in B$, we have $x_j \leq x_k + \beta$, so 
\begin{align*}
\xdot_j - \xdot_\ell &\leq \delta x_j  - (\delta + \epsilon)(x_j - \beta)+ \frac{\epsilon\alpha}{2}\\
\xdot_j - \xdot_\ell &\leq -\epsilon x_j  + (\delta + \epsilon)\beta + \frac{\epsilon\alpha}{2}.
\end{align*}
Now, for all $x\notin A$, we have $x_j \geq x_k + \alpha \geq \alpha$, thus-
\begin{align*}
\xdot_j - \xdot_\ell &\leq -\epsilon \alpha + (\delta + \epsilon)\beta + \frac{\epsilon\alpha}{2}= 0,
\end{align*}
as desired. 
\end{proof}



\begin{lem}\label{lem:source_becomes_smallest_1}
Let $L \subseteq V_G$ be our set of active neurons,  numbered according to Definition \ref{def:order_omega} such that neuron 1 is a source in $G|_L$. Let $\ell$ be a vertex which is reachable from $1$ along a directed path. Then for each $\eta \geq 0$, there exists some  $T \geq 0$ and some $\zeta> 0$ such that if $x_k(t), |\xdot_k(t)| \leq \zeta$ for all  time $t$ and all inactive neurons $k\notin L$ such that $x(t) \in \Omega_\ell^{G|_L}(\eta, \zeta)$ for all $t \geq T$. 
\end{lem}

\begin{proof}
We prove this by induction, with the vertices labeled according to Definition \ref{def:order_omega}. If $\ell = 1$ this result is trivially true. 

Now, we assume as an inductive hypothesis that this result holds for all vertices $k < \ell$, and show that it must hold for $\ell$.  Then by Lemma \ref{lem:lyapunov}, we have that there is a local Lyapunov function $L$ for $B = \Omega_{\ell-1}^{G|_L}(\eta/2, \zeta)$ and  $A =\Omega_\ell^{G|_L}(\beta, \zeta)\cap B$ for $\beta = \frac{ \eta\epsilon}{2(\epsilon + \delta)}.$ Now, by the inductive hypothesis, there exists a time $T'$ such that $x(t) \in B$ for all $t \geq T'$. Thus, all trajectories must enter and remain in $B$, so they approach $A$. Thus, after some time $T$ all trajectories must actually enter and become trapped in the set  $\Omega_\ell^{G|_L}(\eta, \zeta)$. 
\end{proof}

Now, we have shown that each source eventually becomes (approximately) smaller than all vertices which are reachable from it. However, to apply Lemma \ref{lem:smallest_sources_die}, we need to show the source eventually becomes  (approximately) smaller than \emph{all} active neurons. 

\begin{lem}\label{lem:smallest_source_becomes_smallest}
Let $L \subseteq V_G$ be our set of active neurons,  numbered according to Definition \ref{def:order_omega} such that neuron 1 is a source in $G|_L$. Suppose $x_1(0) < x_k(0)$ for all other sources $k$ in $G|_L$. Then for each $\eta \geq 0$, there exists $\zeta> 0$ such that if $x_j \leq \zeta$ for all $j\notin L$ and $T \geq 0$ such that $x(t) \in \Omega_\ell^{G|_L}(\eta, \zeta)$ for all $\ell \in L$, $t \geq T$. 
\end{lem}

\begin{proof}
By assumption, every vertex $\ell$ is reachable from some source $k$ along a directed path.  Thus by numbering the vertices according to Definition  \ref{def:order_omega} such that $k$ is sent to $1$, we can apply Lemma  \ref{lem:source_becomes_smallest_1}, to show that exists a time $T_{k\ell}$ such that $x_k \leq x_\ell + \eta$ for all $t\geq T_{k\ell}$. Now, since  $x_1(0) < x_k(0)$ for all other sources $k$, there is some $\zeta$ such that if  $x_j \leq \zeta$ for all $j\notin L$, the order of $x_1$ and $x_k$ cannot switch, thus $x_1$ will remain smaller than $x_k$ for all other sources $k$. Thus, by taking $T \geq T_{k\ell}$ for each vertex $\ell$ and source $k$, we have that 
$x_j \leq x_j \leq x_\ell + \eta$  for each vertex $\ell$. Thus, for  $t \geq T$, we have  $x(t) \in \Omega_\ell^{G|_L}(\eta, \zeta)$, as desired. 
\end{proof}

Finally, we are ready to prove Theorem \ref{thm:sources_die}. 

\begin{proof}
Let $G$ be a graph for which every vertex is reachable from a source, and consider a CTLN with graph $G$. Let $j$ be the source in $G$ which satisfies $x_j \leq x_k$ for all other sources  at the initial condition. By Lemma \ref{lem:smallest_source_becomes_smallest}, there exists a time $T$ such that $x\in \Omega_\ell^{G}(\eta)$ for all neurons $\ell$ and the values of $\eta$ an used in Lemma \ref{lem:smallest_sources_die}. Therefore, $\lim_{t\to\infty} x_{j} = 0$. 
\end{proof}

Now, we use this result to prove Theorems \ref{thm:dag} and \ref{thm:dag_onto_symmetric}. The first part of our proof is to show that, in the case of a DAG, all neurons other than the sinks have their activity approach zero, and in the case of a symmetric graph, all neurons outside the symmetric part have their activity approach zero. We prove this for a more general family of graphs, which we define below. 

\begin{defn} 
Let $G$ be a graph and $\omega, \tau \subseteq V_G$. We say that $(\omega, \tau)$ is an \emph{inductively stable DAG decomposition} of $G$ if  $\omega \sqcup \tau$ is a partition of the vertices of $G$ satisfying the following inductive definition  
\begin{enumerate}
\item $G|_\omega$ is a DAG
\item $G|_\tau$ contains all sinks of $G$ 
\item there are no edges from $\tau$ back to $\omega$ 
\item every vertex of $\tau$ is reachable along a directed path from a vertex in $\omega$. 
\item for any source $i\in \omega$, $\omega \setminus \{i\}, \tau$ is an inductively stable DAG decomposition of $G|_{V_G\setminus \{i\}}$. 
\end{enumerate}
\end{defn}

\begin{lem}\label{lem:dag_decomp}
Let $G$ be a graph with inductively stable DAG decomposition $( \omega, \tau)$. Then for any $i\in \omega$, $\lim_{t\to \infty}x_i = 0$. 
\end{lem}


\begin{proof}

Let $G$ be a graph with inductively stable DAG decomposition $( \omega, \tau)$. We first prove that every vertex of $G$ is reachable from a source. First, if $i\in \omega$, then a path which follows edges backwards must remain in $\omega$, and must eventually terminate, since $G_\omega$ is a DAG. The vertex where this path terminates must be a source.  Now, by assumption, every vertex in $\tau$ is reachable along a path from a vetex in $\omega$. Thus, from a vertex in $\omega$, we can trace a path backwards into $\tau$, and then back to a source. 

Now, by Theorem \ref{thm:sources_die}, there is some source $i$ of $G$ whose activity must approach zero. Further, for this to be possible, all trajectories of the TLN must approach the $i^{th}$ nullcline. 
Thus we are guaranteed that for each value of $\zeta$, there exists a time $T$ such $x_i(t)\leq \zeta$, and $|\xdot_i(t)| \leq \zeta$ for all $t \geq T$. 
Now, by assumption, $\omega\setminus\{i\}, \tau$ is an inductively stable DAG decomposition of $G|_{V_G\setminus i}$.  
By choosing $\zeta$ small enough, we can satisfy the conditions of Lemmas \ref{lem:smallest_sources_die} and \ref{lem:lyapunov} when restricting to the graph  $G|_{V_G\setminus i}$. 
We can apply this argument inductively to show that for each $i\in \omega$, $\zeta > 0$, there is a time $T$ such that $x_i(t) \leq \zeta$ for all $t\geq T$. Thus, for any $i\in \omega$, $\lim_{t\to \infty}x_i = 0$. 
\end{proof}

Thus, we have shown that whenever $G$ has an inductively stable DAG decomposition $\omega$, $\tau$, all activity of the CTLN on $G$ becomes concentrated on $G|_\tau$. Now, we wish to prove that if $G_|\tau$ is symmetric, then all trajectories of the $CTLN$ on $G$ approach a fixed point. 
In order to prove this, we first prove the following lemma, which allows us to neglect the impact of neurons in $\omega$ upon those of $\tau$ once they have decayed sufficiently. 

\begin{lem}\label{lem:lyapunov_hell}
Let $\xdot = g(x)$ be a dynamical system on a compact set $A$ with a Lyapunov like function $L: A \to \R$ satisfying the following: 

\begin{itemize}
\item $\dot L \leq 0$ for all $x\in A$ 
\item $\dot L = 0$ only on a finite set of fixed points $X = \{x\in A\mid g(x) = 0\}$, 
\item $L$ is bounded below on $A$.  
\end{itemize}

Then for every $\epsilon > 0$, there exists $\delta > 0$ such that if $\dot x = g'(x, t)$ is a dynamical system satisfying $|g(x) - g'(x, t)| < \delta$, then there exists $T$ such that all trajectories of of the system $\dot x = g'(x, t)$ satisfy $|x(t) - X| < \epsilon$ for all $t > T.$


\end{lem}

\begin{figure}
\includegraphics[width = 6 in]{ThresholdLinear/Figures/Lyapunov_horror.pdf}
\caption{(a) The quantity $D(\delta)$. (b) The quantity $\epsilon'(\delta)$. (c) The quantity $E(\delta, x)$.  \label{fig:lyapunov}}
\end{figure}

\begin{proof}
We consider three quantities, $D(\delta)$, $\epsilon'(\delta)$,and $E(\delta)$. First, $D(\delta)$ gives the maximum value of $\int_{t_1}^{t_2} \nabla L(x(t)) \cdot g'(x(t),t)dt$ can assume along trajectories of the system $\xdot = g'(x, t)$  which begin and end in an $\epsilon/2$ neighborhood of $X$, but leave an $\epsilon$ neighborhood of $X$ along the way. We show that $D(\delta)$ approaches a negative limit as $\delta \to 0$. Notice that  
\begin{align*}\int_{t_1}^{t_2} \nabla L(x(t)) \cdot g'(x(t),t)dt \leq (t_2 - t_1)  \max_{x \in A, d(x, X) \geq \epsilon/2} (\nabla L(x(t)) \cdot g(x(t),t)).
\end{align*}
Now, since $\nabla L(x) \cdot g'(x,t)$ attains its negative maximum value $\alpha < 0$ on the compact set $\{x \in A\mid d(x, X) \geq \epsilon\}$ , and  $g'(x, t) \to g(x)$ as $ \delta\to 0$, we must have that  $\max_{x \in A, d(x, X) \geq \epsilon/2} (\nabla L(x) \cdot g'(x,t)) \to \alpha < 0$ as $\delta \to 0$.  Further, any trajectory which begins in an $\epsilon/2$ neighborhood of $X$, leaves an $\epsilon$ neighborhood of $X$, and returns to an  an $\epsilon/2$ neighborhood of $X$ must have length at least $\epsilon$, provided we have chosen $\epsilon$ small enough that all fixed points in $X$ are separated by a distance of at most $\epsilon$.  

Finally, since $g(x)$ is bounded above, so is $g'(x, t)$. Thus for a trajectory of length $\epsilon$, we must have $t_2 - t_1 \geq \epsilon / \max_{x\in A}(|g'(x,t)|)$. This must approach the positive limit $t_2 - t_1 \geq \epsilon / \max_{x\in A}(|g(x)|)$ as $\delta\to 0$. Thus, the product $(t_2 - t_1)  \max_{x \in A, d(x, X) \geq \epsilon/2} (\nabla L(x) \cdot g'(x,t))$ approaches a negative limit at $\delta \to 0$. Thus, so does $D(\delta)$. 

Now, we consider $\epsilon'(\delta)$, which we define as the maximum value of $\epsilon$ such that $ \nabla L(x) \cdot g'(x,t) < 0$ for all $x$ such that $|x - X| \geq \epsilon'$. Again, we have that $\epsilon' \to 0$ as $\delta \to 0$, since $ \nabla L(x) \cdot g'(x,t)\to \nabla L(x) \cdot g(x)$, and  $\nabla L(x) \cdot g(x) < 0$ for all $x\notin X$. Finally, we define 
\begin{align*}E(\delta, x):=\max_{y \in B_{\epsilon'(\delta)}(x)} L(y) - \min_{z \in B_{\epsilon'(\delta)}(x)}  L(z) 
\end{align*}
 Notice that  as $\delta \to 0$, $E(\delta, x) \to 0$ by continuity of $L$. Now, let $$E(\delta) := \max_{x \in X} E(\delta, x).$$ Since we are taking this maximum over a finite set, we also have that $E(\delta) \to 0$ as $\delta \to 0$. 
 
Thus, for $\delta$ small enough, we have $|E(\delta)| < |D(\delta)|$. When this is achieved, we claim that it is impossible for a trajectory to start within $B_{\epsilon'}(X)$, leave  $B_{\epsilon}(X)$, and return to $B_{\epsilon'}(X)$. We choose $\delta$ such that $\epsilon' < \epsilon/2$. Then along any trajectory starts from and returns from  $B_{\epsilon'}(X)$, the value of $L$ must decrease along the trajectory by at least $D(\delta)$. However, since the most the value of $L$ can change within $B_{\epsilon'}(x)$ is $E(\delta) < D(\delta)$, this is not possible. 

Finally, we show that this means that there exists $T$ such that all trajectories of of the system $\dot x = g'(x, t)$ satisfy $|x(t) - X| < \epsilon$ for all $t > T.$ By our definition of $\epsilon'(\delta)$, we have that $ \nabla L(x) \cdot g'(x,t) < 0$ outside of $B_{\epsilon'}(X)$. Thus, since $L$ is bounded below, all trajectories must visit the set $B_{\epsilon'}(X)$. Now, for each particular fixed point $x^*\in X$, it is not possible for a trajectory to leave the set $B_\epsilon(x^*)$ and return to $B_{\epsilon'}(x^*)$. Thus, since there are only finitely many fixed points $x^*$, our trajectory must eventually get stuck in  $B_\epsilon(x^*)$ for one of them. 


\end{proof}



\begin{proof}[Proof of Theorem \ref{thm:dag}]
Let $G$ be a DAG. Let $\tau$ be the set of all sinks of $G$, and $\omega$ be $V_G\setminus\tau$. Notice that this is an inductively stable DAG decomposition of $G$. Then by Lemma \ref{lem:dag_decomp}, $\lim_{t\to \infty}x_i(t) = 0$ for all $i\in \omega$. 
Now, since $G|_\tau$ is symmetric, it has  a Lyapunov-like function $L$ by \cite{hahnloser2000permitted}. 
Therefore, by considering the effect of $x_i, i\in \omega$ as a time varying external input on $x_j, j\in \tau$, by our Lemma \ref{lem:lyapunov_hell}, for each $\eta > 0$, we can find a time $T'$ such that $\{x_j\}_{j\in \tau}$  is contained within an $\eta$ neighborhood of a fixed point of the CTLN defined by $G|_\tau$. 
Thus, as $T\to \infty$, the trajectory approaches a fixed point whose support is contained within $\tau$. 
\end{proof}


\begin{proof}[Proof of Theorem \ref{thm:dag_onto_symmetric}]
Let $G$ be a graph and $\omega, \tau$ a partition of the vertices of $G$ such that $G|_\tau$ is symmetric and connected, $G|_\omega$ is a DAG, and there are no edges from $\tau$ to $\omega$. Then by Lemma \ref{lem:dag_decomp}, $\lim_{t\to \infty}x_i(t) = 0$ for all $i\in \omega$. 
Now, since $G|_\tau$ is symmetric, it has  a Lyapunov-like function $L$ by \cite{hahnloser2000permitted}. 
Therefore, by considering the effect of $x_i, i\in \omega$ as a time varying external input on $x_j, j\in \tau$, by our Lemma \ref{lem:lyapunov_hell}, for each $\eta > 0$, we can find a time $T'$ such that $\{x_j\}_{j\in \tau}$  is contained within an $\eta$ neighborhood of a fixed point of the CTLN defined by $G|_\tau$. 
Thus, as $T\to \infty$, the trajectory approaches a fixed point whose support is contained within $\tau$. 
\end{proof}









\section{Main results: competitive TLNs}
In \cite{curto2019robust}, Curto, Langdon, and Morrison relax the strict CTLN conditions, and investigate how and when the graph $G_W$ constrains the dynamics of a competitive TLN. In particular, they say that a graph $G$ is a \emph{robust motif} if $G$ fully determines $FP(W)$ for all weight matrices $W$ such that $G_W = G$. Their Theorem 1.6 gives a complete characterization of which graphs $G$ are robust motifs. 

\begin{thm}[Theorem 1.6, \cite{curto2019robust}]
 $G$ is a robust motif if and only if one of the following holds:
 \begin{enumerate}
\item $G$ belongs to one of the infinite families DAG1 or DAG2, or
\item  $G$ is one of the four invariant permitted motifs (the singleton, the 2-clique, the independent set of size 2, or the 3-cycle).
\end{enumerate}
\end{thm}

In particular, TLNs in the infinite families DAG1 and DAG2 each have a single fixed point, which is stable. However, the fixed point structure of a dynamical system does not fully determine its activity: in principle, a dynamical system with a unique fixed point which is stable may also have a limit cycle or a chaotic attractor. Thus, we would like to show that the families DAG1 and DAG2 are robust in the following sense:

\begin{conj}\label{conj:dyn_robust}
Let $(W, \theta)$ define a TLN such that $G_W$ is a member of DAG1 or DAG2. Then the unique fixed point is always a global attractor.
\end{conj}

We are not able to prove this conjecture for the full families DAG1 or DAG2. However, we define a smaller infinite family of graphs, \emph{shallow DAG1}, and show that graphs in this infinite family are dynamically robust in this sense. 

\begin{defn}
Let $G$ be a member of DAG1 with source node $s$ and target node $u$. We say $G$ is a member of \emph{shallow DAG1} if  it satisfies the additional property that if $i\to j$, then $i = s$ or $j = u$. 
 That is, if a node $j$ is not the target, then it may only receive input from the source $s$. 
\end{defn}

\begin{figure}[ht!]
\begin{center}
\includegraphics{ThresholdLinear/Figures/dynamic_robust.pdf}
\caption{A graph is a member of shallow DAG1 if only the target receives from a non-source vertex.}
\end{center}
\end{figure}

We prove Conjecture \ref{conj:dyn_robust} in the special case where $G$ is a member of shallow DAG1. 

\begin{thm}\label{thm:dag1global}
Let $G$ be a member of shallow DAG 1, and  $(W, \theta)$ be a TLN with  $G_W = G$.  This TLN has a unique fixed point which is a global attractor. 
\end{thm}

We also prove a second result, that if $G$ is any member of DAG1 and the coefficients are close enough to the CTLN coefficients, then all trajectories of the CTLN approach a fixed point. 

\begin{prop}\label{prop:near_ctln}
Let $G$ be a member of DAG1. There is an open set in $\R^{n\times n}$ containing the CTLN coefficients for $G$ such that if the weight matrix $W$ falls in this set, the TLN has a unique fixed point which is a global attractor. 
\end{prop}

\subsection{Shallow DAG1}

In order to prove Theorem \ref{thm:dag1global},  we generalize shallow DAG1 to a larger family of TLNs using strong domination. In order to do this, we need a notion of strong domination with respect to a set $\sigma\subseteq[n]$.

\begin{defn}
Neuron $k$ strongly dominates neuron $j$ with respect to $\sigma \subseteq [n]$ if $\wt W_{ji} \leq \wt W_{ki}$ for all $i\in \sigma$. 
\end{defn}

\begin{defn} Let $W$ be the weight matrix of a TLN. We say that $W$ satisfies the \emph{shallow DAG1 domination property} if there exist neurons $s$ and $u$ such that the following conditions hold:
\begin{enumerate}
\item  $u$ strongly dominates $s$ with respect to $[n]$
\item  for all $i\notin\{s, u\}$,  $u$ strongly dominates $i$ with respect to $[n]\setminus \{s\}$. 
\end{enumerate}

\end{defn}

\begin{prop}
If $G$ is a member of shallow DAG1, and $G_W = G$, then $W$ satisfies the shallow DAG1 domination property. 
Further, suppose that $G$ is a graph such that $W$ satisfies the shallow DAG1 property whenever $G_W = G$. Then $G$ is a member of shallow DAG1. 
\end{prop}

\begin{proof}
First, suppose $G$ is a member of shallow DAG1. Because $s$ is a source and $u$ is a target, then $W_{ui} >-1$ for all $i\neq u$, and $W_{si} < -1$ for all $i\neq s$. Thus $\wt W_{ui} > \wt W_{si}$ for all $i$, thus $u$ strongly dominates $s$. 
Now, because if $i\to j$, either $i = s$ or $j = u$, we have $W_{ij} < -1$ for all $j\neq s, i$ and $W_{uj} > -1$ for all $j\neq u$. Thus, $\wt W_{uj} > \wt W_{ij}$. 

Now, we show that if $G$ is not a member of shallow DAG1, there is some weight matrix $W$ such that $G = G_W$, but $W$ does not satisfy the shallow DAG1 domination property. If $s$ is not a source, then there is some $i$ such that $i\to s$. Then we can choose $W_{ui}$ such that $W_{ui} <W_{si}$.  Likewise, if $u$ is not a target,  then there is some $i$ such that $i\not \to u$. Then we can choose $W_{ui} < W_{si}$. In both of these cases, we violate the condition that $u$ strongly dominates $s$. 

Now, suppose that there is some $i\neq s$, $j\neq s$ such that $i\to j$. Then $W_{ji} > -1$. Then we can choose $W_{ji} > W_{ui}$, which means that $u$ does not strongly dominate $j$ with respect to $[n]\setminus \{s\}$. 
\end{proof}

We will prove that if a TLN satisfies the shallow DAG1 domination property, it has a unique fixed point which is globally attracting. This means if the graph  $G$ is a member of the shallow DAG1 family, then any TLN with $G_W = G$ has a unique fixed point which is globally attracting. Thus, these graphs are dynamically robust in the sense of Conjecture \ref{conj:dyn_robust}. 

\begin{prop}\label{prop:dag1domglobal}
Let $W$ be the weight matrix of a TLN satisfying the shallow DAG1 domination property. 
Then all activity of the TLN defined by $W$ approaches a stable fixed point at which $u$ is the only active neuron. 
\end{prop}

Notice that this implies Theorem \ref{thm:dag1global}, since all TLNs whose graphs are in DAG1 satisfy the shallow DAG1 domination property. 

%We begin with a simple lemma about strong domination. 
%
%\begin{lem}  \label{lem:strong_domination} 
%If $k$ strongly dominates $j$ with respect to $\sigma$, then 
%$$h_k^*(x) - h_j^*(x) > 0$$
%for all 
%$
%x\in \{\R^n \mid 
% x_i = 0 \mbox{ if } i\notin \sigma, 
%x_i \geq 0 \mbox{ if } i\in \sigma
%\}\setminus\{0\}
%$
%In particular, when $\sigma = [n]$, $h_k^*(x) > h_j^*(x)$ on the entire positive orthant, excluding the origin. 
%\end{lem}
%
%\begin{proof}
%We have 
%
%\begin{align*}
%h_k^*(x) - h_j^*(x)  &= \left(-x_k+ \sum_{i=1}^n W_{ki}x_i  + \theta \right) - \left(-x_j + \sum_{i=1}^n W_{ji}x_{i} + \theta \right) \\
%h_k^*(x) - h_j^*(x)  &= \sum_{i = 1}^n \wt W_{ki}x_i -  \sum_{i = 1}^n \wt W_{ji} x_i  = \sum_{i = 1}^n  (\wt W_{ki} - \wt W_{ji} )x_i 
%\end{align*}
%By the definition of strong domination, all coefficients $\wt W_{ki} - \wt W_{ji} $ of this sum are positive for $i\in \sigma$. Thus  when $ x\in \{\R^n \mid 
% x_i = 0 \mbox{ if } i\notin \sigma, 
%x_i \geq 0 \mbox{ if } i\in \sigma
%\}\setminus\{0\}$, 
%we have $h_k^*(x) - h_j^*(x) < 0 $. 
%
%\end{proof}
%
%This lemma has the following geometric interpretation: if $k$ strongly dominates $j$ with respect to $[n]$, then $H_j \cap H_k \cap \R^n_{> 0} = \emptyset$. Further, $H_k$ is separated from the origin by $H_j$. If  $k$ strongly dominates $j$ with respect to $\sigma$, then $H_k$ is separated from the origin by $H_j$ within the surface where $x_i$ is set to zero for all $i\in [n]\setminus \sigma$.  

\begin{lem}\label{lem:strong_dom_deriv}
If $k$ strongly dominates $j$, then either:
\begin{align*}
\xdot_k  > \xdot_j 
\end{align*}
or

\begin{align*}
y_j < 0,\,\, \xdot_j = -x_j
\end{align*}
\end{lem}

\begin{proof}
We have 
\begin{align*}
\xdot_k - \xdot_j &= -x_k +x_j + [y_k]_+ - [y_j]+\\
\xdot_k - \xdot_j &= h_k^*(x) - h_j^*(x) + ([y_k]_+ -y_k) - ([y_j]_+- y_j) 
\end{align*}
By Observation \ref{obs:strong_domination}, the term $h_k^*(x) - h_j^*(x)$ is always positive. By the definition of the threshold nonlinearity, the term $[y_k]_+ -y_k$ is always positive. Thus, we can only have $\xdot_k - \xdot_j \leq 0$ when the term $[y_j]_+- y_j$  is positive, which occurs when $y_j < 0$, $\xdot_j = -x_j$. 
\end{proof}

The next lemma is main part of the proof of Proposition \ref{prop:dag1domglobal}. 
Essentially, we are showing that for TLNs which satisfy the shallow DAG1 domination property, the function $x_u - x_s$ is a Lyapunov-like function within $\cA$. 
We will use this to show that trajectories which enter $\cA$ must approach a fixed point. 

\begin{lem}\label{lem:lyapanov}
If a TLN satisfies the shallow DAG1 domination property, then $\xdot_u - \xdot_s >  0$ on the interior of  $\cA$, with equality achieved on the boundary of $\cA$ on the set where $\xdot_u = \xdot_s = 0$. 
\end{lem}

\begin{figure}[ht!]
\begin{center}
\includegraphics[width = 4 in]{ThresholdLinear/Figures/robust_4.pdf}
\end{center}
\caption{Linear chambers and nullclines restricted to the $x_s, x_u$ plane. Nullclines are shown in red and blue, boundaries of linear chambers are shown in gray. The surface $\dot{x_s} = \dot{x_u}$ is shown in green.  \label{fig:cham}   }
\end{figure}

\begin{proof}
We prove this statement by considering the surface where $\xdot_u = \xdot_s$, and show that it does not intersect with the interior of $\cA$. Because the equations for $\xdot_s$ and $\xdot_u$ are threshold-linear, the surface  $\xdot_u = \xdot_s$ consists of at most four hyperplanes, one in each linear chamber. The surface $\dot{x_s} = \dot{x_u}$ and the linear chambers are illustrated in two dimensions in Figure \ref{fig:cham}. 

We first consider the case where $y_s\geq 0$, which covers the linear chambers $y_s \geq 0, y_u \geq 0$ and $y_s \geq 0, y_u< 0$. By Lemma \ref{lem:strong_dom_deriv}, we have $\xdot_u > \xdot_s$. 
%We first show that the surface  $\xdot_u = \xdot_s$  does not actually intersect with the chambers $\sum_{i=1}^n W_{ui}x_i + \theta\geq 0,     \,\, \sum_{i=1}^n W_{si}x_i + \theta \geq 0$ or $\sum_{i=1}^n W_{ui}x_i + \theta < 0,     \,\, \sum_{i=1}^n W_{si}x_i + \theta \geq 0$. 
%
%\begin{itemize}
% 
% \item 
% %$++$: 
% 
% $\sum_{i=1}^n W_{ui}x_i + \theta\geq 0,     \,\, \sum_{i=1}^n W_{si}x_i + \theta \geq 0$. \\ 
% In this case, the threshold nonlinearities have no effect, and 
% \begin{align*}
%\xdot_u- \xdot_s &= h_u^*(x) - h_s^*(x)%\xdot_u - \xdot_s &= (-1 - W_{su})x_u +(1+W_{us})x_s +  \sum_{i\neq s,u}^n (W_{ui}-W_{si})x_i 
% \end{align*}
%Because $u$ strongly dominates $s$, by  Lemma \ref{lem:strong_domination} this expression is always positive for all $x\in \R^n_\geq \setminus \{0\}$.   Thus, $\xdot_u-\xdot_s > 0$  within this chamber. 
%
%\item 
%% $-+$: 
%$\sum_{i=1}^n W_{ui}x_i + \theta < 0,     \,\, \sum_{i=1}^n W_{si}x_i + \theta \geq 0$. \\
% In this case, only the threshold nonlinearity for $u$ has an effect, so 
% \begin{align*}
%\xdot_u- \xdot_s &= x_s - x_u  - \sum_{i=1}^n W_{si}x_i -\theta\\
%\xdot_u- \xdot_s&= h_u^*(x) - h_s^*(x)- \left(\sum_{i=1}^n W_{ui}x_i -\theta\right)
% \end{align*}
%Again by Lemma \ref{lem:strong_domination}, the sum of the first four terms  is positive throughout the positive orthant. Where this case applies, the quantity  $\sum_{i=1}^n W_{ui}x_i -\theta$ is negative. 
%Thus $\xdot_u -\xdot_s > 0$ within this chamber as well. 
% \end{itemize}
% 
% 
Thus, the surface  $\xdot_u = \xdot_s$  does not actually intersect either of these chambers or their closures. 

We next consider the region where $y_s < 0$, which covers the chambers $y_s < 0, y_u \geq 0$ and $y_s < 0, y_u < 0$. We let $b\neq s, u$ be some bystander neuron.  We show that the surface where $\xdot_u = \xdot_s$ is strictly confined to the negative side of the $x_b$ nullcline $H_b$. To do this, we consider the quantity $\xdot_u - \xdot_s - \xdot_b$, and show that  $\xdot_u - \xdot_s - \xdot_b > 0$ when  $\xdot_b> 0$. 

Notice that when $\xdot_b > 0$, we must have $y_b > 0$. Thus, 
\begin{align*}
 \xdot_u - \xdot_s - \xdot_b &= -x_u + x_s + x_b + [y_u]_+-[y_s]_+- [y_b]\\
 \xdot_u - \xdot_s - \xdot_b &= -x_u + x_s + x_b + [y_u]_+- y_b\\
  \xdot_u - \xdot_s - \xdot_b &\geq -x_u + x_s + x_b + y_u- y_b\
 \end{align*}
 Now, we expand this to 
    \begin{align*}
\xdot_u-\xdot_s -\xdot_b &= x_b + x_s - x_u + \left(\sum_{i=1}^n W_{ui}x_i +\theta\right)  -\left( \sum_{i=1}^n W_{bi}x_i + \theta\right)\\
\xdot_u-\xdot_s -\xdot_b &= (1 -W_{bs}+W_{us})x_s +(-1-W_{bu})x_u + (1 +W_{ub})x_b + \sum_{i\neq u, s,b}^n (W_{ui}-W_{bi})x_i 
\end{align*}

The coefficients $  (1 -W_{bs}+W_{us})$, $(-1-W_{bu})$, and  $(1 +W_{ub})$  are positive because $u$ strongly dominates $s$ with respect to $[n]$.  The coefficients $(W_{ui}-W_{bi})$ are positive because $b$ strongly dominates $u$ with respect to $[n]\setminus \{s\}$.  Thus, this quantity is positive within the positive orthant.  Thus, when $\xdot_b > 0$, we must also have $\xdot_u - \xdot_s > 0$. This means that the surface where $\xdot_u = \xdot_s$ is contained strictly within the negative side of  $H_b$.  
 
% \begin{itemize}
% \item 
%  $y_u\geq 0,     \,\, y_s< 0$. \\ 
%  In this case, we have 
%  \begin{align*}
% \xdot_u - \xdot_s &= x_s - x_u +\sum_{i=1}^n W_{ui}x_i +\theta \\
%  \end{align*}
%  Now, let $b$ be some ``bystander" neuron, $b\neq s, u$. We show that the surface where $\xdot_u = \xdot_s$ is confined to the negative side of the $x_b$ nullcline $H_b$. Notice that when $\xdot_b > 0$, we must have $\xdot_b = -x_b + \sum_{i=1}^n W_{bi}x_i + \theta$.  Thus when $\xdot_b> 0$, where this case applies, 
%   \begin{align*}
%\xdot_u-\xdot_s -\xdot_b = x_b + x_s - x_u + \left(\sum_{i=1}^n W_{ui}x_i +\theta\right)  -\left( \sum_{i=1}^n W_{bi}x_i + \theta\right)\\
%\xdot_u-\xdot_s -\xdot_b = (1 -W_{bs}+W_{us})x_s +(-1-W_{bu})x_u + (1 +W_{ub})x_b + \sum_{i\neq u, s,b}^n (W_{ui}-W_{bi})x_i 
%\end{align*}
%The coefficients $  (1 -W_{bs}+W_{us})$, $(-1-W_{bu})$, and  $(1 +W_{ub})$  are positive because $u$ is a target and $s$ is a source. The coefficients $(W_{ui}-W_{bi})$ are positive on the assumption that if $b$ is not the target, it only receives from the source $s$. Thus, this quantity is positive within the positive orthant.  Thus, when $\xdot_b > 0$, we must also have $\xdot_u - \xdot_s \geq 0$. This means that the surface where $\xdot_u = \xdot_s$ is contained within the negative side of  $H_b$.  
%\item $\sum_{i=1}^n W_{ui}x_i + \theta < 0.,\,\,   \sum_{i=1}^n W_{si}x_i + \theta < 0$. \\

%In this case, we have 
%
%
%\begin{align*}
%\xdot_u - \xdot_s &= x_s - x_u \end{align*}
%
%Then the surface where $\xdot_s = \xdot_u$ is given by the plane $x_s = x_u$.
% \end{itemize}
% 
% Finally, we look at how these two pieces of $\xdot_s = \xdot_u$ intersect. The piece of the surface $x_s = x_u$ is bounded away from the origin by the piece $ \xdot_u - \xdot_s = x_s - x_u +\sum_{i=1}^n W_{ui}x_i +\theta $. 
%We showed that for every bystander neuron $b$, the piece of the surface  $ \xdot_u - \xdot_s = x_s - x_u +\sum_{i=1}^n W_{ui}x_i +\theta $ is contained on negative side of the $x_b$ nullcline $H_b$. 
%
% This surface is also contained on the closure of the negative side of both the $x_u$ and $x_s$ nullclines $H_u$ and $H_s$. To see this, we again apply Lemma \ref{lem:strong_domination}. However, we to have $\xdot_u = \xdot_s = 0$ along the intersection $H_u \cap E_s$. 

Finally, by Lemma \ref{lem:strong_dom_deriv}, if $\xdot_u = \xdot_s$, then $\xdot_s = -x_s\leq 0$, so we must have $\xdot_u \leq 0$. This means that the surface $\xdot_u = \xdot_s$ is confined to the negative side of $H_u$, but this might not be strict. 
 
Since our bystander neuron was arbitrary, we have shown that within the mixed-sign chamber $\cA$, $\xdot_u \geq \xdot_s$. On the piece of the boundary of the mixed sign chamber made up by $H_u$, we have $\xdot_u = \xdot_s = 0$ along the surface defined by $x_s = 0, -x_u + \sum_{i = 1}W_{ui}x_i +\theta = 0$. 
\end{proof}


Finally, we are ready to prove Proposition \ref{prop:dag1domglobal}. 
\begin{proof}

By Theorem \ref{thm:mixed_sign}, all trajectories approach $\cA$. First, we consider trajectories which do not ever enter $\cA$. Such trajectories remain in either $\cA^+$ or $\cA^-$ for all time. Then along these trajectories, the signs of each derivative $\xdot_i$ are fixed. Thus, for each $i$, the value of $x_i$ approaches a constant. Thus, these trajectories approach a limit, which must be a fixed point. This must be the unique fixed point of the network. 

Next, we consider trajectories which do enter $\cA$. By Lemma \ref{lem:lyapanov}, once the trajectory has entered $\cA$, it is subject to the constraint $\xdot_u - \xdot_s > 0$. Then this trajectory must approach the limit on the boundary of $\cA$ where $\xdot_u = \xdot_s = 0$. On this set, by Lemma \ref{lem:strong_dom_deriv}, $x_s = 0$. Thus, this trajectory must approach the surface where $x_s = 0$. 

Now, by condition (2) of the shallow DAG1 decomposition property, for all $i\notin \{s, u\}$, we have that $u$ strongly dominates $i$ with respect to $[n]\setminus \{s\}$. Thus, within the plane where $x_s = 0$, for each $i\neq u$, $H_i$ strictly separates $H_u$ from the origin. Because this separation is strict, there must be some $\epsilon > 0$ such that $H_i$ separates $H_u$ from the origin for all $x\in \R^n_{\geq 0}$ satisfying $0 \leq x_s < \epsilon$. Because the trajectory approaches this surface where $x_s =0$, after some time, the trajectory must satisfy $x_s < \epsilon$. At this point, to remain within the mixed-sign region $\cA$, the trajectory must have $\xdot_u > 0$. 

Thus, the trajectory must approach the nullcline for $x_u$. In particular, since we are increasing as we approach the nullcline, we must approach $H_u$. Thus, the trajectory also gets trapped on the negative side of each $H_i$. Therefore, since the signs of all derivatives are fixed, the trajectory must approach a limit, which must be a fixed point.  This must be the unique fixed point of the network. 
 \end{proof}

\subsection{Near CTLNs}

If a CTLN is a member of either DAG1 or DAG2, then by Theorem \ref{thm:dag_onto_symmetric} the unique fixed point is globally attracting. However, this result does not automatically extend to general TLNs. We are able to prove, however, that if a TLN has a graph $G_W$ that is a member of DAG1, and if the weights in $W$ are not too different from the CTLN weights, then the unique fixed point is a global attractor. 


\begin{prop}\label{prop:near_ctln}
Let $G$ be a member of DAG1 with a target vertex $n$. Let $W$ be a weight matrix satisfying $G_W = G$ and  for all $i,k\neq n$, $W_{nk} - W_{ik}> \frac{1}{d_{in}(i)}  (W_{in} + 1)$. Then all trajectories of a TLN defined by $W$ approach the unique fixed point. 
\end{prop}

Notice that this is a relaxation of the CTLN condition. The quantity $ \frac{1}{d_{in}(i)}  (W_{in} + 1)$ is negative, since $n$ is a sink. Now, in the CTLN case, since $n$ is a target, the quantity $W_{nk} - W_{ik}$ is always non-negative. We relax the CTLN condition by allowing the terms $W_{nk} - W_{ik}$ to be negative, but not \emph{too negative}, relative to 
$\frac{1}{d_{in}(i)}  (W_{in} + 1)$. The condition  $W_{nk} - W_{ik}> \frac{1}{d_{in}(i)}  (W_{in} + 1)$ is met on an open set of the parameter space containing the CTLN parameters. 

Our proof resembles that of Theorem \ref{thm:sources_die}, using local Lyapunov functions for a sequence of nested sets. 
\begin{figure}
\includegraphics[width =6 in]{ThresholdLinear/Figures/dag_lyapunov.pdf}

\caption{Proof idea for Proposition \ref{prop:near_ctln}. We label the vertices of $G$ with $1, \ldots, n$ according to a topological order (right).  A sequence of local Lyapunov-like functions  $L_1, \ldots, L_{n-1}$ (left) force trajectories into a nested sequence of regions $\Omega_1 \supset \Omega_2 \supset \cdots \supset \Omega_{n-1}$. }
\end{figure}

\begin{figure}
\includegraphics[width =4  in]{ThresholdLinear/Figures/composite_nested.pdf}

\caption{The regions $\Omega_1$ and $\Omega_2$ for a three-neuron network are obtained by intersecting the cones $\{x\mid x_1 \leq x_3\}$ and $\{x \mid x_1, x_2 \leq x_3\}$, illustrated here, with $\cA$. }
\end{figure}



\begin{defn}
Fix a topological ordering of the vertices of $G$ such that the source is numbered 1 and the target is numbered  $n$. 
Define 
\begin{align*}
\Omega_i(\epsilon) :&= \{ x\in \R^n_{\geq 0}\mid x_j \leq x_n +\epsilon\mbox{ for all } j \leq i\}\cap \cA\\
\Omega_i :&= \Omega_i(0)\\
\Omega_0 :&= \cA\\
\end{align*}

\end{defn}



Now, we will eventually prove that for some $\delta_i$, $L = x_i - x_n$ is a local Lyapunov function for $A = \Omega_i$, $B = \Omega_{i-1}(\delta_i)$. We will need to prove two lemmas first. 

\begin{lem}\label{lem:i_vs_n}
Under the assumptions of Proposition \ref{prop:near_ctln},
there exists a constant $\delta_i := \delta_i(W) > 0$ such that if $x\in \Omega_{i-1}(\delta_i)$, then $h_i^*(x) - h_n^*(x) < 0$. 
\end{lem}

\begin{proof}
We have 
\begin{align*}
  h_i^*(x) - h_n^*(x) = -(1 + W_{ni})x_i + (1 + W_{in})x_n + \sum_{k\to i} (W_{ik} - W_{nk})x_k + \sum_{j\not\to i}(W_{ij}-W_{nj})x_j .
\end{align*}
Notice that except for those of $ \sum_{k\to i} (W_{ik} - W_{nk})x_k$, all coefficients of this sum are non-positive.  Thus 

\begin{align*}
  h_i^*(x) - h_n^*(x) \leq  (1 + W_{in})x_n + \sum_{k\to i} (W_{ik} - W_{nk})x_k  + C,
\end{align*}

where $C = -(1 + W_{ni})x_i + \sum_{j\not\to i}(W_{ij}-W_{nj})x_j $. 

Let $a = \max_{k\to i}(W_{ik}-W_{nk})$. If $a\leq0$, then all terms of the sum are non-positive, thus we have   $h_i^*(x) - h_n^*(x) \leq 0$ throughout the positive orthant. Otherwise, we use the assumption that $x\in \Omega_{i-1}(\delta_i )$ to show that 
\begin{align*}
  h_i^*(x) - h_n^*(x) \leq (1 + W_{in})x_n + \sum_{k\to i} a x_k + C \\
  h_i^*(x) - h_n^*(x) \leq (1 + W_{in})x_n + \sum_{k\to i} a (x_n + \delta_i) +C \\
  h_i^*(x) - h_n^*(x) \leq (1 + W_{in} +d_{in}(i)a)x_n + d_{in}(i)a\delta_i + C 
\end{align*}
The term $(1 + W_{in} +d_{in}(i)a)x_n$ is negative by the assumption that  $W_{nk} - W_{ik}> \frac{1}{d_{in}(i)}  (W_{in} + 1)$. On the other hand, the term $ d_{in}(i)a\delta_i $ is positive. We show that for the appropriate $\delta_i $,  $x\in \Omega_{i-1}(\delta_i) $ implies that 
$ (1 + W_{in} +d_{in}(i)a)x_n + d_{in}(i)a\delta_i  \leq 0$. 

By Corollary  \ref{cor:total_pop}, $x\in \cA$ implies that $\sum_{\ell = 1}^n x_\ell \geq \frac{1}{-\min(W_{ij})}$. Let $c := \frac{1}{-\min(W_{ij})}$. Then $\sum_{\ell = 1}^n x_\ell \geq c$. Thus, there is some neuron $\ell$ such that $x_\ell \geq c/n$. Now, we consider two cases. First, if $\ell \leq i$, then we have $x_\ell \leq x_n + \delta$, so $x_n \geq c/n - \delta$. 
Then \begin{align*}
  h_i^*(x) - h_n^*(x) \leq (1 + W_{in} +d_{in}(i)a)\left(c/n - \delta \right)+ d_{in}(i)a\delta_i  + C
\end{align*}
  %  
Thus, for 
    
\begin{align*}
\delta_i (W) < \frac{-(1 + W_{in} + d_{in}(i)a)(c/n-\delta)}{d_{in}(i)a}
\end{align*}
we have 
\begin{align*}
  h_i^*(x) - h_n^*(x) &\leq 0
\end{align*}
as desired. 

Now, we consider the second case, when $\ell \geq i$. In this case, we expand the term $C$:

\begin{align*}
h_i^*(x) - h_n^*(x) \leq (1 + W_{in} +d_{in}(i)a)x_n + d_{in}(i)a\delta_i +  -(1 + W_{ni})x_i + \sum_{j\not\to i}(W_{ij}-W_{nj})x_j.
\end{align*}

Now, let $m = \max_{\ell \geq i}(W_{i\ell}-W_{n\ell})$. We are guaranteed $m \leq 0$, since we chose a topological ordering to label our neurons. Thus, we have

\begin{align*}
h_i^*(x) - h_n^*(x) \leq  d_{in}(i)a\delta_i + m x_\ell \\
h_i^*(x) - h_n^*(x) \leq  d_{in}(i)a\delta_i + m c/n .\\
\end{align*}

Thus, for $\delta_i \leq \frac{-mc/n}{d_{in}(i) a}$, we have $h_i^*(x) - h_n^*(x) $ as desired. 

Thus, for $$\delta_i <\frac 1 2\min\left(\frac{-mc/n}{d_{in}(i) a}, \frac{-(1 + W_{in} + d_{in}(i)a)(c/n-\delta)}{d_{in}(i)a}\right),$$
we have  $h_i^*(x) - h_n^*(x) $. 
Here $m =  \max_{\ell \geq i}(W_{i\ell}-W_{n\ell})$, $c = \frac{1}{-\min(W_{ij})}$, and $a = \max_{k\to i}(W_{ik}-W_{nk})$. 



\end{proof}



\begin{lem}
\label{lem:lyapunov_2}
Under the assumptions of Proposition \ref{prop:near_ctln},
there exists a constant $\delta_i := \delta_i(W)>0$ such that the function $L(x) = x_{i} - x_n$ is a local Lyapunov function for $A = \Omega_{i}, B = \Omega_{i-1}(\delta_i)$. 
\end{lem}

\begin{proof}


First, we notice that  for any value of $\delta \geq 0$, $L > 0$ on $\Omega_{i-1}(\delta_i)\setminus  \Omega_{i}(0)$ and $L \leq 0$ on $\Omega_{i}(0)$. Now, we show  that for the value of $\delta_i = \delta_i(W)$ used in Lemma \ref{lem:i_vs_n},  $\dot L < 0$ on $\Omega_{i-1}(\delta_i )\setminus  \Omega_{i}(0)$.  
We have 
\begin{align*}
\dot L (x) = \xdot_{i} -\xdot_n = -x_{i} + x_n + [y_{i}]_+ - [y_n]_+
\end{align*}
Pick $x\in \Omega_{i-1}(\delta_i) \setminus  \Omega_{i}(0)$ 
Since $x\notin  \Omega_{i}(0)$, we have $x_{i} > x_n$. Thus, by Lemma \ref{lem:thresh_ineq}, we have 
\begin{align*}
\xdot_{i} -\xdot_n \leq h^*_i(x) - h_n^*(x) 
\end{align*}
Now, by Lemma \ref{lem:i_vs_n}, $h^*_i(x) - h^*(n) < 0$. Thus $\dot L < 0$ on $\Omega_{i-1}(\delta_i)\setminus  \Omega_{i}(0)$.  


Finally, we check that $ \Omega_{i-1}(0)$ is a forward invariant set for our TLN. For $i = 1$, this follows from Theorem \ref{thm:mixed_sign}. For $i > 1$, this follows from the fact that $L = x_{i-1} - x_{n}$ is a local Lyapunov function for $A = \Omega_{i-1}$, $B  = \Omega_{i-2}(\delta_{i-1})$.

\end{proof}


Finally, we are ready to prove Proposition \ref{prop:near_ctln}. 

\begin{proof}[Proof of Proposition \ref{prop:near_ctln}]

We consider two cases, trajectories which do not enter $\cA$ and those which do. First, if a trajectory does not enter $\cA$, then signs of all derivatives are fixed, thus the trajectory approaches a fixed point. 

Next, we consider trajectories which enter $\cA$. We prove by induction along our topological order that for each $\epsilon> 0$, $i = 1, \ldots, n-1$, there exists $T$ such that if $t \geq T$, $x\in  \Omega_i(\epsilon)$. First, we prove the base case. Since the vertex $1$ is a source and $n$ is a target, $n$ strongly dominates $1$, so $h^*_1(x ) < h^*_n(x)$ for all $x$ in the positive orthant. Further, for $x\notin \Omega_1$, $x_1 > x_n$, so 
\begin{align*}
\xdot_1 - \xdot_n & = -x_1 + x_n + [y_1]_+ - [y_n]_+ \leq    -x_1 + x_n + y_1 - y_n\\
\xdot_1 - \xdot_n  &\leq  h^*_1(x ) - h^*_n(x) \leq 0.
\end{align*}
Thus $L= x_1 - x_n$ is a local Lyapunov like function for $\R^n_{\geq 0}, \Omega_1$. Thus, all trajectories approach $\Omega_1$. Therefore, there exists  $t \geq T$, $x(t) \in \Omega_i(\epsilon)$. 

Now, assume as an inductive hypothesis that the statement has been proved for all $j \leq i$. Pick $\epsilon > 0$. By Lemma \ref{lem:lyapunov_2}, there is a constant $\delta_i> 0$ so that  $L = x_{i+1} -x_n$ is a local Lyapunov function for $A = \Omega_i$, $B = \Omega_{i-1}(\delta) $. By the inductive hypothesis, we can choose $T_i$ so that for all $t\geq T_i$, $x\in \Omega_{i-1}(\delta_i)$. Therefore, by Lemma \ref{lem:lyapanov}, for $t> T$ the trajectory approaches $\Omega_i$. Thus, there is some $T$ such that for all $t\geq T$, $x(t) \in  \Omega_{i}(\epsilon)$.

Thus, for all $\epsilon > 0$, all trajectories enter the set $\Omega_{n-1}(\epsilon)$. Now, we pick $\delta = \max_{i \in[n]} \delta_i$. Then by Lemma \ref{lem:i_vs_n}, $h^*i(x) - h_n^*(x) < 0$ for all $x\in \Omega_{n-1}(\delta)$. This shows that the $x_n$ nullcline is separated from the origin by each $x_i$ nullcline within $\Omega_{n-1}(\delta)$.  Thus $\Omega_{n-1}(\delta) \subseteq H_n^+$. By our inductive argument, all trajectories which enter $\cA$ eventually enter the region $\Omega_{n-1}(\delta)$. Once they enter this region, $\xdot_n > 0$ for all time. Thus, the value of $x_n$ becomes monotonically increasing. Thus, it must approach a limit on $H_n$. Since $H_n$ is contained on the negative side of all other $H_i$, the signs of all derivatives $\xdot_i$ are fixed. Thus, the trajectory must approach the unique fixed point of the network.


\end{proof}





==> eqparbox/README <==
                  +--------------------------------+
                  |EQPARBOX: Equal-widthed parboxes|
                  |By Scott Pakin <pakin@uiuc.edu> |
                  +--------------------------------+


Description
-----------

LaTeX users sometimes need to ensure that two or more blocks of text
occupy the same amount of horizontal space on the page.  To that end,
the eqparbox package defines a new command, \eqparbox, which works
just like \parbox, except that instead of specifying a width, one
specifies a tag.  All eqparboxes with the same tag -- regardless of
where they are in the document -- will stretch to fit the widest
eqparbox with that tag.  This simple, equal-width mechanism can be
used for a variety of alignment purposes, as is evidenced by the
examples in eqparbox's documentation.


Installation
------------

There's nothing special about building eqparbox:

    latex eqparbox.ins     <== Generate eqparbox.sty
    latex eqparbox.dtx     <== Produce the documentation (eqparbox.dvi)
    latex eqparbox.dtx     <== Again, to get labels and eqparboxes right
    makeindex -s gind.ist eqparbox    <== Generate an index
    latex eqparbox.dtx     <== Incorporate the index into the document

If you're new to this, see
http://www.tex.ac.uk/cgi-bin/texfaq2html?label=instpackages for more
information on installing packages.


Copyright and license
---------------------
Copyright (C) 2001 Scott Pakin <pakin@uiuc.edu>

This package may be distributed and/or modified under the conditions
of the LaTeX Project Public License, either version 1.2 of this
license or (at your option) any later version.  The latest version of
this license is in:

    http://www.latex-project.org/lppl.txt

and version 1.2 or later is part of all distributions of LaTeX version
1999/12/01 or later.


==> shortcuts.tex <==



%Theorems
\theoremstyle{definition}
\newtheorem{thm}{Theorem}[chapter]
\newtheorem*{thm*}{Theorem}
\newtheorem{ithm}{Theorem}[chapter]
\newtheorem{cor}{Corollary}[chapter]
\newtheorem{conj}{Conjecture}[chapter]
\newtheorem{lem}{Lemma}[chapter]
\newtheorem{prop}{Proposition}[chapter]
\newtheorem{defn}{Definition}[chapter]
\newtheorem{ex}{Example}[chapter]
\newtheorem{obs}{Observation}[chapter]
\newtheorem{question}{Question}[chapter]
\newtheorem*{question*}{Question}
\newtheorem{const}{Construction}[chapter]

\newcommand{\scC}{\mathcal C}
\newcommand{\scD}{\mathcal D}
\newcommand{\scE}{\mathcal E}
\newcommand{\scH}{\mathcal H}
\newcommand{\scM}{\mathcal M}





\newcommand{\cC}{\mathcal C}
\newcommand{\cU}{\mathcal U}
\newcommand{\cN}{\mathcal N}
\newcommand{\cT}{\mathcal T}
\newcommand{\cM}{\mathcal M}
\newcommand{\cA}{\mathcal A}
\newcommand{\cL}{\mathcal L}
\newcommand{\cE}{\mathcal E}
\newcommand{\cD}{\mathcal D}
\newcommand{\cF}{\mathcal F}
\newcommand{\cV}{\mathcal V}
\newcommand{\cH}{\mathcal H}
\newcommand{\cW}{\mathcal W}
\newcommand{\cP}{\mathcal P}
\newcommand{\cR}{\mathcal R}
\newcommand{\cQ}{\mathcal Q}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Sans Serif
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\sfD{\mathsf{D}}
\def\sfF{\mathsf{F}}
\def\sfI{\mathsf{I}}
\def\sfK{\mathsf{K}}
\def\sfL{\mathsf{L}}
\def\sfP{\mathsf{P}}
\def\sfR{\mathsf{R}}
\def\sfS{\mathsf{S}}
\def\sfT{\mathsf{T}}
\def\sfW{\mathsf{W}}


\newcommand{\pq}{\overline{pq}}
\newcommand{\lra}{\leftrightarrow}







\newcommand{\R}{\mathbb R}
\newcommand{\E}{\mathbb E}
\newcommand{\F}{\mathbb F}

\newcommand{\bS}{\mathbb S}



\newcommand{\xdot}{\dot x}

\DeclareMathOperator{\odim}{odim}
\DeclareMathOperator{\cdim}{cdim}
\DeclareMathOperator{\ndim}{ndim}
\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\cl}{cl}
\DeclareMathOperator{\Int}{int}
\DeclareMathOperator{\code}{code}
\DeclareMathOperator{\nerve}{nerve}
\DeclareMathOperator{\link}{link}
\DeclareMathOperator{\trunk}{trunk}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\FP}{FP}
\DeclareMathOperator{\ur}{urank}
\DeclareMathOperator{\monr}{mrank}
\DeclareMathOperator{\order}{order}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\radr}{radrank}
\DeclareMathOperator{\vertices}{Vert}
\DeclareMathOperator{\sep}{sep}
\DeclareMathOperator{\tk}{trunk}

\newcommand{\aff}{\mathrm{aff}}




\def \shatter{\Delta_{\mathrm{sh}}}
\def \sweep{\Delta_{\mathrm{sw}}}
\newcommand{\pcode}{P_{\code}}






\newcommand{\wt}{\widetilde}
\newcommand{\inv}{^{-1}}

\renewcommand{\emptyset}{\varnothing}



%%% Categories
\DeclareMathOperator{\Code}{\mathbf{Code}}
\DeclareMathOperator{\OMlong}{\mathbf{OrientedMatroid}}
\DeclareMathOperator{\OM}{\mathbf{OM}}
\DeclareMathOperator{\OMatroid}{\mathbf{OM}}
\DeclareMathOperator{\COMlong}{\mathbf{ConditionalOrientedMatroid}}
\DeclareMathOperator{\COM}{\mathbf{COM}}
\DeclareMathOperator{\AOMlong}{\mathbf{AffineOrientedMatroid}}
\DeclareMathOperator{\AOM}{\mathbf{AOM}}
\DeclareMathOperator{\NRing}{\mathbf{NRing}}
\DeclareMathOperator{\Ring}{\mathbf{Ring}}
\DeclareMathOperator{\OMRing}{\mathbf{OMRing}}


